Computing the Haar state of $\mathcal{O}(SL_q(3))$ using value preserving (anti)homomorphisms

In this paper, we introduce two (anti)homomorphisms that preserve the Haar state values of monomials. Together with the modular automorphism, the three (anti)homomorphisms are used in our new algorithm to compute the Haar states of monomials on $\mathcal{O}(SL_q(3))$. Comparing with the algorithm proposed in the author's previous work \cite{lu2023}, the new algorithm reduces the linear relations used in the computation to a half.

==> Chapters/Comul.tex <==
\section{Comultiplication of standard monomials}
Theorem 1 (b) tells us that to compute the Haar state on $\mathcal{O}(SL_q(n))$, it suffices to compute the Haar state of standard monomials. We will use the defining relation $((id\otimes h)\circ \Delta)(x)=h(x)\cdot 1=((h\otimes id)\circ \Delta)(x)$ to compute the Haar state of standard monomials. We start with the investigation of the comultiplication of monomials.
\begin{lemma}\label{Lemma 2}
    Let $x$ be a monomial and we write:
\begin{equation*}
    \Delta(x)=\sum_{i\in I} z_i\otimes y_i,
\end{equation*}
with $I$ an index set and $y_i,z_i$ (non-standard) monomials. Then:
\begin{equation*}
    \alpha(\eta(x))=\alpha(\eta(z_i))\ \ \ \beta(\eta(x))=\beta(\eta(y_i))\ \ \ \beta(\eta(z_i))=\alpha(\eta(y_i)).
\end{equation*}
\end{lemma}
\begin{remark}
    We will say $z_i$ is the \textbf{left component} of the tensor product and $y_i$ is the \textbf{right component} of the tensor product.
\end{remark}
\begin{proof}
    Recall that $\Delta(x_{ij})=\sum_{k=1}^nx_{ik}\otimes x_{kj}$ and $\Delta$ is a morphism of algebra. If $x=\Pi_{l=1}^p x_{i_lj_l}$, then
\begin{equation*}
    \Delta(x)=\Delta(\Pi_{l=1}^p x_{i_l,j_l})=\Pi_{l=1}^p\Delta(x_{i_l,j_l})=\prod_{l=1}^p\left(\sum_{k=1}^nx_{i_l,k}\otimes x_{k,j_l}\right)=\sum_{i\in I} z_i\otimes y_i.
\end{equation*}
For each $z_i$ the $l$-th generator is in the same row as the $l$-th generator in $x$, and for each $y_i$ the $l$-th generator is in the same column as the $l$-th generator in $x$. The column index of the $l$-th generator in $z_i$ is the same as the row index of the $l$-th generator in $y_i$. Thus, the row sum of $x$ equals the row sum of $z_i$; the column sum of $x$ equals the column sum of $y_i$, and the column sum of $z_i$ equals the row sum of $y_i$. 
\end{proof}
\noindent With Lemma \ref{Lemma 2}, we have the following result:

\begin{lemma}\label{Lemma 3}
    If $\eta(x)\in A_n(m)$ then $h(y_i)\ne 0$ (or $h(z_i)\ne 0$) if and only if $\eta(y_i)\in A_n(m)$ ( or $\eta(z_i)\in A_n(m)$). Moreover, $\eta(y_i)\in A_n(m)$ if and only if $\eta(z_i)\in A_n(m)$.
\end{lemma}
\begin{proof}
    Use Theorem 1 a) and Lemma \ref{Lemma 2}.
\end{proof}
\noindent Now, we are ready to prove:\\
\\
\textbf{Theorem 1 c)}: \textit{Let $\{s_l\}_{l\in \mathcal{I}_m}$,  be the set of standard monomials of order $m$. Then, we can write $(Id\otimes h)\circ\Delta(s_l)$ and $(h\otimes Id)\circ\Delta(s_l)$ as linear combinations of $s_j$'s and the coefficient of each $s_j$ is a linear combination of $h(s_i)$'s.}
\begin{proof}
    If $s_l\in B_n(m)$ is a standard monomial, Lemma \ref{Lemma 3} implies that
\begin{equation}
    (id\otimes h)\circ\Delta(s_l)=\sum_{\substack{y\in B_n(m)\\ z\in B_n(m)}} h(y)\cdot z
    \label{ep:4}
\end{equation}
Then, by Lemma \ref{Lemma 1}, we can decompose each $y$ and $z$ as:
\begin{equation}
    y=\sum_{j=1}^{k} d_j^{y}\cdot s_j,
    \label{ep:1}
\end{equation}
\begin{equation}
    z=\sum_{j=1}^{k} d_j^{z}\cdot s_j.
    \label{ep:2}
\end{equation}
Substitute Equation~(\ref{ep:1}) and Equation~(\ref{ep:2}) into Equation~(\ref{ep:4}), we get:
\begin{equation}
    (id\otimes h)\circ\Delta(s_l)=\sum_{j=1}^k\left(\sum_{i=1}^kc_{ij}h(s_i)\right)\cdot s_j.
    \label{eq:2}
\end{equation}
\end{proof}

\begin{remark}
Here, $\{s_i\}_{i=1}^k\subset\{s_l\}_{l\in \mathcal{I}_m}$ is a basis of standard monomials of order $m$. We will say $\boldsymbol{z_i}$ {\bf (or $\boldsymbol{y_i}$) contains} $\boldsymbol{s_j}$ if $d_j^{z_i}\ne 0$ (or $d_j^{y_i}\ne 0$).
\end{remark}

\hfill

 \noindent Since we can identify $1$ with $D_q^m$, we get $(id\otimes h)\circ\Delta(s_l)=h(s_l)\cdot D_q^m$. Notice that we can decompose $D_q^m$ as a linear combination of standard monomials of order $m$. Thus, by comparing the coefficient of the same standard monomial on both sides of $(id\otimes h)\circ\Delta(s_l)=h(s_l)\cdot D_q^m$, we can find a linear relation consisting of the Haar states of standard monomials of order $m$. We call such a linear relation {\bf linear relation of order} $\boldsymbol{m}$. We call a linear system consisting of linear relations of order $m$ a {\bf linear system of order} $\boldsymbol{m}$.

 \begin{remark}
     We can use the relation $(h\otimes id)\circ\Delta(s_l)=h(s_l)\cdot D_q^m$ to construct linear relation of order $m$ as well. But in this paper, all linear relation of order $m$ is derived from $(id\otimes h)\circ\Delta(s_l)=h(s_l)\cdot D_q^m$.
 \end{remark}

==> Chapters/Higher_order.tex <==
\section{Liner relations of higher order}
In this section, let $\{s_l\}_{l=1}^{K_m}$ be a set of linearly independent standard monomials of order $m$. Recall Equation~(\ref{eq:2}):
\begin{equation*}
\begin{split}
    (id\otimes h)\circ\Delta(s_l)=\sum_{j=1}^{K_m}\left(\sum_{i=1}^{K_m}c_{ij}h(s_i)\right)\cdot s_j.
\end{split}
\end{equation*}
We can do the same thing to $h(s_l)\cdot 1=h(s_l)\cdot D_q^m$ and get:
\begin{equation}
    h(s_l)\cdot 1=h(s_l)\cdot D_q^m=\sum_{j=1}^{K_m} b_jh(s_l)\cdot s_j.
    \label{ep:3}
\end{equation}

\hfill

\noindent By comparing the coefficients of standard bases in $(id \otimes h)\circ\Delta(s_l)$ and in $h(s_l)\cdot 1$, we get:
\begin{equation} 
    \sum_{i=1}^{K_m}c_{ij}h(s_i)=b_jh(s_l)
    \label{eq:3}
\end{equation}
for every $1\le j\le K_m$. We will call Equation~(\ref{eq:3}) the \textbf{linear relation derived from equation basis $\boldsymbol{s_l}$ and comparing basis $\boldsymbol{s_j}$}. Each index $1\le l\le K_m$ corresponds to $K_m$ linear relations, so there are $K_m^2$ linear relations. Since there are $K_m$ unknowns, it is possible to construct more than one system of order $m$. Notice that these linear relations all have the zero right-hand side. One way to get a linear relation with the non-zero right-hand side is by decomposing $1=h(1)=h(D_q^m)$ into a sum of standard monomials. Although we can construct more than one system of order $m$, not every system is invertible. We will give a more robust approach to compute the Haar state of $\mathcal{O}(SL_q(3))$ later. \\
\\
In the order 1 case, finding Equation (\ref{eq:2}) and (\ref{ep:3}) is an easy task. However, the situation is much more complicate in higher order case. To understand the difficulty to find the two equations in higher order case, we introduce the \textbf{order restriction} for each summand appearing in the comultiplication of a monomial:\\
\\
\textit{Let $x=\prod_{k\in I}x_{i_k,j_k}$ be a monomial and the comultiplication of $x$ be
\begin{equation*}
    \Delta(x)=\prod_{k\in I}\Delta(x_{i_k,j_k})=\prod_{k\in I}\left(\sum_{l_k=1}^nx_{i_k,l_k}\otimes x_{l_k,j_k}\right)=\sum_{i\in I'} z_i\otimes y_i.
\end{equation*}
Then:
\begin{itemize}
    \item[i)] the $k$-th generator of the left component $z_i$ is in the $i_k$-th row
    \item[ii)] the $k$-th generator of the right component $y_i$ is in the $j_k$-th column
    \item[iii)] The column index of the $l$-th generator in $z_i$ equals to the row index of the $l$-th generator in $y_i$.
\end{itemize}}
\noindent The order restriction is a direct consequence of the fact that the comultiplication is an algebra homomorphism. Since each index $l_k$ ranges from $1$ to $n$, every possible combination of $z_i\otimes y_i$ that satisfies the order restriction will appear in the summation of $\Delta(x)$. In higher order case, this means that Equation (\ref{ep:4}) includes not only summand whose left and right components are standard monomials but also summand whose left and right components are reordering of standard monomials satisfying the order restriction. As an example in $\mathcal{O}(SL_q(3))$, if $(x_{1,1}x_{2,3}x_{3,2})(x_{1,2}x_{2,1}x_{3,3})$ is the left component of one of the tensor products in $\Delta\left((x_{1,1}x_{2,2,}x_{3,3})^2\right)$ then all reordering of the left component satisfying property i) of the order restriction are:
\begin{multicols}{2}
\begin{itemize}
    \item[1)] $(x_{1,1}x_{2,3}x_{3,2})(x_{1,2}x_{2,1}x_{3,3})$
    \item[2)] $(x_{1,2}x_{2,3}x_{3,2})(x_{1,1}x_{2,1}x_{3,3})$
    \item[3)] $(x_{1,1}x_{2,1}x_{3,2})(x_{1,2}x_{2,3}x_{3,3})$
    \item[4)] $(x_{1,1}x_{2,3}x_{3,3})(x_{1,2}x_{2,1}x_{3,2})$
    \item[5)] $(x_{1,2}x_{2,1}x_{3,2})(x_{1,1}x_{2,3}x_{3,3})$
    \item[6)] $(x_{1,2}x_{2,3}x_{3,3})(x_{1,1}x_{2,1}x_{3,2})$
    \item[7)] $(x_{1,1}x_{2,1}x_{3,3})(x_{1,2}x_{2,3}x_{3,2})$
    \item[8)] $(x_{1,2}x_{2,1}x_{3,3})(x_{1,1}x_{2,3}x_{3,2})$.
\end{itemize}
\end{multicols}
\noindent Thus, the comultipilcation of a standard monomial of higher order contains not only standard monomials but also variations of standard monomials satisfying the order restriction. This is the major difference between the case of order 1 and higher order cases. To find a linear relation derived from equation basis $s_l$ and comparing basis $s_j$ in higher order case, we have to:
\begin{itemize}
    \item[i)]find all left (or right) component appearing in $\Delta(s_l)$ that contains $s_j$ and compute the corresponding coefficient $d_j^{z}$ in Equation~(\ref{ep:2});
    \item[ii)] find the decomposition of the right (or left) component in $\Delta(s_l)$ corresponding to the left (or right) component in i) and sum all such decomposition together to get a linear relation;
    \item[iii)] decompose every summand containing $s_j$ in Equation~(\ref{ep:3}) to find $b_j$.
\end{itemize}
All 3 steps involve decomposing non-standard monomials into a linear combination of standard monomials and such decomposition is not easy in general. However, there is a simple criterion to determine whether a standard monomial appears in the decomposition of a non-standard monomial or not.

\hfill

\noindent\textbf{Theorem 1 e)}:\textit{When changing the order of generators in a monomial, the newly generated monomials cannot contain more generator $x_{1,1}$ and $x_{n,n}$ and cannot contain less generator $x_{1,n}$ and $x_{n,1}$ comparing to the monomial being reordered.}

\begin{proof}
    When a new monomial is generated, we replace a pair of $x_{i,k}x_{j,l}$ ($i<j,k<l$) by a pair of $x_{i,l}x_{j,k}$ to get the new monomial. Notice that none of $x_{i,k}$ and $x_{j,l}$ can be $x_{1,n}$ or $x_{n,1}$ and none of $x_{i,l}$ and $x_{j,k}$ can be $x_{1,1}$ or $x_{n,n}$. Thus, $x_{1,n}$ and $x_{n,1}$ can never be replaced by other generators and $x_{1,1}$ and $x_{n,n}$ can never be used as the generator to replace other generators. This finishes the proof.
\end{proof}
\begin{remark}
    The decomposition of a monomial $x$ does not contain those standard monomials whose number of generator $x_{11}$ and $x_{nn}$ (or $x_{1n}$ and $x_{n1}$) exceeds (or less than) that of monomial $x$.
\end{remark}
\noindent Notice that every standard monomial in $\mathcal{O}(SL_q(3))$ contains at least one of $x_{11}$, $x_{13}$, $x_{31}$, and $x_{33}$. Thus, Theorem 1 e) will play an important role in the computation of the Haar state on $\mathcal{O}(SL_q(3))$ later.


==> Chapters/Intro.tex <==
\section{Introduction}
The Haar measure on a compact topological group is a well-studied object. In particular, when the group is $U(n)$, the group of $n\times n$ unitary matrices, there is an elegant formula for the integral of matrix coefficients with respect to the Haar measure. This formula is given by so-called Weingarten functions, introduced by Collins in 2003~\cite{collins2003moments}. The current paper will study a $q$-deformation of the Haar measure on the Drinfeld--Jimbo~\cite{drinfeld1986quantum}~\cite{jimbo1985aq} quantum groups $\mathcal{O}(SL_q(n))$ which is dual to $U_q(sl_n)$~\cite{korogodski1998algebras}.

\hfill

\noindent In the context of $\mathcal{O}(SL_q(n))$, the most relevant algebraic structure is that it is a co-semisimple Hopf algebra. From Sweedler~\cite{sweedler1969hopf}, any co-semisimple Hopf algebra has a unique ``Haar state'' up to normalization. In the context here, co-semisimplicity plays the role of compactness: the Lie algebra of a compact Lie group is always a semisimple Lie algebra. In particular, when $q\rightarrow 1$, the space of functions $O(SL(n))$ on $SL(n)$ is a co-semisimple Hopf algebra, and its Haar state is simply the integral of a function with respect to Haar measure. 

\hfill

\noindent In the $q$-deformed case, there are no explicit formulas in terms of parameter $q$ for the Haar state $\mathcal{O}(SL_q(n))$ except when $n=2$ (Klimyk and Schm{\"u}dgen~\cite{klimyk2012quantum}). The difficulty when $n>2$ arises from the form of the $q$--determinant. When $n=2$, the $q$-determinant is of the form $ad-qbc=1$, where $a,b,c,d$ are the generators of $\mathcal{O}(SL_q(2))$. Because the $q$-determinant only has two terms, once the Haar state of $bc$ is computed, then so is the Haar state of $ad$. However, this simplification does not work in general because the $q$-determinant generally has $n!$ terms. For other related works on $\mathcal{O}(SL_q(n))$, see Nagy~\cite{nagy1993haar}, Vaksman and Soibelman~\cite{vaksman1990algebra}~\cite{levendorskii1991algebras}.

\hfill

\noindent In this paper, the generator of $\mathcal{O}(SL_q(n))$ is denoted as $x_{i,j}$ for $1\le i,j\le n$. 
\begin{definition}
The {\bf{counting matrix}} of a monomial $x\in \mathcal{O}(SL_q(n))$, denoted as $\eta(x)$, is a $n\times n$ matrix with entries $a_{ij}, i,j=1,\dots,n$ where $a_{ij}$ equals the number of appearance of generator $x_{i,j}$ in $x$.
\end{definition}
\begin{definition}
    The \textbf{{row sum}} and \textbf{{column sum}} of a $n\times n$ matrix $A=(a_{ij})_{i,j=1}^n$, denoted as $\alpha(A)$ and $\beta(A)$, are vectors in $\mathbb{R}^n$:
\begin{equation*}
\begin{split}
    \alpha(A)=\left( \sum_{j=1}^n a_{ij} \right)_{i=1}^n, \ \ \ \ \ \ 
    \beta(A)=\left( \sum_{i=1}^n a_{ij} \right)_{j=1}^n.
\end{split}
\end{equation*}
Here, we denote $(k)_{i=1}^n$ as a vector whose entries all equal to $k$.
\end{definition}
\begin{definition}
    Let $A$ be a $n\times n$ matrix with non-negative integer entries. Then $A$ is a \textbf{$\boldsymbol{k}$-doubly stochastic matrix}~\cite{stein1970enumeration} if there is a positive integer $k$ such that $\alpha(A)=(k)_{i=1}^n=\beta(A)$. 
\end{definition}
\begin{definition}
    Let $S_n$ be the permutation group on $n$ letters. Monomials in form $\prod_{\sigma_i\in S_n}(x_{\sigma_i})^{m_i}$, where $m_i\in \mathbb{N}_0$ and $x_{\sigma_i}=\prod_{k=1}^nx_{k,\sigma_i(k)}$ and $(x_{\sigma_i})^0=1$, are called \textbf{standard monomials}. $m=\sum_{i=1}^{n!}m_i$ is called the \textbf{order} and each $x_{\sigma_i}$ is called a \textbf{segment}.
\end{definition}
\noindent The current paper will prove the following theorem on $\mathcal{O}(SL_q(n))$:
\begin{theorem}
The following are true on $\mathcal{O}(SL_q(n))$:
\begin{itemize}
    \item[a)] Let $x$ be a monomial. Then $h(x)\ne 0$ implies that there exist $k\in \mathbb{N}^+$ such that $\eta(x)$ is a ${k}$-doubly stochastic matrix.
    \item[b)] Every monomial with non-zero Haar state value can be written as a linear combination of standard monomials.
    \item[c)]Let $s_l$, $l\in \mathcal{I}_m$ be the set of standard monomials of order $m$. Then, we can write $(Id\otimes h)\circ\Delta(s_l)$ and $(h\otimes Id)\circ\Delta(s_l)$ as linear combinations of $s_j$'s and the coefficient of each $s_j$ is a linear combination of $h(s_i)$'s.
    \item[d)] Let $l(\tau)$ be the inverse number of $\tau\in S_n$. Then :
    \begin{equation*}
    h\left(\prod_{k=1}^nx_{k,\tau(k)}\right)=\frac{(-q)^{l(\tau)}}{\sum_{\sigma\in S_n} (-q)^{2l(\sigma)}}=\frac{(-q)^{l(\tau_i)}}{[n]_{q^2}!},
    \end{equation*}
    where $[n]_{q^2}=\frac{1-q^{2n}}{1-q^2}$ and $[n]_{q^2}!=\prod_{j=1}^n[j]_{q^2}$
    \item[e)] When changing the order of generators in a monomial, the newly generated monomials cannot contain more generator $x_{11}$ and $x_{nn}$ and cannot contain less generator $x_{1n}$ and $x_{n1}$, comparing to the monomial being reordered.
    \item[f)] Define the double flip anti-homomorphism $\omega$ on $\mathcal{O}(SL_q(n))$ as:
    $$\omega(x_{i,j})=x_{n+1-i,n+1-j}$$
    Then, $h\circ\omega(x)=h(x)$ for any $x\in\mathcal{O}(SL_q(n))$
\end{itemize}
\end{theorem}
\noindent For simplicity, the generators of on $\mathcal{O}(SL_q(3))$ are denoted as:
\begin{equation*}
\begin{matrix}
a&b&c\\
d&e&f\\
g&h&k.
\end{matrix}
\end{equation*}
Then, standard monomials of order $m=c_1+c_2+c_3+c_4+c_5+c_6$ are in the form:
$$(aek)^{c_1}(afh)^{c_2}(bdk)^{c_3}(bfg)^{c_4}(cdh)^{c_5}(ceg)^{c_6}.$$
\begin{definition}
    Segments $aek$, $afh$, and $bdk$ are {\bf high-complexity segments}. 
\end{definition}
\begin{definition}
    Segments $bfg$, $cdh$, and $ceg$ are {\bf low-complexity segments}.
\end{definition}
\begin{remark}
    low-complexity segments commutes with each other but high-complexity segments do not commute with any other segments. For more details, check Equation (\ref{apeq:1}) --- (\ref{apeq:6}).
\end{remark}
\noindent On $\mathcal{O}(SL_q(3))$, we will define a monomial basis consisting of standard monomials. Then, an explicit recursive relations for the Haar state of those standard monomials with low-complexity segments only is provided. Finally, an algorithm is proposed to compute the Haar states of standard monomials with high-complexity segments.

==> Chapters/Linear_subspace.tex <==
\section{Linear subspace of elements with non-zero Haar state}
Let $\mathcal{NZ}$ be the linear subspace of elements with non-zero Haar state. We write $A_n(m),\ m\in \mathbb{N}^+$ as the set of $n\times n$ $m$-doubly stochastic matrices and $B_n(m)$ as the set of monomials on $\mathcal{O}(SL_q(n))$ whose counting matrices belong to $A_n(m)$. Theorem 1(a) tells us:
$$\mathcal{NZ}\subset\text{span}\left\langle\bigcup_{m=0}^{\infty} B(m)\right\rangle$$
Thus, to compute the Haar state on $\mathcal{O}(SL_q(n))$, it suffice to study each $\text{span}\langle B_n(m)\rangle$. We will give a criterion to pick a basis of $\text{span}\langle B_n(m)\rangle$.

\hfill

\noindent First, we introduce a total order '$<$' on $A_n(m)$.
For every $C=(c_{ij})_{i,jk=1}^n\in A_n(m)$, we associate a vector 
\begin{equation*}
    \mathcal{V}(C)=(c_{11},c_{12},\dots,c_{1n},c_{21},c_{22},\dots,c_{nn}),
\end{equation*}
and we compare such vectors in lexicographic order. We say matrices $C<D$ if $\mathcal{V}(C)<\mathcal{V}(D)$. With this total order, we have the following observation:

\hfill

\noindent{\it If $x=P\cdot x_{ik}x_{jl}\cdot Q\in B_n(m)$ $(i<j,k<l)$ where $P,Q$ are two monomials and we switch the order of $x_{ik}x_{jl}$ so that:}
\begin{equation*}
    x=y+(q-q^{-1})z,
\end{equation*}
{\it where $y=P\cdot x_{jl}x_{ik}\cdot Q$ and $z=P\cdot x_{il}x_{jk}\cdot Q$, then $y,z\in B_n(m)$ and $\eta(z)<\eta(x)=\eta(y)$.} 

\hfill

\noindent Based on the observation, we get the following lemma:
\begin{lemma}\label{Lemma 1}
    For each $M\in A_n(m)$, we fix monomial $x_M\in B_n(m)$ such that $\eta(x_M)=M$. If $\phi\in B_n(m)$ is a monomial with counting matrix $M$, then we can decompose $\phi$ as:
\begin{equation}
    \phi=c_M\cdot x_M+\sum_{\substack{P<M\\P\in A_n(m)}}c_P\cdot x_P.
    \label{eq:1}
\end{equation}
\end{lemma}
\begin{remark}
    Lemma \ref{Lemma 1} provides a criterion for picking a basis for each $B_n(m)$.
\end{remark}
\begin{proof}
    Since $\phi$ and $x_M$ have the same counting matrix, we can permute the generators in $\phi$ to the same order as in $x_M$. We denote this process as a chain:
\begin{equation*}
    \phi=\phi_0\rightarrow \phi_1\rightarrow\phi_2\rightarrow\cdots\rightarrow \phi_k=x_M,
\end{equation*}
where each $\phi_i$ is a reordering of $\phi$ and we get $\phi_{i+1}$ by switching the order of two adjacent generators in $\phi_i$. From $\phi_i$ to $\phi_{i+1}$, we may get a new term $\varphi_{i+1}$. As discussed before, $\eta(\varphi_{i+1})\in A_n(m)$ and $\eta(\varphi_{i+1})<\eta(\phi_{i+1})=M$. We can permute these newly generated $\varphi_i$'s to their corresponding $x_{\eta(\varphi_{i+1})}$'s, and we may get new terms in this process as well. However, each time we repeat this permuting process to a monomial $y$, the counting matrix of the newly generated monomial is always smaller than $\eta(y)$. Since the counting matrix of the newly generated monomial is always descending, we can finish this permuting process in finite steps. In other words, we will get a chain on which every transposition does not generate new monomials. Then, every monomial appearing in the summation will be in the desired form, and we get Equation~(\ref{eq:1}).
\end{proof}

\hfill

\noindent\textbf{Theorem 1 b)}: \textit{Every monomial with non-zero Haar state value can be written as a linear combination of standard monomials.}
\begin{proof}
    By the {\bf Birkhoff-Von Neumann Theorem}~\cite{birkhoff1946three}~\cite{von1953certain}, every $M\in A_n(m)$ can be decomposed into $M=m_1\sigma_1+m_2\sigma_2+\cdots +m_{n!}\sigma_{n!}$, where $\sigma_i$'s are matrix in $A_n(1)$ and $m_i$'s are non-negative integers whose sum is $m$. Notice that each matrix $\sigma_i$ can be identified with a permutation on $n$ letters. We denote the corresponding permutation as $\sigma_i$ as well. Then, the counting matrix of the monomial $\prod_{\sigma_i\in S_n}(x_{\sigma_i})^{m_i}$ is $M$. This implies that for every $M\in A_n(m)$, we can choose $x_M$ in form $\prod_{\sigma_i\in S_n}(x_{\sigma_i})^{m_i}$. Combining with Lemma \ref{Lemma 1}, the statement in Theorem 1 b) is clear. 
\end{proof}

\hfill

\noindent Notice that the set of standard monomials of order $m$ contains a monomial basis of $\text{span}\langle B_n(m)\rangle$, but the set itself is not a basis of $\text{span}\langle B_n(m)\rangle$. The reason is that different standard monomials could have the same counting matrix and standard monomials with the same counting matrix are linearly dependent(see Equation (\ref{apeq:7}) at the beginning of Part II). When $n,m$ is large, given $M\in A_n(m)$ it is difficult to find all standard monomials whose counting matrices are $M$. However, we will provide a criterion to pick a monomial basis from the set of all standard monomials on $\mathcal{O}(SL_q(3))$ later.


==> Chapters/Linear_sys_1.tex <==
\section{System of order 1}
In this section, we will prove Theorem 1 d). The standard basis for $B_n(1)$ is in the form of $x_{\tau_i}=\Pi_{k=1}^nx_{k,\tau_i(k)}$ where $\tau_i$ is a permutation on $n$ letters. We have:
\begin{equation*}
    \Delta(x_{\tau_i})=\Delta(\Pi_{k=1}^nx_{k,\tau_i(k)})=\displaystyle{\prod_{k=1}^n\left(\sum_{p=1}^nx_{k,p}\otimes x_{p,\tau_i(k)}\right)}.
\end{equation*}
By Lemma \ref{Lemma 3}, after applying $(id\otimes h)$ to $\Delta(x_{\tau_i})$, we get:
\begin{equation}
    \begin{split}
        (id\otimes h)\circ\Delta(x_{\tau_i})=\sum_{\sigma_j\in S_n}h( \Pi_{k=1}^nx_{\sigma_j(k),\tau_i(k)})\cdot\Pi_{k=1}^nx_{k,\sigma_j(k)}. 
    \end{split}\label{eq:linear}
\end{equation}
On the other hand, recall that
\begin{equation}
    1=D_q=\sum_{\sigma_j\in S_n} (-q)^{l(\sigma_j)}\prod_{k=1}^nx_{k,\sigma_j(k)},
    \label{eq:dp}
\end{equation}
where $l(\sigma_j)$ is the inverse number of $\sigma_j$.

\hfill

\noindent Thus, using $(id\otimes h)\circ\Delta(x_{\tau_i})=h(x_{\tau_i})\cdot 1$ and comparing the coefficients of each standard basis, we get for every $\sigma_j \in S_n$:
\begin{equation}
    h( \Pi_{k=1}^nx_{\sigma_j(k),\tau_i(k)})=(-q)^{l(\sigma_j)}h(x_{\tau_i}).
    \label{eq:4}
\end{equation}
In general, $\Pi_{k=1}^nx_{\sigma_j(k),\tau_i(k)}$ is not a standard monomial. However, if we choose $\sigma_j$ such that $\sigma_j(k)=n+1-\tau_i(k)$, then every generator in $\Pi_{k=1}^nx_{\sigma_j(k),\tau_i(k)}$ commutes with each other and $\Pi_{k=1}^nx_{\sigma_j(k),\tau_i(k)}=\Pi_{k=1}^nx_{k,n+1-k}$. Moreover, $l(\sigma_j)=\frac{n(n-1)}{2}-l(\tau_i)$. Thus, from Equation~(\ref{eq:4}) we get:
\begin{equation}
    h(\Pi_{k=1}^nx_{k,n+1-k})=(-q)^{\frac{n(n-1)}{2}-l(\tau_i)}h(\Pi_{k=1}^nx_{k,\tau_i(k)}).
    \label{eq:5}
\end{equation}
Therefore, using Equation~(\ref{eq:5}) and Equation~(\ref{eq:dp}) we get:
\begin{equation}
\begin{split}
    1&=h(1)=\sum_{\sigma_j\in S_n} (-q)^{l(\sigma_j)}h(\Pi_{k=1}^nx_{k,\sigma_j(k)})\\
    &=\left(\sum_{\sigma_j\in S_n} (-q)^{2l(\sigma_j)-\frac{n(n-1)}{2}}\right)h(\Pi_{k=1}^nx_{k,n+1-k}),
\end{split}
\end{equation}
which gives
\begin{equation}
    h(\Pi_{k=1}^nx_{k,n+1-k})=\frac{(-q)^{\frac{n(n-1)}{2}}}{\sum_{\sigma_j\in S_n} (-q)^{2l(\sigma_j)}}.
\end{equation}
Then by Equation~(\ref{eq:4}), notice that the inverse number for the $\tau_i$ corresponding to $\Pi_{k=1}^nx_{k,n+1-k}$ is just $\frac{n(n-1)}{2}$, we get for every $\tau_i\in S_n$:
\begin{equation}
    h(\Pi_{k=1}^nx_{k,\tau_i(k)})=\frac{(-q)^{l(\tau_i)}}{\sum_{\sigma_j\in S_n} (-q)^{2l(\sigma_j)}}.
    \label{eq:sys1}
\end{equation}
Let $I_n(k)$ be the number of permutations on $n$ letters with $k$ inversions. Then, the denominator of Eq(\ref{eq:sys1}) can be rewritten as:
\begin{equation*}
    \sum_{\sigma_j\in S_n} (-q)^{2l(\sigma_j)}=\sum_{k=0}^{\frac{n(n+1)}{2}}I_n(k)q^{2k}.
\end{equation*}
By Andrews~\cite{andrews1998theory}, the generating function of $I_n(k)$ is
\begin{equation*}
    \sum_{k=0}^{\frac{n(n+1)}{2}}I_n(k)x^{k}=\prod_{j=1}^n\frac{1-x^j}{1-x}. 
\end{equation*}
So the denominator of Eq(\ref{eq:sys1}) can be rewritten as
\begin{equation*}
    \sum_{\sigma_j\in S_n} (-q)^{2l(\sigma_j)}=\prod_{j=1}^n\frac{1-q^{2j}}{1-q^2}=[n]_{q^2}!,
\end{equation*}
and we get:
\begin{equation*}
    h(\Pi_{k=1}^nx_{k,\tau_i(k)})=\frac{(-q)^{l(\tau_i)}}{[n]_{q^2}!}.
\end{equation*}
This finishes the proof of Theorem 1 d).

==> Chapters/Non-zero_cretirion.tex <==
\section{Characterization of monomial $\boldsymbol{x}$ such that $\boldsymbol{h(x)\ne 0}$} 
Not every monomial has a non-zero Haar state value. In this section, we will give a criterion to determine whether the Haar state of a monomial is zero.

\hfill

\noindent Let $D_n$ be the diagonal subgroup of $SL_q(n)$. Recall that the coordinate Hopf algebra $\mathcal{O}(D_n)$ is the commutative algebra $\mathbb{C}[t_1,t_1^{-1},\cdots,t_n,t_n^{-1}]$ of all Laurent polynomials in $n$ indeterminates $t_1,t_2,\dots,t_n$ with comultiplication $\Delta(t_i)=t_i\otimes t_i$ and counit $\varepsilon(t_i)=1$. The surjective homomorphism $\pi_{D_n}:\mathcal{O}(SL_q(n))\mapsto \mathcal{O}(D_n)$ is given by $\pi_{D_n}(x_{ij})=\delta_{ij}t_i$. Since we have $D_q^k=1_{\mathcal{O}(SL_q(n))}$ for all $k\in \mathbb{N}^+$, $\pi_{D_n}$ tells us $1_{\mathcal{O}(D_n)}=\pi_{D_n}(1_{\mathcal{O}(SL_q(n))})=\pi_{D_n}(D_q^k)=(\Pi_{i=1}^nt_i)^k$. 

\hfill

\noindent The left and right action of $\mathcal{O}(SL_q(n))$ on $\mathcal{O}(D_n)$, denoted as $L_{D_n}$ and $R_{D_n}$, is defined as:
\begin{equation*}
    \begin{split}
        L_{D_n}&=(\pi_{D_n}\otimes Id)\circ \Delta,\\
        R_{D_n}&=(Id\otimes \pi_{D_n})\circ \Delta.
    \end{split}
\end{equation*}
Given vector $v=(v_1,v_2,\dots,v_n)\in \mathbb{R}^n$, we write $t^v=\Pi_{i=1}^nt_i^{v_i}$. If $x$ is a monomial, we have:
\begin{equation*}
    \begin{split}
        L_{D_n}(x)&=t^{\alpha(\eta(x))}\otimes x,\\
        R_{D_n}(x)&=x\otimes t^{\beta(\eta(x))}.
    \end{split}
\end{equation*}

\hfill

\noindent The next theorem is a generalization of Klimyk and Schmudgen's observation~\cite{klimyk2012quantum}. It gives the necessary condition such that $h(x)\ne 0$ for $x\in \mathcal{O}(SL_q(n))$:

\hfill

\noindent\textbf{Theorem 1 a)}: {\it Let $x$ be a monomial. Then $h(x)\ne 0$ implies that there exist $k\in \mathbb{N}^+$ such that $\eta(x)$ is a ${k}$-doubly stochastic matrix.}
\begin{proof}
    Consider $(\pi_{D_n}\otimes h)\circ \Delta(x)$. There are two ways to compute this object:
\begin{equation*}
\begin{split}
    (\pi_{D_n}\otimes h)\circ \Delta(x)&=\pi_{D_n}\circ (Id\otimes h)\circ \Delta(x)=\pi_{D_n}(h(x)\cdot 1_{\mathcal{O}(SL_q(n))})\\
    &=h(x)\cdot 1_{\mathcal{O}(D_n)},\\
    (\pi_{D_n}\otimes h)\circ \Delta(x)&=(id \otimes h)\circ (\pi_{D_n}\otimes id)\circ \Delta(x)=(id \otimes h)\circ L_{D_n}(x)\\
    &=(id \otimes h)(t^{\alpha(\eta(x))}\otimes x)\\
    &=h(x)\cdot t^{\alpha(\eta(x))}.
\end{split}
\end{equation*}
Thus, $h(x)\cdot 1_{\mathcal{O}(D_n)}=h(x)\cdot t^{\alpha(\eta(x))}$. Since $h(x)\ne 0$, we get $1_{\mathcal{O}(D_n)}= t^{\alpha(\eta(x))}$. This means that we can find integer $k_1>0$ such that $t^{\alpha(\eta(x))}=(\Pi_{i=1}^nt_i)^{k_1}$. Thus, $\alpha(\eta(x))=(k_1)_{i=1}^n$.

\noindent Apply the same argument to $(h\otimes \pi_{D_n})\circ \Delta(x)$, we get $1_{\mathcal{O}(D_n)}= t^{\beta(\eta(x))}$. Thus, we can find $k_2>0$ such that $\beta(\eta(x))=(k_2)_{i=1}^n$. But we must have $k_1=k_2$ since
\begin{equation*}
    nk_1=\sum_{i=1}^n\sum_{j=1}^na_{ij}=nk_2.  
\end{equation*} 
\end{proof}

==> Chapters/Source_Matrix/Source_Matrix.tex <==
\section{The Source Matrix on $\mathcal{O}(SL_q(3))$}
In this section, we will construct a linear systems of order $m$ called the \textbf{Source Matrix of order} $\boldsymbol{m}$ based on the relation $((id\otimes h)\circ \Delta)(x)=h(x)\cdot 1$. We start with the motivation of our construction.\\
\\
Recall the 3 difficulties we introduced in section 6. To reduce the computation in step i), we prefer to pick a comparing basis $s_j$ such that the number of $z_i$'s in Equation (\ref{ep:4}) whose decomposition contain $s_j$ is as small as possible. To reduce the computation in step ii), we prefer to pick a equation basis $s_l$ such that in Equation (\ref{ep:4}) the decomposition of the $y_j$'s corresponding to the $z_j$'s in step i) is as simple as possible. To reduce the computation in step iii), we prefer to pick a comparing basis $s_j$ such that the number of terms in the expansion of $D_q^m$ whose decomposition contain $s_j$ is as small as possible.\\
\\
According to Theorem 1 e), the decomposition of a monomial does not contain those standard monomials whose number of generator $a$ and $k$ exceed that of the original monomial. Thus, we should pick those standard monomials containing as many generator $a$ and $k$ as possible to be the comparing basis $s_j$ so that only limited number of $z_j$'s in Equation (\ref{ep:4}) contains $s_j$. Theorem 1 e) also tells us that the decomposition of a monomial contains only those standard monomials whose number of generator $c$ and $g$ equals to or exceeds that of the original monomial. Thus, we should pick those equation basis $s_l$ such that in Equation (\ref{ep:4}) the $y_j$'s corresponding to those $z_j$'s which contains $s_j$ contain as many generator $c$ and $g$ as possible so that the decomposition of $y_j$'s contain only a limited number of standard monomials.\\
\\
Based on the analysis, we pick standard monomial $(ceg)^m$ as the equation basis and consider the linear relation derived from comparing basis $(aek)^{m-1}afh$, $(aek)^{m-1}bdk$, $(aek)^{m-2}afhbdk$, $(aek)^{m-1}bfg$, $(aek)^{m-1}cdh$, and $(aek)^{m-1}ceg$, respectively. Notice that these comparing basis contains at least $m-1$ generator $a$ and at least $m-1$ generator $k$. We exclude the comparing basis $(aek)^m$ since the corresponding linear relation is an identity. According to the order restriction, we list all the terms $z_j\otimes y_j$ in $\Delta\left((ceg)^m\right)$ whose $z_j$ contains one of our chosen comparing basis. Notice that these $z_j$'s are variations of our chosen comparing basis under the order restriction.\\
\\
Variations of $(aek)^{m-1}afh$:
\begin{enumerate}
    \item[1)] $(aek)^lafh(aek)^{m-1-l}\otimes\\(ceg)^lchd(ceg)^{m-1-l}$
    \item[2)] $(aek)^lafk(aek)^kaeh(aek)^{m-2-l-k}\otimes\\(ceg)^lchg(ceg)^{k}ced(ceg)^{m-2-l-k}$
    \item[3)] $(aek)^laeh(aek)^kafk(aek)^{m-2-l-k}\otimes\\(ceg)^lced(ceg)^{k}chg(ceg)^{m-2-l-k}$
\end{enumerate}
Variations of $(aek)^{m-1}bdk$:
\begin{enumerate}
    \item[1)] $(aek)^lbdk(aek)^{m-1-l}\otimes\\
    (ceg)^lfbg(ceg)^{m-1-l}$
    \item[2)] $(aek)^lbek(aek)^kadk(aek)^{m-2-l-k}\otimes\\(ceg)^lfeg(ceg)^kcbg(ceg)^{m-2-l-k}$
    \item[3)] $(aek)^ladk(aek)^kbek(aek)^{m-2-l-k}\otimes\\(ceg)^lcbg(ceg)^kfeg(ceg)^{m-2-l-k}$ 
\end{enumerate}
Variations of $(aek)^{m-2}afhbdk$:
\begin{enumerate}
    \item[1)] $(aek)^{i_1}b(eka)^{i_2}dk(aek)^{i_3}af(kae)^{i_4}h(aek)^{m-2-i_1-i_2-i_3-i_4}\otimes\\(ceg)^{i_1}f(egc)^{i_2}bg(ceg)^{i_3}ch(gce)^{i_4}d(ceg)^{m-2-i_1-i_2-i_3-i_4}$
    \item[2)] $(aek)^{i_1}af(kae)^{i_2}h(aek)^{i_3}b(eka)^{i_4}dk(aek)^{m-2-i_1-i_2-i_3-i_4}\otimes\\(ceg)^{i_1}ch(gce)^{i_2}d(ceg)^{i_3}f(egc)^{i_4}bg(ceg)^{m-2-i_1-i_2-i_3-i_4}$
    \item[3)] $(aek)^{i_1}be(kae)^{i_2}h(aek)^{i_3}afk(aek)^{i_4}adk(aek)^{m-3-i_1-i_2-i_3-i_4}\otimes\\(ceg)^{i_1}fe(gce)^{i_2}d(ceg)^{i_3}chg(ceg)^{i_4}cbg(ceg)^{m-3-i_1-i_2-i_3-i_4}$
    \item[4)] $(aek)^{i_1}afk(aek)^{i_2}adk(aek)^{i_3}be(kae)^{i_4}h(aek)^{m-3-i_1-i_2-i_3-i_4}\otimes\\(ceg)^{i_1}chg(ceg)^{i_2}cbg(ceg)^{i_3}fe(gce)^{i_4}d(ceg)^{m-3-i_1-i_2-i_3-i_4}$ 
    \item[5)] $(aek)^{i_1}adk(aek)^{i_2}be(kae)^{i_3}h(aek)^{i_4}afk(aek)^{m-3-i_1-i_2-i_3-i_4}\otimes\\(ceg)^{i_1}cbg(ceg)^{i_2}fe(gce)^{i_3}d(ceg)^{i_4}chg(ceg)^{m-3-i_1-i_2-i_3-i_4}$  
    \item[6)] $(aek)^{i_1}adk(aek)^{i_2}af(kae)^{i_3}h(aek)^{i_4}bek(aek)^{m-3-i_1-i_2-i_3-i_4}\otimes\\(ceg)^{i_1}cbg(ceg)^{i_2}ch(gce)^{i_3}d(ceg)^{i_4}feg(ceg)^{m-3-i_1-i_2-i_3-i_4}$ 
    \item[7)] $(aek)^{i_1}aeh(aek)^{i_2}b(eka)^{i_3}dk(aek)^{i_4}afk(aek)^{m-3-i_1-i_2-i_3-i_4}\otimes\\(ceg)^{i_1}ced(ceg)^{i_2}f(egc)^{i_3}bg(ceg)^{i_4}chg(ceg)^{m-3-i_1-i_2-i_3-i_4}$  
    \item[8)] $(aek)^{i_1}aeh(aek)^{i_2}afk(aek)^{i_3}adk(aek)^{i_4}bek(aek)^{m-4-i_1-i_2-i_3-i_4}\otimes\\(ceg)^{i_1}ced(ceg)^{i_2}chg(ceg)^{i_3}fbg(ceg)^{i_4}feg(ceg)^{m-4-i_1-i_2-i_3-i_4}$  
    \item[9)] $(aek)^{i_1}b(eka)^{i_2}fk(aek)^{i_3}ad(kae)^{i_4}h(aek)^{m-2-i_1-i_2-i_3-i_4}\otimes\\(ceg)^{i_1}f(egc)^{i_2}hg(ceg)^{i_3}cb(gce)^{i_4}d(ceg)^{m-2-i_1-i_2-i_3-i_4}$ 
    \item[10)] $(aek)^{i_1}b(eka)^{i_2}f(kae)^{i_3}h(aek)^{i_4}adk(aek)^{m-2-i_1-i_2-i_3-i_4}\otimes\\(ceg)^{i_1}f(egc)^{i_2}h(gce)^{i_3}d(ceg)^{i_4}cbg(ceg)^{m-2-i_1-i_2-i_3-i_4}$ 
    \item[11)] $(aek)^{i_1}afk(aek)^{i_2}b(eka)^{i_3}d(kae)^{i_4}h(aek)^{m-2-i_1-i_2-i_3-i_4}\otimes\\(ceg)^{i_1}chg(ceg)^{i_2}f(egc)^{i_3}b(gce)^{i_4}d(ceg)^{m-2-i_1-i_2-i_3-i_4}$ 
    \item[12)] $(aek)^{i_1}afk(aek)^{i_2}be(kae)^{i_3}h(aek)^{i_4}adk(aek)^{m-3-i_1-i_2-i_3-i_4}\otimes\\(ceg)^{i_1}chg(ceg)^{i_2}fe(gce)^{i_3}d(ceg)^{i_4}cbg(ceg)^{m-3-i_1-i_2-i_3-i_4}$ 
    \item[13)] $(aek)^{i_1}ad(kae)^{i_2}h(eka)^{i_3}b(eka)^{i_4}fk(aek)^{m-2-i_1-i_2-i_3-i_4}\otimes\\(ceg)^{i_1}cb(gce)^{i_2}d(ceg)^{i_3}f(egc)^{i_4}hg(ceg)^{m-2-i_1-i_2-i_3-i_4}$ 
    \item[14)] $(aek)^{i_1}ad(kae)^{i_2}h(aek)^{i_3}afk(aek)^{i_4}bek(aek)^{m-3-i_1-i_2-i_3-i_4}\otimes\\(ceg)^{i_1}cb(gce)^{i_2}d(ceg)^{i_3}chg(ceg)^{i_4}feg(ceg)^{m-3-i_1-i_2-i_3-i_4}$ 
    \item[15)] $(aek)^{i_1}aeh(aek)^{i_2}adk(aek)^{i_3}b(eka)^{i_4}fk(aek)^{m-3-i_1-i_2-i_3-i_4}\otimes\\(ceg)^{i_1}ced(ceg)^{i_2}cbg(ceg)^{i_3}f(egc)^{i_4}hg(ceg)^{m-3-i_1-i_2-i_3-i_4}$
    \item[16)] $(aek)^{i_1}aeh(aek)^{i_2}adk(aek)^{i_3}afk(aek)^{i_4}bek(aek)^{m-4-i_1-i_2-i_3-i_4}\otimes\\(ceg)^{i_1}ced(ceg)^{i_2}cbg(ceg)^{i_3}chg(ceg)^{i_4}feg(ceg)^{m-4-i_1-i_2-i_3-i_4}$
    \item[17)] $(aek)^{i_1}b(eka)^{i_2}d(kae)^{i_3}h(aek)^{i_4}afk(aek)^{m-2-i_1-i_2-i_3-i_4}\otimes\\(ceg)^{i_1}f(egc)^{i_2}b(gce)^{i_3}d(ceg)^{i_4}chg(ceg)^{m-2-i_1-i_2-i_3-i_4}$
    \item[18)] $(aek)^{i_1}be(kae)^{i_2}h(aek)^{i_3}adk(aek)^{i_4}afk(aek)^{m-3-i_1-i_2-i_3-i_4}\otimes\\(ceg)^{i_1}fe(gce)^{i_2}d(ceg)^{i_3}cbg(ceg)^{i_4}chg(ceg)^{m-3-i_1-i_2-i_3-i_4}$
    \item[19)] $(aek)^{i_1}afk(aek)^{i_2}ad(kae)^{i_3}h(aek)^{i_4}bek(aek)^{m-3-i_1-i_2-i_3-i_4}\otimes\\(ceg)^{i_1}chg(ceg)^{i_2}cb(gce)^{i_3}d(ceg)^{i_4}feg(ceg)^{m-3-i_1-i_2-i_3-i_4}$
    \item[20)] $(aek)^{i_1}af(kae)^{i_2}h(kae)^{i_3}adk(aek)^{i_4}bek(aek)^{m-3-i_1-i_2-i_3-i_4}\otimes\\(ceg)^{i_1}ch(gce)^{i_2}d(ceg)^{i_3}cbg(ceg)^{i_4}feg(ceg)^{m-3-i_1-i_2-i_3-i_4}$  
    \item[21)] $(aek)^{i_1}adk(aek)^{i_2}b(eka)^{i_3}f(kae)^{i_4}h(aek)^{m-2-i_1-i_2-i_3-i_4}\otimes\\(ceg)^{i_1}cbg(ceg)^{i_2}f(egc)^{i_3}h(gce)^{i_4}d(ceg)^{m-2-i_1-i_2-i_3-i_4}$ 
    \item[22)] $(aek)^{i_1}adk(aek)^{i_2}afk(aek)^{i_3}be(kae)^{i_4}h(aek)^{m-3-i_1-i_2-i_3-i_4}\otimes\\(ceg)^{i_1}cbg(ceg)^{i_2}chg(ceg)^{i_3}fe(gce)^{i_4}d(ceg)^{m-3-i_1-i_2-i_3-i_4}$ 
    \item[23)] $(aek)^{i_1}aeh(aek)^{i_2}b(eka)^{i_3}fk(aek)^{i_4}adk(aek)^{m-3-i_1-i_2-i_3-i_4}\otimes\\(ceg)^{i_1}ced(ceg)^{i_2}f(egc)^{i_3}hg(ceg)^{i_4}cbg(ceg)^{m-3-i_1-i_2-i_3-i_4}$ 
    \item[24)] $(aek)^{i_1}aeh(aek)^{i_2}afk(aek)^{i_3}b(eka)^{i_4}dk(aek)^{m-3-i_1-i_2-i_3-i_4}\otimes\\(ceg)^{i_1}ced(ceg)^{i_2}chg(ceg)^{i_3}f(egc)^{i_4}bg(ceg)^{m-3-i_1-i_2-i_3-i_4}$ 
\end{enumerate}
Variations of $(aek)^{m-1}bfg$:
\begin{enumerate}
    \item[1)] $(aek)^{i_1}b(eka)^{i_2}f(kae)^{i_3}g(aek)^{m-1-i_1-i_2-i_3}\otimes\\(ceg)^{i_1}f(egc)^{i_2}h(gce)^{i_3}a(ceg)^{m-1-i_1-i_2-i_3}$ 
    \item[2)] $(aek)^{i_1}afk(aek)^{i_2}be(kae)^{i_3}g(aek)^{m-2-i_1-i_2-i_3}\otimes\\(ceg)^{i_1}chg(ceg)^{i_2}fe(gce)^{i_3}a(ceg)^{m-2-i_1-i_2-i_3}$ 
    \item[3)] $(aek)^{i_1}be(kae)^{i_2}g(aek)^{i_3}afk(aek)^{m-2-i_1-i_2-i_3}\otimes\\(ceg)^{i_1}fe(gce)^{i_2}a(ceg)^{i_3}chg(ceg)^{m-2-i_1-i_2-i_3}$ 
    \item[4)] $(aek)^{i_1}af(kae)^{i_2}g(aek)^{i_3}bek(aek)^{m-2-i_1-i_2-i_3}\otimes\\(ceg)^{i_1}ch(gce)^{i_2}a(ceg)^{i_3}feg(ceg)^{m-2-i_1-i_2-i_3}$ 
    \item[5)] $(aek)^{i_1}aeg(aek)^{i_2}b(eka)^{i_3}fk(aek)^{m-2-i_1-i_2-i_3}\otimes\\(ceg)^{i_1}cea(ceg)^{i_2}f(egc)^{i_3}hg(ceg)^{m-2-i_1-i_2-i_3}$ 
    \item[6)] $(aek)^{i_1}aeg(aek)^{i_2}afk(aek)^{i_3}bek(aek)^{m-3-i_1-i_2-i_3}\otimes\\(ceg)^{i_1}cea(ceg)^{i_2}chg(ceg)^{i_3}feg(ceg)^{m-3-i_1-i_2-i_3}$ 
\end{enumerate}
Variations of $(aek)^{m-1}cdh$:
\begin{enumerate}
    \item[1)] $(aek)^{i_1}c(eka)^{i_2}d(kae)^{i_3}h(aek)^{m-1-i_1-i_2-i_3}\otimes\\(ceg)^{i_1}k(egc)^{i_2}b(gce)^{i_3}d(ceg)^{m-1-i_1-i_2-i_3}$ 
    \item[2)] $(aek)^{i_1}ce(kae)^{i_2}h(aek)^{i_3}adk(aek)^{m-2-i_1-i_2-i_3}\otimes\\(ceg)^{i_1}k(egc)^{i_2}ed(ceg)^{i_3}cbg(ceg)^{m-2-i_1-i_2-i_3}$ 
    \item[3)] $(aek)^{i_1}aeh(aek)^{i_2}c(eka)^{i_3}dk(aek)^{m-2-i_1-i_2-i_3}\otimes\\(ceg)^{i_1}ced(ceg)^{i_2}k(egc)^{i_3}bg(ceg)^{m-2-i_1-i_2-i_3}$ 
    \item[4)] $(aek)^{i_1}adk(aek)^{i_2}ce(kae)^{i_3}h(aek)^{m-2-i_1-i_2-i_3}\otimes\\(ceg)^{i_1}cbg(ceg)^{i_2}k(egc)^{i_3}ed(ceg)^{m-2-i_1-i_2-i_3}$ 
    \item[5)] $(aek)^{i_1}ad(kae)^{i_2}h(aek)^{i_3}cek(aek)^{m-2-i_1-i_2-i_3}\otimes\\(ceg)^{i_1}cb(gce)^{i_2}d(ceg)^{i_3}keg(ceg)^{m-2-i_1-i_2-i_3}$ 
    \item[6)] $(aek)^{i_1}aeh(aek)^{i_2}adk(aek)^{i_3}cek(aek)^{m-3-i_1-i_2-i_3}\otimes\\(ceg)^{i_1}ced(ceg)^{i_2}cbg(ceg)^{i_3}keg(ceg)^{m-3-i_1-i_2-i_3}$ 
\end{enumerate}
Variations of $(aek)^{m-1}ceg$:
\begin{enumerate}
    \item[1)] $(aek)^laeg(aek)^kcek(aek)^{m-2-l-k}\otimes\\(ceg)^lcea(ceg)^kkeg(ceg)^{m-2-l-k}$ 
    \item[2)] $(aek)^lce(kae)^kg(aek)^{m-2-l-k}\otimes\\(ceg)^lke(gce)^ka(ceg)^{m-1-l-k}$ 
\end{enumerate}
The right components corresponding to our chosen comparing basis contain at least $m-1$ generator $c$ and at least $m-1$ generator $g$. Thus, the unknowns in these linear relations are the Haar state of $aek(ceg)^{m-1}$, $afh(ceg)^{m-1}$, $bdk(ceg)^{m-1}$, $bfgcdh(ceg)^{m-2}$, $bfg(ceg)^{m-1}$, $cdh(ceg)^{m-1}$, and $(ceg)^{m}$. Now we get $6$ linear relations containing $7$ unknowns. To get a solvable linear system, we add the quantum determinant relation:
\begin{equation*}
    \begin{split}
        &h\left((ceg)^{m-1}\right)=h\left(D_q(ceg)^{m-1}\right)\\
        =&h\left(aek(ceg)^{m-1}\right)-q\cdot h\left(afh(ceg)^{m-1}\right)-q\cdot h\left(bdk(ceg)^{m-1}\right)\\
        &+q^2\cdot h\left(bfg(ceg)^{m-1}\right)+q^2\cdot h\left(cdh(ceg)^{m-1}\right)-q^3\cdot h\left(ceg(ceg)^{m-1}\right).
    \end{split}
\end{equation*}
The linear system of order $m$ consisting of the 7 equations is called the \textbf{Source Matrix of order} $\boldsymbol{m}$. Besides the quantum determinant relation, the right-hand-sides of all other linear relations are zero. Thus, the linear system is recursive. The Haar state of $(ceg)^{m-1}$ is solved from the Source Matrix of order $m-1$ and then used as the only non-zero right-hand-side term in the Source Matrix of order $m$. The general solution to the Source Matrix of order $m$ is:
\begin{equation*}
    \begin{split}
        h(aek(ceg)^{m-1})&=\frac{(-q)^{3m-2}(q^2-1)^3(q^4-1)(1+q^4-q^2-q^{2m+2})}{q(q^{2m}-1)^2(q^{2m+2}-1)^2(q^{2m+4}-1)}\\
        h(afh(ceg)^{m-1})&=\frac{(-q)^{3m-2}(q^2-1)^4(q^4-1)}{(q^{2m}-1)^2(q^{2m+2}-1)^2(q^{2m+4}-1)}\\
        h(bdk(ceg)^{m-1})&=\frac{(-q)^{3m-2}(q^2-1)^4(q^4-1)}{(q^{2m}-1)^2(q^{2m+2}-1)^2(q^{2m+4}-1)}\\
        h(bfgcdh(ceg)^{m-2})&=\frac{(-q)^{3m-2}(q^2-1)^4(q^4-1)}{(q^{2m}-1)^2(q^{2m+2}-1)^2(q^{2m+4}-1)}\\
        h(bfg(ceg)^{m-1})&=\frac{(-q)^{3m-1}(q^2-1)^3(q^4-1)}{(q^{2m}-1)(q^{2m+2}-1)^2(q^{2m+4}-1)}\\
        h(cdh(ceg)^{m-1})&=\frac{(-q)^{3m-1}(q^2-1)^3(q^4-1)}{(q^{2m}-1)(q^{2m+2}-1)^2(q^{2m+4}-1)}\\
        h((ceg)^{m})&=\frac{(-q)^{3m}(q^2-1)^2(q^4-1)}{(q^{2m+2}-1)^2(q^{2m+4}-1)}.
    \end{split}
\end{equation*}
For the entries of the Source matrix of order $m$, see Table~\ref{tab:source} on the next page.\\
\\
Through direct computation, we can verify that the Source Matrix of order $2$ and $3$ fit in the general form.  In following subsection we provide the steps to compute the contribution of tensor products in the forms of:
\begin{enumerate}
    \item[1)] $(aek)^lafh(aek)^{m-1-l}\otimes\\(ceg)^lchd(ceg)^{m-1-l}$
    \item[2)] $(aek)^lafk(aek)^kaeh(aek)^{m-2-l-k}\otimes\\(ceg)^lchg(ceg)^{k}ced(ceg)^{m-2-l-k}$
    \item[3)] $(aek)^laeh(aek)^kafk(aek)^{m-2-l-k}\otimes\\(ceg)^lced(ceg)^{k}chg(ceg)^{m-2-l-k}$
\end{enumerate}
to each linear relation in the Source Matrix. The contributions of other tensor products to the Source Matrix are computed similarly.

\begin{landscape}
%\begin{TAB}(r,0cm,0cm)[3pt]
\begin{table}[htb!]
    \centering
    \caption{The source matrix with all its entries.}
\resizebox{1.65\textheight}{!}{
\begin{tabular}{c|cccccccc}
%{c|ccccccc}
%\hline
 & $aekceg$ & $afhceg$ & $bdkceg$ & $bfgcdh$ & $bfgceg$ & $cdhceg$ & $cegceg$ & LHS \\ \hline
$D_q$ & $1$ & $-q$ & $-q$ & $0$ & $q^2$ & $q^2$ & $-q^3$ & $h((ceg)^{m-1})$ \\
 $aekceg$&$\frac{q^2(q^{2n}-1)^2}{q^{2n}(q^2-1)^2}$  & $\frac{-q(q^{2n}-1)^2}{q^{2n}(q^2-1)}$ & $\frac{q^3(1-q^{2n})^3}{q^{4n}(q^2-1)^2}$ & $\frac{(q^3-q^{2n+1})(q^{2n}-1)^3}{q^{4n}(q^2-1)^2}$ & $\frac{(q^{2n}-1)^2}{q^{2n}}$ & $\frac{n(q^{2n}-1)^2}{q^{2n}}$ & $\frac{(q^{2n}-1)((n+1)q^4-2nq^2+n)}{q^{2n+1}(q^2-1)}$ & 0 \\
 $aekbfg$& 0 & $\frac{q^2(q^{2n}-1)^3}{q^{2n}(q^2-1)^3}$ & 0 & 0 & $\frac{-q(q^{2n}-1)^2}{q^{2n}(q^2-1)}$ & $\frac{-nq(q^{2n}-1)^2}{q^{2n}(q^2-1)}$ & $\frac{(q^{2n}-1)(n-(n+1)q^2)}{q^{2n}(q^2-1)}$ & 0 \\ 
 $aekcdh$& 0 & 0 & $\frac{q^4(q^{2n}-1)^3}{q^{4n}(q^2-1)^3}$ & $\frac{(q^{2n}-1)^3(q^{2n+2}-q^4)}{q^{4n}(q^2-1)^3}$ & $\frac{-q(q^{2n}-1)^2}{q^{2n}(q^2-1)}$ & $\frac{-nq(q^{2n}-1)^2}{q^{2n}(q^2-1)}$ & $\frac{(q^{2n}-1)(n-(n+1)q^2)}{q^{2n}(q^2-1)}$ & 0 \\
 $afhbdk$& 0 & 0 & 0 & $\frac{(q^{2n}-1)^3(q^{2n+2}-q^4)}{q^{4n}(q^2-1)^4}$ & $c_1$ & $c_2$ & $c_3$ & 0 \\
 $aekbdk$& 0 & 0 & 0 & 0 & $\frac{q^2(q^{2n}-1)^2}{q^{2n}(q^2-1)^2}$ & 0 & $\frac{q(q^{2n}-1)}{q^{2n}(q^2-1)}$ & 0 \\
 $aekafh$& 0 & 0 & 0 & 0 & 0 & $\frac{q^2(q^{2n}-1)^2}{q^{2n}(q^2-1)^2}$ & $\frac{q(q^{2n}-1)}{q^{2n}(q^2-1)}$ & 0 \\ %\hline
\end{tabular}
}
\label{tab:source}
\end{table}


%\end{TAB}
\begin{equation*}
    \begin{split}
        c_1&=\frac{(q^{2n}-1)^2(q^{2n-2}+(n-1)q^{2n}-(n-1)q^{2n+2}-1)}{q^{4n-3}(q^2-1)^3}\\
        c_2&=\frac{(q^{2n}-1)^2(nq^{2n-2}-(n-1)q^{2n}-1)}{q^{4n-3}(q^2-1)^3}\\
        c_3&=\frac{(q^{2n}-1)(q^{2n+4}-n(q^4-1)q^{2n}-q^2)}{q^{4n}(q^2-1)^2}
    \end{split}
\end{equation*}
\end{landscape}


\input{Chapters/Source_Matrix/afh}
% \input{Chapters/Source_Matrix/bdk}
% \input{Chapters/Source_Matrix/afhbdk}
% \input{Chapters/Source_Matrix/bfg}
% \input{Chapters/Source_Matrix/cdh}
% \input{Chapters/Source_Matrix/ceg}

% \noindent We have finished the computation of the Source matrix of order $m$. The solution to the Source Matrix can be verified by direction computation.

% When picking the comparing basis, we want the number of left (or right) components that contains the comparing basis to be as less as possible. Theorem 1 e) tells us that the decomposition of a monomial $x$ does not contain those standard monomials whose number of generator $a$ and $k$ exceeds that of monomial $x$. Hence, we should pick those standard monomials with more numbers of generator $a$ and $k$ as comparing basis so that left (or right) components whose number of generator $a$ and $k$ does not exceed that of the comparing basis can be ignored. \\
% \\
% To construct the Source Matrix of order $m$, we will pick all standard monomials of order $m$ with at least $m-1$ generator $a$ and at least $m-1$ generator $k$ as comparing basis. We will use the relation $(id\otimes h)\circ\Delta(x)=h(x)\cdot 1$ to derive linear relations and the equation basis is always a standard monomial. Thus by the order restriction, the standard monomials we choose are: $(aek)^{m-1}afh$, $(aek)^{m-1}bdk$, $(aek)^{m-2}afhbdk$, $(aek)^{m-1}bfg$, $(aek)^{m-1}cdh$, and $(aek)^{m-1}ceg$. Here, we do not use $(aek)^m$ since the corresponding linear relation is an identity. Then only left components that are reordering of these comparing basis satisfying the order restriction (the equation basis is a standard monomial) will be considered when deriving linear relations from comultiplications.\\
% \\
% When picking the equation basis, we want the decomposition of those right components corresponding to the left components that contains our chosen comparing basis to be as simple as possible. Theorem 1 e) tells us that the decomposition of a monomial $x$ contains only those standard monomials whose number of generator $c$ and $g$ exceeds or equals to that of monomial $x$. Thus, we want those right components to contain as many generator $c$ and $g$ as possible so that standard monomials with less number of generator $c$ and $g$ will not appear in the decomposition.\\
% \\
% If we choose standard monomial $(ceg)^m$ as the equation basis, then the right components corresponding to the left components 

==> Chapters/Source_Matrix/afh.tex <==
\subsection{Linear relation derived from comparing basis $(aek)^{m-1}afh$}
\subsubsection{Left components}
\paragraph{Left component in the form of $(aek)^lafh(aek)^{m-1-l}$}\label{2.1.1}
Besides considering the coefficient of $(aek)^{m-1}afh$, the decomposition of the above Left components may contains other standard monomials with $m-1$ generator $a$ and $m-1$ generator $k$. Since there is only $m-1$ generator $k$'s in these left components, we may ignore the new monomials generated by switching $k$ with other generators.
\begin{equation*}
    \begin{split}
        &(aek)^lafh(aek)^{m-1-l}\\
        =&(aek)^{m-1}afh+(q-q^{-1})\sum_{i=1}^{m-1-l}(aek)^{l+i-1}abdk(aek)^{m-1-l-i}fh+\cdots\\
        &-(q-q^{-1})*\sum_{i=1}^{m-1-l}(aek)^la(aek)^{i-1}cdek(aek)^{m-1-l-i}h\\
        &-(q-q^{-1})*\sum_{i=1}^{m-1-l}(aek)^laf(aek)^{i-1}bgek(aek)^{m-1-l-i}
    \end{split}
\end{equation*}
Notice that every term appearing in the decomposition contains exactly $m-1$ generator $a$ and $m-1$ generator $k$ besides $(aek)^{m-1}afh$. Thus, we have:
\begin{equation*}
    \begin{split}
        &(aek)^{l+i-1}abdk(aek)^{m-1-l-i}fh\\
        =&(aek)^{m-2}afhbdk+(q^2-1)*(aek)^{m-1}bfg+(q^2-1)*(aek)^{m-1}cdh\\
        &-(q^2-1)^2/q*(aek)^{m-1}ceg\cdots,
    \end{split}
\end{equation*}
and
\begin{equation*}
    \begin{split}
        &(aek)^la(aek)^{i-1}cdek(aek)^{m-1-l-i}h\\
        =&q^2*(aek)^{m-1}cdh+\cdots,
    \end{split}
\end{equation*}
and
\begin{equation*}
    \begin{split}
        &(aek)^laf(aek)^{i-1}bgek(aek)^{m-1-l-i}\\
        =&q^2*(aek)^{m-1}bfg-(q^3-q)*(aek)^{m-1}ceg+\cdots.
    \end{split}
\end{equation*}
Together, we have:
\begin{equation*}
    \begin{split}
        &(aek)^lafh(aek)^{m-1-l}\\
        =&(aek)^{m-1}afh+(q-q^{-1})(m-1-l)*(aek)^{m-2}afhbdk\\
        &-(q-q^{-1})(m-1-l)*(aek)^{m-1}bfg-(q-q^{-1})(m-1-l)*(aek)^{m-1}cdh\\
        &+(q-q^{-1})^2(m-1-l)*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}

\paragraph{Left component in the form of $(aek)^lafk(aek)^kaeh(aek)^{m-2-l-k}$}\label{2.1.2}
Again, we may ignore the new monomials generated from switching generator $k$ with other generators. Thus, we get:
\begin{equation*}
    (aek)^lafk(aek)^kaeh(aek)^{m-2-l-k}=(aek)^laf(aek)^{k+1}h(aek)^{m-2-l-k}+\cdots
\end{equation*}
For $(aek)^laf(aek)^{k+1}h(aek)^{m-2-l-k}$, we have:
\begin{equation*}
    \begin{split}
        &(aek)^laf(aek)^{k+1}h(aek)^{m-2-l-k}\\
        =&(aek)^lafh(aek)^{m-1-l}\\
        &+(q^2-1)q(k+1)(aek)^lbfg(aek)^{m-2-l}\\
        &-(q^2-1)^2(k+1)(aek)^lceg(aek)^{m-2-l}+\cdots
    \end{split}
\end{equation*}

Then, using the result of subsection \ref{2.1.1}, we get:
\begin{equation*}
    \begin{split}
        &(aek)^lafk(aek)^kaeh(aek)^{m-2-l-k}\\
        =&(aek)^{m-1}afh+(q-q^{-1})(m-1-l)*(aek)^{m-2}afhbdk\\
        &+(q-q^{-1})\left[(k+1)q^2-(m-1-l)\right]*(aek)^{m-1}bfg\\
        &-(q-q^{-1})(m-1-l)*(aek)^{m-1}cdh\\
        &+(q-q^{-1})^2\left[(m-1-l)-(k+1)q^2\right]*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}

\paragraph{Left component in the form of $(aek)^laeh(aek)^kafk(aek)^{m-2-l-k}$ }\label{2.1.3}
Again, we may ignore the new monomials generated from switching generator $k$ with other generators. Thus, we get:
\begin{equation*}
    (aek)^laeh(aek)^kafk(aek)^{m-2-l-k}=q^2*(aek)^{l+1}h(aek)^{k}af(aek)^{m-2-l-k}+\cdots
\end{equation*}
For $(aek)^{l+1}h(aek)^{k}af(aek)^{m-2-l-k}$, we have:
\begin{equation*}
    \begin{split}
        &(aek)^{l+1}h(aek)^{k}af(aek)^{m-2-l-k}\\
        =&(aek)^{l+k+1}afh(aek)^{m-2-l-k}\\
        &-(q-q^{-1})*\sum_{i=1}^{k+1}(aek)^{k+l+1}bfg(aek)^{m-2-l-k}+\cdots\\
    \end{split}
\end{equation*}
Using the result from section \ref{2.1.1}, we get:
\begin{equation*}
    \begin{split}
        &(aek)^laeh(aek)^kafk(aek)^{m-2-l-k}\\
        =&q^2*(aek)^{l+1}h(aek)^{k}af(aek)^{m-2-l-k}+\cdots\\
        =&q^2*(aek)^{m-1}afh+q^2(q-q^{-1})(m-2-l-k)*(aek)^{m-2}afhbdk\\
        &-q^2(q-q^{-1})(m-1-l)*(aek)^{m-1}bfg\\
        &-q^2(q-q^{-1})(m-2-l-k)*(aek)^{m-1}cdh\\
        &+q^2(q-q^{-1})^2(m-2-l-k)*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\subsubsection{Right components}
\paragraph{Right component corresponding to $(aek)^lafh(aek)^{m-1-l}$}\label{2.2.1}
When the left component is $(aek)^lafh(aek)^{m-1-l}$, the corresponding right component is $(ceg)^lchd(ceg)^{m-1-l}$. We have:
\begin{equation*}
    (ceg)^lchd(ceg)^{m-1-l}=cdh(ceg)^{m-1}-(q-q^{-1})*(ceg)^m
\end{equation*}
Recall the decomposition of $(aek)^lafh(aek)^{m-1-l}$ in subsection \ref{2.1.1}. By summing over index $l$, the contribution of $(ceg)^lchd(ceg)^{m-1-l}$ to the linear relation corresponding to comparing basis $\boldsymbol{(aek)^{m-1}afh}$ is:
$$m*cdh(ceg)^{m-1}-m(q-q^{-1})*(ceg)^{m}.$$
The contribution to the linear relation corresponding to comparing basis\\ $\boldsymbol{(aek)^{m-2}afhbdk}$ is:
\begin{equation*}
    \begin{split}
        &(q-q^{-1})\sum_{l=0}^{m-1}(m-1-l)*\left[cdh(ceg)^{m-1}-(q-q^{-1})*(ceg)^m\right]\\
        =&(q-q^{-1})\frac{m(m-1)}{2}*cdh(ceg)^{m-1}-(q-q^{-1})^2\frac{m(m-1)}{2}*(ceg)^m
    \end{split}
\end{equation*}
Similarly, the contribution to the linear relations corresponding to comparing basis $\boldsymbol{(aek)^{m-1}bfg}$ and $\boldsymbol{(aek)^{m-1}cdh}$ are the same:
\begin{equation*}
    \begin{split}
        &-(q-q^{-1})\sum_{l=0}^{m-1}(m-1-l)*\left[cdh(ceg)^{m-1}-(q-q^{-1})*(ceg)^m\right]\\
        =&-(q-q^{-1})\frac{m(m-1)}{2}*cdh(ceg)^{m-1}+(q-q^{-1})^2\frac{m(m-1)}{2}*(ceg)^m
    \end{split}
\end{equation*}
The contribution to the linear relations corresponding to comparing basis\\ $\boldsymbol{(aek)^{m-1}ceg}$ is:
\begin{equation*}
    \begin{split}
        &(q-q^{-1})^2\sum_{l=0}^{m-1}(m-1-l)*\left[cdh(ceg)^{m-1}-(q-q^{-1})*(ceg)^m\right]\\
        =&(q-q^{-1})^2\frac{m(m-1)}{2}*cdh(ceg)^{m-1}-(q-q^{-1})^3\frac{m(m-1)}{2}*(ceg)^m
    \end{split}
\end{equation*}
\paragraph{Right component corresponding to $(aek)^lafk(aek)^kaeh(aek)^{m-2-l-k}$}\label{2.2.2}
When the left component is $(aek)^lafk(aek)^kaeh(aek)^{m-2-l-k}$, the corresponding right component is $(ceg)^lchg(ceg)^{k}ced(ceg)^{m-2-l-k}$. We have:
\begin{equation*}
    \begin{split}
        &(ceg)^lchg(ceg)^{k}ced(ceg)^{m-2-l-k}\\
        =&q^{-2k-2}*cdh(ceg)^{m-1}-q^{-2k-2}(q-q^{-1})*(ceg)^m
    \end{split}
\end{equation*}
Recall the decomposition of $(aek)^lafk(aek)^kaeh(aek)^{m-2-l-k}$ in subsection \ref{2.1.2}. We write $\mathcal{F}=cdh(ceg)^{m-1}-(q-q^{-1})*(ceg)^m$. By summing over index $l$ and $k$, the contribution of $(ceg)^lchg(ceg)^{k}ced(ceg)^{m-2-l-k}$ to the linear relation corresponding to comparing basis $\boldsymbol{(aek)^{m-1}afh}$ is:
\begin{equation*}
    \begin{split}
        &\sum_{l=0}^{m-2}\sum_{k=0}^{m-2-l}\left[q^{-2k-2}*cdh(ceg)^{m-1}-q^{-2k-2}(q-q^{-1})*(ceg)^m\right]\\
        =&\left[(m-1)\frac{1}{q^2-1}+\frac{q^{-2m+2}-1}{(1-q^{2})^2}\right]*\mathcal{F}
    \end{split}
\end{equation*}
The contribution to the linear relation corresponding to comparing basis\\ $\boldsymbol{(aek)^{m-2}afhbdk}$ is:
\begin{equation*}
    \begin{split}
        &\sum_{l=0}^{m-2}\sum_{k=0}^{m-2-l}(q-q^{-1})(m-1-l)q^{-2k-2}*\mathcal{F}\\
        =&\left[\frac{m(m-1)}{2q}-\frac{q^{-2}-mq^{-2m}+(m-1)q^{-2m-2}}{q(1-q^{-2})^2}\right]*\mathcal{F}\\
    \end{split}
\end{equation*}
The contribution to the linear relations corresponding to comparing basis $\boldsymbol{(aek)^{m-1}bfg}$ is:
\begin{equation*}
    \begin{split}
        &\sum_{k=0}^{m-2}\sum_{l=0}^{m-2-k}(q-q^{-1})\left[(k+1)q^2-(m-1-l)\right]q^{-2k-2}*\mathcal{F}\\
        =&\frac{(mq^5-2mq^3+mq+q^5+q^3-q)(q^{-2m}-1)}{(1-q^2)^2}*\mathcal{F}\\
        &+\frac{4mq^6-(m^2+5m)q^4+2m^2q^2-m^2+m}{2q(1-q^2)^2}*\mathcal{F}
    \end{split}
\end{equation*}
The contribution to the linear relations corresponding to comparing basis $\boldsymbol{(aek)^{m-1}cdh}$ is:
\begin{equation*}
    \begin{split}
        &-\sum_{l=0}^{m-2}\sum_{k=0}^{m-2-l}(q-q^{-1})(m-1-l)q^{-2k-2}*\mathcal{F}\\
        =&\left[\frac{q^{-2}-mq^{-2m}+(m-1)q^{-2m-2}}{q(1-q^{-2})^2}-\frac{m(m-1)}{2q}\right]*\mathcal{F}\\
    \end{split}
\end{equation*}
The contribution to the linear relations corresponding to comparing basis $\boldsymbol{(aek)^{m-1}ceg}$ is:
\begin{equation*}
    \begin{split}
        &\sum_{k=0}^{m-2}\sum_{l=0}^{m-2-k}(q-q^{-1})^2\left[(m-1-l)-(k+1)q^2\right]q^{-2k-2}*\mathcal{F}\\
        =&\frac{(2mq^6-4mq^4+2mq^2+2q^6+2q^4-2q^2)(q^{-2m}-1)}{2q^2(1-q^2)}*\mathcal{F}\\
        &+\frac{4mq^6-(m^2+5m)q^4+2m^2q^2-m^2+m}{2q^2(1-q^2)}*\mathcal{F}
    \end{split}
\end{equation*}
\paragraph{Right component corresponding to $(aek)^laeh(aek)^kafk(aek)^{m-2-l-k}$}\label{2.2.3}
When the left component is $(aek)^laeh(aek)^kafk(aek)^{m-2-l-k}$, the corresponding right component is $(ceg)^lced(ceg)^{k}chg(ceg)^{m-2-l-k}$. We have:
\begin{equation*}
    \begin{split}
        (ceg)^lced(ceg)^{k}chg(ceg)^{m-2-l-k}=q^{2k}*cdh(ceg)^{m-1}\\
    \end{split}
\end{equation*}
Recall the decomposition of $(aek)^laeh(aek)^kafk(aek)^{m-2-l-k}$ in subsection \ref{2.1.3}. By summing over index $l$ and $k$, the contribution of $(ceg)^lced(ceg)^{k}chg(ceg)^{m-2-l-k}$ to the linear relation corresponding to comparing basis $\boldsymbol{(aek)^{m-1}afh}$ is:
\begin{equation*}
    \begin{split}
        &\sum_{l=0}^{m-2}\sum_{k=0}^{m-2-l}q^{2k+2}*cdh(ceg)^{m-1}\\
        =&\left[(m-1)\frac{1}{q^{-2}-1}+\frac{q^{2m-2}-1}{(1-q^{-2})^2}\right]*cdh(ceg)^{m-1}\\
    \end{split}
\end{equation*}
The contribution to the linear relation corresponding to comparing basis\\ $\boldsymbol{(aek)^{m-2}afhbdk}$ is:
\begin{equation*}
    \begin{split}
        &\sum_{l=0}^{m-2}\sum_{k=0}^{m-2-l}(q-q^{-1})(m-2-l-k)q^{2k+2}*cdh(ceg)^{m-1}\\
        =&\left[\frac{q^{2m-3}-(m-1)q+(m-2)q^{-1}}{(1-q^{-2})^2}-\frac{(m-2)(m-1)q}{2}\right]*cdh(ceg)^{m-1}
    \end{split}
\end{equation*}
The contribution to the linear relations corresponding to comparing basis\\ $\boldsymbol{(aek)^{m-1}bfg}$ is:
\begin{equation*}
    \begin{split}
        &\sum_{l=0}^{m-2}\sum_{k=0}^{m-2-l}-(q-q^{-1})(m-1-l)q^{2k+2}*cdh(ceg)^{m-1}\\
        =&\left[\frac{m(m-1)q}{2}-\frac{q^3-mq^{2m+1}+(m-1)q^{2m+3}}{(1-q^2)^2}\right]*cdh(ceg)^{m-1}
    \end{split}
\end{equation*}
The contribution to the linear relations corresponding to comparing basis\\ $\boldsymbol{(aek)^{m-1}cdh}$ is:
\begin{equation*}
    \begin{split}
        &\sum_{l=0}^{m-2}\sum_{k=0}^{m-2-l}-(q-q^{-1})(m-2-l-k)q^{2k+2}*cdh(ceg)^{m-1}\\
        =&\left[\frac{(m-2)(m-1)q}{2}-\frac{q^{2m-3}-(m-1)q+(m-2)q^{-1}}{(1-q^{-2})^2}\right]*cdh(ceg)^{m-1}
    \end{split}
\end{equation*}
The contribution to the linear relations corresponding to comparing basis\\ $\boldsymbol{(aek)^{m-1}ceg}$ is:
\begin{equation*}
    \begin{split}
        &\sum_{l=0}^{m-2}\sum_{k=0}^{m-2-l}(q-q^{-1})^2(m-2-l-k)q^{2k+2}*cdh(ceg)^{m-1}\\
        =&\left[\frac{q^{2m-2}-(m-1)q^2+(m-2)}{(1-q^{-2})}-\frac{(m-2)(m-1)(q^2-1)}{2}\right]*cdh(ceg)^{m-1}
    \end{split}
\end{equation*}
\subsubsection{Contribution to the linear relations corresponding to different comparing basis}
\paragraph{Comparing basis $(aek)^{m-1}afh$}\label{2.3.1}
The linear relation corresponding to $(aek)^{m-1}afh$ contains standard monomial $cdh(ceg)^{m-1}$ and $(ceg)^m$. The coefficient of $cdh(ceg)^{m-1}$ is:
\begin{equation*}
    \begin{split}
        &m+\frac{m-1}{q^2-1}+\frac{q^{-2m+2}-1}{(1-q^2)^2}+\frac{m-1}{q^{-2}-1}+\frac{q^{2m-2}-1}{(1-q^{-2})^2}\\
        =&\frac{q^2(q^m-q^{-m})^2}{(1-q^2)^2}
    \end{split}
\end{equation*}
When computing the coefficient of $(ceg)^m$, we have to consider the coefficient of $(aek)^{m-1}afh$ in $D_q^m$. By Theorem 1 e), terms in $D_q^m$ whose decomposition contains  $(aek)^{m-1}afh$ has to be in the form of $(aek)^lafh(aek)^{m-l-1}$. Thus, the coefficient of $(aek)^{m-1}afh$ in $D_q^m$ is $-mq$. Then, the coefficient of $(ceg)^{m}$ is:
\begin{equation*}
    \begin{split}
        &-m(q-q^{-1})+mq-(q-q^{-1})*\left(\frac{m-1}{q^2-1}+\frac{q^{-2m+2}-1}{(1-q^2)^2}\right)\\
        =&\frac{1}{q}-\frac{q^{-2m+2}-1}{q(q^2-1)}=\frac{q(1-q^{-2m})}{(q^2-1)}
    \end{split}
\end{equation*}
\paragraph{Comparing basis $(aek)^{m-2}afhbdk$}\label{2.3.2}
The contribution to the coefficient of $cdh(ceg)^{m-1}$ in the linear relation corresponding to comparing basis $(aek)^{m-2}afhbdk$ is:
\begin{equation*}
    \begin{split}
        &(q-q^{-1})\frac{m(m-1)}{2}+\frac{m(m-1)}{2q}-\frac{q^{-2}-mq^{-2m}+(m-1)q^{-2m-2}}{q(1-q^{-2})^2}\\
        &+\frac{q^{2m-3}-(m-1)q+(m-2)q^{-1}}{(1-q^{-2})^2}-\frac{(m-2)(m-1)q}{2}\\
        =&\frac{(1-q^{2m})(mq^2-q^{2m}-m+1)}{q^{2m-1}(1-q^2)^2}
    \end{split}
\end{equation*}
The contribution to the coefficient of $(ceg)^{m}$ in the linear relation corresponding to comparing basis $(aek)^{m-2}afhbdk$ is:
\begin{equation*}
    \begin{split}
        &-(q-q^{-1})^2\frac{m(m-1)}{2}-(q-q^{-1})\frac{m(m-1)}{2q}\\
        &+(q-q^{-1})\frac{q^{-2}-mq^{-2m}+(m-1)q^{-2m-2}}{q(1-q^{-2})^2}\\
        =&-(q^2-1)\frac{m(m-1)}{2}+\frac{q^{-2}-mq^{-2m}+(m-1)q^{-2m-2}}{1-q^{-2}}\\
    \end{split}
\end{equation*}
\paragraph{Comparing basis $(aek)^{m-1}bfg$}\label{2.3.3}
The contribution to the coefficient of $cdh(ceg)^{m-1}$ in the linear relation corresponding to comparing basis $(aek)^{m-1}bfg$ is:
\begin{equation*}
    \begin{split}
        &-(q-q^{-1})\frac{m(m-1)}{2}+\frac{m(m-1)q}{2}-\frac{q^3-mq^{2m+1}+(m-1)q^{2m+3}}{(1-q^2)^2}\\
        &+\frac{(2mq^6-4mq^4+2mq^2+2q^6+2q^4-2q^2)(q^{-2m}-1)}{2q(1-q^2)^2}\\
        &+\frac{4mq^6-(m^2+5m)q^4+2m^2q^2-m^2+m}{2q(1-q^2)^2}\\
        =&\frac{2mq^5-(3m+1)q^3+mq}{(1-q^2)^2}+\frac{mq^{2m+1}-(m-1)q^{2m+3}}{(1-q^2)^2}\\
        &+\frac{(mq^5-2mq^3+mq+q^5+q^3-q)(q^{-2m}-1)}{(1-q^2)^2}\\
    \end{split}
\end{equation*}
The contribution to the coefficient of $(ceg)^{m}$ in the linear relation corresponding to comparing basis $(aek)^{m-1}bfg$ is:
\begin{equation*}
    \begin{split}
        &(q-q^{-1})^2\frac{m(m-1)}{2}-(q-q^{-1})\frac{4mq^6-(m^2+5m)q^4+2m^2q^2-m^2+m}{2q(1-q^2)^2}\\
        &-(q-q^{-1})\frac{(mq^5-2mq^3+mq+q^5+q^3-q)(q^{-2m}-1)}{(1-q^2)^2}\\
        =&\frac{(5m-m^2)q^4+(2m^2-8m)q^2+(3m-m^2)}{2(1-q^2)}\\
        &+\frac{(mq^4-2mq^2+m+q^4+q^2-1)(q^{-2m}-1)}{1-q^2}\\
    \end{split}
\end{equation*}
\paragraph{Comparing basis $(aek)^{m-1}cdh$}\label{2.3.4}
Notice that the sign of the coefficient of $(aek)^{m-1}cdh$ is always the opposite as that of $(aek)^{m-2}afhbdk$ in the decomposition of all 3 possible forms of right components. The contribution to the coefficient of $cdh(ceg)^{m-1}$ in the linear relation corresponding to comparing basis $(aek)^{m-1}cdh$ is:
\begin{equation*}
    \begin{split}
        &-(q-q^{-1})\frac{m(m-1)}{2}+\frac{q^{-2}-mq^{-2m}+(m-1)q^{-2m-2}}{q(1-q^{-2})^2}-\frac{m(m-1)}{2q}\\
        &+\frac{(m-2)(m-1)q}{2}-\frac{q^{2m-3}-(m-1)q+(m-2)q^{-1}}{(1-q^{-2})^2}\\
        =&-\frac{q^{2m-3}-mq^{-1}+(m-2)q^{-3}+mq^{-2m-1}-(m-1)q^{-2m-3}}{(1-q^{-2})^2}
    \end{split}
\end{equation*}
The contribution to the coefficient of $(ceg)^{m}$ in the linear relation corresponding to comparing basis $(aek)^{m-1}cdh$ is:
\begin{equation*}
    \begin{split}
        &(q-q^{-1})^2\frac{m(m-1)}{2}+(q-q^{-1})\frac{m(m-1)}{2q}\\
        &-(q-q^{-1})\frac{q^{-2}-mq^{-2m}+(m-1)q^{-2m-2}}{q(1-q^{-2})^2}\\
        &=(q^2-1)\frac{m(m-1)}{2}-\frac{q^{-2}-mq^{-2m}+(m-1)q^{-2m-2}}{1-q^{-2}}
    \end{split}
\end{equation*}
\paragraph{Comparing basis $(aek)^{m-1}ceg$}\label{2.3.5}
The contribution to the coefficient of $cdh(ceg)^{m-1}$ in the linear relation corresponding to comparing basis $(aek)^{m-1}ceg$ is:
\begin{equation*}
    \begin{split}
        &(q-q^{-1})^2\frac{m(m-1)}{2}+\frac{(2mq^6-4mq^4+2mq^2+2q^6+2q^4-2q^2)(q^{-2m}-1)}{2q^2(1-q^2)}\\
        &+\frac{4mq^6-(m^2+5m)q^4+2m^2q^2-m^2+m}{2q^2(1-q^2)}\\
        &+\frac{q^{2m-2}-(m-1)q^2+(m-2)}{(1-q^{-2})}-\frac{(m-2)(m-1)(q^2-1)}{2}\\
        =&\frac{(mq^4-2mq^2+m+q^4+q^2-1)(q^{-2m}-1)}{(1-q^2)}+\frac{-2mq^4+2mq^2+q^{2m}-1}{q^2-1}
    \end{split}
\end{equation*}
The contribution to the coefficient of $(ceg)^{m}$ in the linear relation corresponding to comparing basis $(aek)^{m-1}ceg$ is:
\begin{equation*}
    \begin{split}
        &-(q-q^{-1})^3\frac{m(m-1)}{2}-(q-q^{-1})\frac{4mq^6-(m^2+5m)q^4+2m^2q^2-m^2+m}{2q^2(1-q^2)}\\
        &-(q-q^{-1})\frac{(mq^4-2mq^2+m+q^4+q^2-1)(q^{-2m}-1)}{(1-q^2)}\\
        =&\frac{(3m-m^2-2)q^3}{2}+(m^2-2m-1)q+\frac{m+2-m^2}{2q}+(m+1)q^{-2m+3}\\
        &+(1-2m)q^{-2m+1}+(m-1)q^{-2m-1}
    \end{split}
\end{equation*}

==> Chapters/Source_Matrix/afhbdk.tex <==
\subsection{Linear relation derived from comparing basis $(aek)^{m-2}afhbdk$}
\subsubsection{Left components}\label{4.1}
Besides the variations of $(aek)^{m-1}afh$ and $(aek)^{m-1}bdk$, there are 24 possible forms of left components whose decomposition contains $(aek)^{m-2}afhbdk$. Notice that the decomposition of left components that are variants of $(aek)^{m-1}bfg$, $(aek)^{m-1}cdh$, or $(aek)^{m-1}ceg$ does not contain $(aek)^{m-2}afhbdk$ since every standard monomial appearing in the decomposition corresponding to these monomials must contain at least one generator $c$ and/or generator $g$. These 24 possible forms correspond to the permutation of generator $f$, $h$, $b$, and $d$:
\begin{enumerate}
    \item[1)] $(aek)^{i_1}b(eka)^{i_2}dk(aek)^{i_3}af(kae)^{i_4}h(aek)^{m-2-i_1-i_2-i_3-i_4}$
    \item[2)] $(aek)^{i_1}af(kae)^{i_2}h(aek)^{i_3}b(eka)^{i_4}dk(aek)^{m-2-i_1-i_2-i_3-i_4}$
    \item[3)] $(aek)^{i_1}be(kae)^{i_2}h(aek)^{i_3}afk(aek)^{i_4}adk(aek)^{m-3-i_1-i_2-i_3-i_4}$
    \item[4)] $(aek)^{i_1}afk(aek)^{i_2}adk(aek)^{i_3}be(kae)^{i_4}h(aek)^{m-3-i_1-i_2-i_3-i_4}$ 
    \item[5)] $(aek)^{i_1}adk(aek)^{i_2}be(kae)^{i_3}h(aek)^{i_4}afk(aek)^{m-3-i_1-i_2-i_3-i_4}$  
    \item[6)] $(aek)^{i_1}adk(aek)^{i_2}af(kae)^{i_3}h(aek)^{i_4}bek(aek)^{m-3-i_1-i_2-i_3-i_4}$ 
    \item[7)] $(aek)^{i_1}aeh(aek)^{i_2}b(eka)^{i_3}dk(aek)^{i_4}afk(aek)^{m-3-i_1-i_2-i_3-i_4}$  
    \item[8)] $(aek)^{i_1}aeh(aek)^{i_2}afk(aek)^{i_3}adk(aek)^{i_4}bek(aek)^{m-4-i_1-i_2-i_3-i_4}$  
    \item[9)] $(aek)^{i_1}b(eka)^{i_2}fk(aek)^{i_3}ad(kae)^{i_4}h(aek)^{m-2-i_1-i_2-i_3-i_4}$ 
    \item[10)] $(aek)^{i_1}b(eka)^{i_2}f(kae)^{i_3}h(aek)^{i_4}adk(aek)^{m-2-i_1-i_2-i_3-i_4}$ 
    \item[11)] $(aek)^{i_1}afk(aek)^{i_2}b(eka)^{i_3}d(kae)^{i_4}h(aek)^{m-2-i_1-i_2-i_3-i_4}$ 
    \item[12)] $(aek)^{i_1}afk(aek)^{i_2}be(kae)^{i_3}h(aek)^{i_4}adk(aek)^{m-3-i_1-i_2-i_3-i_4}$ 
    \item[13)] $(aek)^{i_1}ad(kae)^{i_2}h(eka)^{i_3}b(eka)^{i_4}fk(aek)^{m-2-i_1-i_2-i_3-i_4}$ 
    \item[14)] $(aek)^{i_1}ad(kae)^{i_2}h(aek)^{i_3}afk(aek)^{i_4}bek(aek)^{m-3-i_1-i_2-i_3-i_4}$ 
    \item[15)] $(aek)^{i_1}aeh(aek)^{i_2}adk(aek)^{i_3}b(eka)^{i_4}fk(aek)^{m-3-i_1-i_2-i_3-i_4}$
    \item[16)] $(aek)^{i_1}aeh(aek)^{i_2}adk(aek)^{i_3}afk(aek)^{i_4}bek(aek)^{m-4-i_1-i_2-i_3-i_4}$
    \item[17)] $(aek)^{i_1}b(eka)^{i_2}d(kae)^{i_3}h(aek)^{i_4}afk(aek)^{m-2-i_1-i_2-i_3-i_4}$
    \item[18)] $(aek)^{i_1}be(kae)^{i_2}h(aek)^{i_3}adk(aek)^{i_4}afk(aek)^{m-3-i_1-i_2-i_3-i_4}$
    \item[19)] $(aek)^{i_1}afk(aek)^{i_2}ad(kae)^{i_3}h(aek)^{i_4}bek(aek)^{m-3-i_1-i_2-i_3-i_4}$
    \item[20)] $(aek)^{i_1}af(kae)^{i_2}h(kae)^{i_3}adk(aek)^{i_4}bek(aek)^{m-3-i_1-i_2-i_3-i_4}$  
    \item[21)] $(aek)^{i_1}adk(aek)^{i_2}b(eka)^{i_3}f(kae)^{i_4}h(aek)^{m-2-i_1-i_2-i_3-i_4}$ 
    \item[22)] $(aek)^{i_1}adk(aek)^{i_2}afk(aek)^{i_3}be(kae)^{i_4}h(aek)^{m-3-i_1-i_2-i_3-i_4}$ 
    \item[23)] $(aek)^{i_1}aeh(aek)^{i_2}b(eka)^{i_3}fk(aek)^{i_4}adk(aek)^{m-3-i_1-i_2-i_3-i_4}$ 
    \item[24)] $(aek)^{i_1}aeh(aek)^{i_2}afk(aek)^{i_3}b(eka)^{i_4}dk(aek)^{m-3-i_1-i_2-i_3-i_4}$ 
\end{enumerate}
Each left component of the 24 cases has $m-1$ generator $a$ and $m-1$ generator $k$. Thus, we may ignore those new monomials generated by switching generator $a$ or $k$ with other generators. We list the decomposition of each case below with standard monomials containing less than $m-1$ generator $a$ and/or $k$ omitted.\\
\\
\textbf{Case 1):}\\
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}b(eka)^{i_2}dk(aek)^{i_3}af(kae)^{i_4}h(aek)^{m-2-i_1-i_2-i_3-i_4}\\
        =&(aek)^{m-2}bdkafh+\cdots\\
        =&q^{-2}*(aek)^{m-2}afhbdk+(1-q^{-2})*(aek)^{m-1}bfg+\\
        &+(1-q^{-2})*(aek)^{m-1}cdh-\frac{(1-q^2)^2}{q^3}*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 2):}\\
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}af(kae)^{i_2}h(aek)^{i_3}b(eka)^{i_4}dk(aek)^{m-2-i_1-i_2-i_3-i_4}\\
        =&(aek)^{m-2}afhbdk+\cdots
    \end{split}
\end{equation*}
\textbf{Case 3):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}be(kae)^{i_2}h(aek)^{i_3}afk(aek)^{i_4}adk(aek)^{m-3-i_1-i_2-i_3-i_4}\\
        =&(aek)^{m-3}behafkadk+\cdots\\
        =&q^2*(aek)^{m-2}afhbdk+(q^4-q^2)*(aek)^{m-1}cdh\\
        &-q(q^2-1)^2*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 4):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}afk(aek)^{i_2}adk(aek)^{i_3}be(kae)^{i_4}h(aek)^{m-3-i_1-i_2-i_3-i_4}\\
        =&q^2*(aek)^{m-2}afhbdk+(q^4-q^2)*(aek)^{m-1}bfg\\
        &-q(q^2-1)^2*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 5):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}adk(aek)^{i_2}be(kae)^{i_3}h(aek)^{i_4}afk(aek)^{m-3-i_1-i_2-i_3-i_4}\\
        =&(aek)^{m-3}adkbehafk+\cdots\\
        =&q^2*(aek)^{m-2}afhbdk+(q^4-q^2)*(aek)^{m-1}bfg\\
        &+(q^4-q^2)*(aek)^{m-1}cdh-q(q^2-1)^2*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 6):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}adk(aek)^{i_2}af(kae)^{i_3}h(aek)^{i_4}bek(aek)^{m-3-i_1-i_2-i_3-i_4}\\
        =&(aek)^{m-3}adkafhbek+\cdots\\
        =&(aek)^{m-2}afhbdk+(q^2-1)*(aek)^{m-1}bfg\\
        &-\frac{(q^2-1)^2}{q}*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 7):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}aeh(aek)^{i_2}b(eka)^{i_3}dk(aek)^{i_4}afk(aek)^{m-3-i_1-i_2-i_3-i_4}\\
        =&(aek)^{m-3}aehbdkafk+\cdots\\
        =&(aek)^{m-2}afhbdk+(q^2-1)*(aek)^{m-1}cdh\\
        &-\frac{(q^2-1)^2}{q}*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 8):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}aeh(aek)^{i_2}afk(aek)^{i_3}adk(aek)^{i_4}bek(aek)^{m-4-i_1-i_2-i_3-i_4}\\
        =&(aek)^{m-4}aehafkadkbek+\cdots\\
        =&q^4*(aek)^{m-2}afhbdk+\cdots
    \end{split}
\end{equation*}
\textbf{Case 9):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}b(eka)^{i_2}fk(aek)^{i_3}ad(kae)^{i_4}h(aek)^{m-2-i_1-i_2-i_3-i_4}\\
        =&(aek)^{m-2}bfkadh+\cdots\\
        =&\frac{1}{q}*(aek)^{m-2}afhbdk+(q-q^{-1})*(aek)^{m-1}bfg\\
        &+(q-q^{-1})*(aek)^{m-1}cdh-\frac{(1-q^2)^2}{q^2}*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 10):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}b(eka)^{i_2}f(kae)^{i_3}h(aek)^{i_4}adk(aek)^{m-2-i_1-i_2-i_3-i_4}\\
        =&(aek)^{m-2}bfhadk+\cdots\\
        =&(aek)^{m-2}afhbdk+(q^2-1)*(aek)^{m-1}cdh\\
        &-\frac{(q^2-1)^2}{q}*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 11):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}afk(aek)^{i_2}b(eka)^{i_3}d(kae)^{i_4}h(aek)^{m-2-i_1-i_2-i_3-i_4}\\
        =&(aek)^{m-2}afkbdh+\cdots\\
        =&(aek)^{m-2}afhbdk+(q^2-1)*(aek)^{m-1}bfg\\
        &-\frac{(q^2-1)^2}{q}*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 12):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}afk(aek)^{i_2}be(kae)^{i_3}h(aek)^{i_4}adk(aek)^{m-3-i_1-i_2-i_3-i_4}\\
        =&(aek)^{m-3}afkbehadk+\cdots\\
        =&q*(aek)^{m-2}afhbdk+\cdots
    \end{split}
\end{equation*}
\textbf{Case 13):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}ad(kae)^{i_2}h(eka)^{i_3}b(eka)^{i_4}fk(aek)^{m-2-i_1-i_2-i_3-i_4}\\
        =&(aek)^{m-2}adhbfk+\cdots\\
        =&q*(aek)^{m-2}afhbdk+(q^3-q)*(aek)^{m-1}bfg\\
        &+(q^3-q)*(aek)^{m-1}cdh-(q^2-1)^2*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 14):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}ad(kae)^{i_2}h(aek)^{i_3}afk(aek)^{i_4}bek(aek)^{m-3-i_1-i_2-i_3-i_4}\\
        =&(aek)^{m-3}adhafkbek+\cdots\\
        =&q^2*(aek)^{m-2}afhbdk+(q^4-q^2)*(aek)^{m-1}bfg\\
        &-q(q^2-1)^2*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 15):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}aeh(aek)^{i_2}adk(aek)^{i_3}b(eka)^{i_4}fk(aek)^{m-3-i_1-i_2-i_3-i_4}\\
        =&(aek)^{m-3}aehadkbfk+\cdots\\
        =&q^2*(aek)^{m-2}afhbdk+(q^4-q^2)*(aek)^{m-1}cdh\\
        &-q(q^2-1)^2*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 16):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}aeh(aek)^{i_2}adk(aek)^{i_3}afk(aek)^{i_4}bek(aek)^{m-4-i_1-i_2-i_3-i_4}\\
        =&(aek)^{m-4}aehadkafkbek+\cdots\\
        =&q^3*(aek)^{m-2}afhbdk+\cdots
    \end{split}
\end{equation*}
\textbf{Case 17):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}b(eka)^{i_2}d(kae)^{i_3}h(aek)^{i_4}afk(aek)^{m-2-i_1-i_2-i_3-i_4}\\
        =&(aek)^{m-2}bdhafk+\cdots\\
        =&(aek)^{m-2}afhbdk+(q^2-1)*(aek)^{m-1}bfg\\
        &+(q^2-1)*(aek)^{m-1}cdh-\frac{(q^2-1)^2}{q}*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 18):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}be(kae)^{i_2}h(aek)^{i_3}adk(aek)^{i_4}afk(aek)^{m-3-i_1-i_2-i_3-i_4}\\
        =&(aek)^{m-3}behadkafk+\cdots\\
        =&q*(aek)^{m-2}afhbdk+(q^3-q)*(aek)^{m-1}cdh\\
        &-(q^2-1)^2*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 19):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}afk(aek)^{i_2}ad(kae)^{i_3}h(aek)^{i_4}bek(aek)^{m-3-i_1-i_2-i_3-i_4}\\
        =&(aek)^{m-3}afkadhbek+\cdots\\
         =&q*(aek)^{m-2}afhbdk+(q^3-q)*(aek)^{m-1}bfg\\
        &-(q^2-1)^2*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 20):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}af(kae)^{i_2}h(kae)^{i_3}adk(aek)^{i_4}bek(aek)^{m-3-i_1-i_2-i_3-i_4}\\
        =&(aek)^{m-3}afhadkbek+\cdots\\
        =&q^2*(aek)^{m-2}afhbdk+\cdots
    \end{split}
\end{equation*}
\textbf{Case 21):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}adk(aek)^{i_2}b(eka)^{i_3}f(kae)^{i_4}h(aek)^{m-2-i_1-i_2-i_3-i_4}\\
        =&(aek)^{m-2}adkbfh+\cdots\\
        =&(aek)^{m-2}afhbdk+(q^2-1)(aek)^{m-1}bfg\\
        &+(q^2-1)*(aek)^{m-1}cdh-\frac{(q^2-1)^2}{q}*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 22):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}adk(aek)^{i_2}afk(aek)^{i_3}be(kae)^{i_4}h(aek)^{m-3-i_1-i_2-i_3-i_4}\\
        =&(aek)^{m-3}adkafkbeh+\cdots\\
        =&q*(aek)^{m-2}afhbdk+(q^3-q)*(aek)^{m-1}bfg\\
        &-(q^2-1)^2*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 23):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}aeh(aek)^{i_2}b(eka)^{i_3}fk(aek)^{i_4}adk(aek)^{m-3-i_1-i_2-i_3-i_4}\\
        =&(aek)^{m-3}aehbfkadk+\cdots\\
         =&q*(aek)^{m-2}afhbdk+(q^3-q)*(aek)^{m-1}cdh\\
        &-(q^2-1)^2*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 24):}
\begin{equation*}
\begin{split}
    &(aek)^{i_1}aeh(aek)^{i_2}afk(aek)^{i_3}b(eka)^{i_4}dk(aek)^{m-3-i_1-i_2-i_3-i_4}\\
    =&(aek)^{m-3}aehafkbdk+\cdots\\
    =&q^2*(aek)^{m-2}afhbdk+\cdots
\end{split}
\end{equation*}
\subsubsection{Right components}\label{4.2}
We list the 24 cases of right components corresponding to the 24 cases of cases of left components in the previous subsection.
\begin{enumerate}
    \item[1)] $(ceg)^{i_1}f(egc)^{i_2}bg(ceg)^{i_3}ch(gce)^{i_4}d(ceg)^{m-2-i_1-i_2-i_3-i_4}$
    \item[2)] $(ceg)^{i_1}ch(gce)^{i_2}d(ceg)^{i_3}f(egc)^{i_4}bg(ceg)^{m-2-i_1-i_2-i_3-i_4}$
    \item[3)] $(ceg)^{i_1}fe(gce)^{i_2}d(ceg)^{i_3}chg(ceg)^{i_4}cbg(ceg)^{m-3-i_1-i_2-i_3-i_4}$
    \item[4)] $(ceg)^{i_1}chg(ceg)^{i_2}cbg(ceg)^{i_3}fe(gce)^{i_4}d(ceg)^{m-3-i_1-i_2-i_3-i_4}$
    \item[5)] $(ceg)^{i_1}cbg(ceg)^{i_2}fe(gce)^{i_3}d(ceg)^{i_4}chg(ceg)^{m-3-i_1-i_2-i_3-i_4}$
    \item[6)] $(ceg)^{i_1}cbg(ceg)^{i_2}ch(gce)^{i_3}d(ceg)^{i_4}feg(ceg)^{m-3-i_1-i_2-i_3-i_4}$
    \item[7)] $(ceg)^{i_1}ced(ceg)^{i_2}f(egc)^{i_3}bg(ceg)^{i_4}chg(ceg)^{m-3-i_1-i_2-i_3-i_4}$
    \item[8)] $(ceg)^{i_1}ced(ceg)^{i_2}chg(ceg)^{i_3}fbg(ceg)^{i_4}feg(ceg)^{m-4-i_1-i_2-i_3-i_4}$
    \item[9)] $(ceg)^{i_1}f(egc)^{i_2}hg(ceg)^{i_3}cb(gce)^{i_4}d(ceg)^{m-2-i_1-i_2-i_3-i_4}$
    \item[10)] $(ceg)^{i_1}f(egc)^{i_2}h(gce)^{i_3}d(ceg)^{i_4}cbg(ceg)^{m-2-i_1-i_2-i_3-i_4}$ 
    \item[11)] $(ceg)^{i_1}chg(ceg)^{i_2}f(egc)^{i_3}b(gce)^{i_4}d(ceg)^{m-2-i_1-i_2-i_3-i_4}$
    \item[12)] $(ceg)^{i_1}chg(ceg)^{i_2}fe(gce)^{i_3}d(ceg)^{i_4}cbg(ceg)^{m-3-i_1-i_2-i_3-i_4}$
    \item[13)] $(ceg)^{i_1}cb(gce)^{i_2}d(ceg)^{i_3}f(egc)^{i_4}hg(ceg)^{m-2-i_1-i_2-i_3-i_4}$
    \item[14)] $(ceg)^{i_1}cb(gce)^{i_2}d(ceg)^{i_3}chg(ceg)^{i_4}feg(ceg)^{m-3-i_1-i_2-i_3-i_4}$
    \item[15)] $(ceg)^{i_1}ced(ceg)^{i_2}cbg(ceg)^{i_3}f(egc)^{i_4}hg(ceg)^{m-3-i_1-i_2-i_3-i_4}$
    \item[16)]$(ceg)^{i_1}ced(ceg)^{i_2}cbg(ceg)^{i_3}chg(ceg)^{i_4}feg(ceg)^{m-4-i_1-i_2-i_3-i_4}$
    \item[17)] $(ceg)^{i_1}f(egc)^{i_2}b(gce)^{i_3}d(ceg)^{i_4}chg(ceg)^{m-2-i_1-i_2-i_3-i_4}$
    \item[18)] $(ceg)^{i_1}fe(gce)^{i_2}d(ceg)^{i_3}cbg(ceg)^{i_4}chg(ceg)^{m-3-i_1-i_2-i_3-i_4}$
    \item[19)] $(ceg)^{i_1}chg(ceg)^{i_2}cb(gce)^{i_3}d(ceg)^{i_4}feg(ceg)^{m-3-i_1-i_2-i_3-i_4}$
    \item[20)] $(ceg)^{i_1}ch(gce)^{i_2}d(ceg)^{i_3}cbg(ceg)^{i_4}feg(ceg)^{m-3-i_1-i_2-i_3-i_4}$
    \item[21)] $(ceg)^{i_1}cbg(ceg)^{i_2}f(egc)^{i_3}h(gce)^{i_4}d(ceg)^{m-2-i_1-i_2-i_3-i_4}$
    \item[22)] $(ceg)^{i_1}cbg(ceg)^{i_2}chg(ceg)^{i_3}fe(gce)^{i_4}d(ceg)^{m-3-i_1-i_2-i_3-i_4}$
    \item[23)] $(ceg)^{i_1}ced(ceg)^{i_2}f(egc)^{i_3}hg(ceg)^{i_4}cbg(ceg)^{m-3-i_1-i_2-i_3-i_4}$
    \item[24)] $(ceg)^{i_1}ced(ceg)^{i_2}chg(ceg)^{i_3}f(egc)^{i_4}bg(ceg)^{m-3-i_1-i_2-i_3-i_4}$
    \end{enumerate}
    We list the decomposition of these cases in below with $i=i_1$, $j=i_1+i_2$, $k=i_1+i_2+i_3$, $l=i_1+i_2+i_3+i_4$\\
    \textbf{Case 1):}
    \begin{equation*}
        \begin{split}
            &(ceg)^{i_1}f(egc)^{i_2}bg(ceg)^{i_3}ch(gce)^{i_4}d(ceg)^{m-2-i_1-i_2-i_3-i_4}\\
            =&q^{2i-2j+2k-2l}*fbgchd(ceg)^{m-2}\\
            =&q^{2i-2j+2k-2l}*[bfgcdh(ceg)^{m-2}-(q-q^{-1})*bfg(ceg)^{m-1}\\
            &-(q-q^{-1})*cdh(ceg)^{m-1}+\frac{(q^2-1)^2}{q^2}*(ceg)^{m}]
        \end{split}
    \end{equation*}
    \textbf{Case 2):}
    \begin{equation*}
        \begin{split}
            &(ceg)^{i_1}ch(gce)^{i_2}d(ceg)^{i_3}f(egc)^{i_4}bg(ceg)^{m-2-i_1-i_2-i_3-i_4}\\
            =&q^{2i-2j+2k-2l}*chdfbg(ceg)^{m-2}\\
            =&q^{2i-2j+2k-2l}*[bfgcdh(ceg)^{m-2}-(q-q^{-1})*bfg(ceg)^{m-1}\\
            &-(q-q^{-1})*cdh(ceg)^{m-1}+\frac{(q^2-1)^2}{q^2}*(ceg)^{m}]
        \end{split}
    \end{equation*}
    \textbf{Case 3)}
    \begin{equation*}
        \begin{split}
            &(ceg)^{i_1}fe(gce)^{i_2}d(ceg)^{i_3}chg(ceg)^{i_4}cbg(ceg)^{m-3-i_1-i_2-i_3-i_4}\\
            =&q^{2i-2j+2k-2l}*fedchgcbg(ceg)^{m-3}\\
            =&q^{2i-2j+2k-2l}*\left[\frac{1}{q^4}*bfgcdh(ceg)^{m-2}+\frac{1-q^2}{q^5}*cdh(ceg)^{m-1}\right]
        \end{split}
    \end{equation*}
    \textbf{Case 4)}
    \begin{equation*}
        \begin{split}
            &(ceg)^{i_1}chg(ceg)^{i_2}cbg(ceg)^{i_3}fe(gce)^{i_4}d(ceg)^{m-3-i_1-i_2-i_3-i_4}\\
            =&q^{2i-2j+2k-2l}*chgcbgfed(ceg)^{m-3}\\
            =&q^{2i-2j+2k-2l}*\left[\frac{1}{q^4}*bfgcdh(ceg)^{m-2}+\frac{1-q^2}{q^5}*bfg(ceg)^{m-1}\right]
        \end{split}
    \end{equation*}
    \textbf{Case 5)}
    \begin{equation*}
        \begin{split}
            &(ceg)^{i_1}cbg(ceg)^{i_2}fe(gce)^{i_3}d(ceg)^{i_4}chg(ceg)^{m-3-i_1-i_2-i_3-i_4}\\
            =&q^{-2i+2j-2k+2l}*cbgfedchg(ceg)^{m-3}\\
            =&q^{-2i+2j-2k+2l}*bfgcdh(ceg)^{m-2}
        \end{split}
    \end{equation*}
    \textbf{Case 6)}
    \begin{equation*}
        \begin{split}
            &(ceg)^{i_1}cbg(ceg)^{i_2}ch(gce)^{i_3}d(ceg)^{i_4}feg(ceg)^{m-3-i_1-i_2-i_3-i_4}\\
            =&q^{-2i+2j-2k+2l}*cbgchdfeg(ceg)^{m-3}\\
            =&q^{-2i+2j-2k+2l}*[q^2*bfgcdh(ceg)^{m-2}-(q^3-q)*bfg(ceg)^{m-1}]
        \end{split}
    \end{equation*}
    \textbf{Case 7)}
    \begin{equation*}
        \begin{split}
            &(ceg)^{i_1}ced(ceg)^{i_2}f(egc)^{i_3}bg(ceg)^{i_4}chg(ceg)^{m-3-i_1-i_2-i_3-i_4}\\
            =&q^{-2i+2j-2k+2l}*cedfbgchg(ceg)^{m-3}\\
            =&q^{-2i+2j-2k+2l}*[q^2*bfgcdh(ceg)^{m-2}-(q^3-q)*cdh(ceg)^{m-1}]
        \end{split}
    \end{equation*}
    \textbf{Case 8)}
    \begin{equation*}
        \begin{split}
            &(ceg)^{i_1}ced(ceg)^{i_2}chg(ceg)^{i_3}fbg(ceg)^{i_4}feg(ceg)^{m-4-i_1-i_2-i_3-i_4}\\
            =&q^{-2i+2j-2k+2l}*[cedchgcbgfeg(ceg)^{m-4}]\\
            =&q^{-2i+2j-2k+2l}*bfgcdh(ceg)^{m-2}
        \end{split}
    \end{equation*}
    \textbf{Case 9)}
    \begin{equation*}
        \begin{split}
            &(ceg)^{i_1}f(egc)^{i_2}hg(ceg)^{i_3}cb(gce)^{i_4}d(ceg)^{m-2-i_1-i_2-i_3-i_4}\\
            =&q^{2i+2j-2k-2l}*fhgcbd(ceg)^{m-2}\\
            =&q^{2i+2j-2k-2l}*[\frac{1}{q^3}*bfgcdh(ceg)^{m-2}+\frac{1-q^2}{q^4}*bfg(ceg)^{m-1}\\
            &+\frac{1-q^2}{q^4}*cdh(ceg)^{m-1}+\frac{(1-q^2)^2}{q^5}*(ceg)^{m}]
        \end{split}
    \end{equation*}
    \textbf{Case 10)}
    \begin{equation*}
        \begin{split}
            &(ceg)^{i_1}f(egc)^{i_2}h(gce)^{i_3}d(ceg)^{i_4}cbg(ceg)^{m-2-i_1-i_2-i_3-i_4}\\
            =&q^{2i+2j-2k-2l}*fhdcbg(ceg)^{m-2}\\
            =&q^{2i+2j-2k-2l}*[\frac{1}{q^2}*bfgcdh(ceg)^{m-2}+\frac{1-q^2}{q^3}*bfg(ceg)^{m-1}\\
            &+\frac{1-q^2}{q^3}*cdh(ceg)^{m-1}+\frac{(1-q^2)^2}{q^4}*(ceg)^{m}]
        \end{split}
    \end{equation*}
    \textbf{Case 11)}
    \begin{equation*}
        \begin{split}
            &(ceg)^{i_1}chg(ceg)^{i_2}f(egc)^{i_3}b(gce)^{i_4}d(ceg)^{m-2-i_1-i_2-i_3-i_4}\\
            =&q^{2i+2j-2k-2l}*chgfbd(ceg)^{m-3}\\
            =&q^{2i+2j-2k-2l}*[\frac{1}{q^2}*bfgcdh(ceg)^{m-2}+\frac{1-q^2}{q^3}*bfg(ceg)^{m-1}\\
            &+\frac{1-q^2}{q^3}*cdh(ceg)^{m-1}+\frac{(1-q^2)^2}{q^4}*(ceg)^{m}]
        \end{split}
    \end{equation*}
    \textbf{Case 12)}
    \begin{equation*}
        \begin{split}
            &(ceg)^{i_1}chg(ceg)^{i_2}fe(gce)^{i_3}d(ceg)^{i_4}cbg(ceg)^{m-3-i_1-i_2-i_3-i_4}\\
            =&q^{2i+2j-2k-2l}*chgfedcbg(ceg)^{m-3}\\
            =&q^{2i+2j-2k-2l}*[\frac{1}{q^5}*bfgcdh(ceg)^{m-2}+\frac{1-q^2}{q^6}*bfg(ceg)^{m-1}\\
            &+\frac{1-q^2}{q^6}*cdh(ceg)^{m-1}+\frac{(1-q^2)^2}{q^7}*(ceg)^{m}]
        \end{split}
    \end{equation*}
    \textbf{Case 13)}
    \begin{equation*}
        \begin{split}
            &(ceg)^{i_1}cb(gce)^{i_2}d(ceg)^{i_3}f(egc)^{i_4}hg(ceg)^{m-2-i_1-i_2-i_3-i_4}\\
            =&q^{-2i-2j+2k+2l}*cbdfhg(ceg)^{m-2}\\
            =&q^{-2i-2j+2k+2l}*q*bfgcdh(ceg)^{m-2}
        \end{split}
    \end{equation*}
    \textbf{Case 14)}
    \begin{equation*}
        \begin{split}
            &(ceg)^{i_1}cb(gce)^{i_2}d(ceg)^{i_3}chg(ceg)^{i_4}feg(ceg)^{m-3-i_1-i_2-i_3-i_4}\\
            =&q^{-2i-2j+2k+2l}*cbdchgfeg(ceg)^{m-3}\\
            =&q^{-2i-2j+2k+2l}*q^2*bfgcdh(ceg)^{m-2}
        \end{split}
    \end{equation*}
    \textbf{Case 15)}
    \begin{equation*}
        \begin{split}
            &(ceg)^{i_1}ced(ceg)^{i_2}cbg(ceg)^{i_3}f(egc)^{i_4}hg(ceg)^{m-3-i_1-i_2-i_3-i_4}\\
            =&q^{-2i-2j+2k+2l}*cedcbgfhg(ceg)^{m-3}\\
            =&q^{-2i-2j+2k+2l}*q^2*bfgcdh(ceg)^{m-2}
        \end{split}
    \end{equation*}
    \textbf{Case 16)}
    \begin{equation*}
        \begin{split}
            &(ceg)^{i_1}ced(ceg)^{i_2}cbg(ceg)^{i_3}chg(ceg)^{i_4}feg(ceg)^{m-4-i_1-i_2-i_3-i_4}\\
            =&q^{-2i-2j+2k+2l}*cedcbgchgfeg(ceg)^{m-4}\\
            =&q^{-2i-2j+2k+2l}*q^3*bfgcdh(ceg)^{m-2}
        \end{split}
    \end{equation*}
    \textbf{Case 17)}
    \begin{equation*}
        \begin{split}
            &(ceg)^{i_1}f(egc)^{i_2}b(gce)^{i_3}d(ceg)^{i_4}chg(ceg)^{m-2-i_1-i_2-i_3-i_4}\\
            =&q^{2i-2j-2k+2l}*fbdchg(ceg)^{m-2}\\
            =&q^{2i-2j-2k+2l}*[bfgcdh(ceg)^{m-2}-(q-q^{-1})*cdh(ceg)^{m-1}]
        \end{split}
    \end{equation*}
    \textbf{Case 18)}
    \begin{equation*}
        \begin{split}
            &(ceg)^{i_1}fe(gce)^{i_2}d(ceg)^{i_3}cbg(ceg)^{i_4}chg(ceg)^{m-3-i_1-i_2-i_3-i_4}\\
            =&q^{2i-2j-2k+2l}*fedcbgchg(ceg)^{m-3}\\
            =&q^{2i-2j-2k+2l}*[q^{-1}bfgcdh(ceg)^{m-2}-(1-q^{-2})*cdh(ceg)^{m-1}]
        \end{split}
    \end{equation*}
    \textbf{Case 19)}
    \begin{equation*}
        \begin{split}
            &(ceg)^{i_1}chg(ceg)^{i_2}cb(gce)^{i_3}d(ceg)^{i_4}feg(ceg)^{m-3-i_1-i_2-i_3-i_4}\\
            =&q^{2i-2j-2k+2l}*chgcbdfeg(ceg)^{m-3}\\
            =&q^{2i-2j-2k+2l}*[q^{-1}bfgcdh(ceg)^{m-2}-(1-q^{-2})*bfg(ceg)^{m-1}]
        \end{split}
    \end{equation*}
    \textbf{Case 20)}
    \begin{equation*}
        \begin{split}
            &(ceg)^{i_1}ch(gce)^{i_2}d(ceg)^{i_3}cbg(ceg)^{i_4}feg(ceg)^{m-3-i_1-i_2-i_3-i_4}\\
            =&q^{2i-2j-2k+2l}*chdcbgfeg(ceg)^{m-3}\\
            =&q^{2i-2j-2k+2l}*[bfgcdh(ceg)^{m-2}-(q-q^{-1})*bfg(ceg)^{m-1}]
        \end{split}
    \end{equation*}
    \textbf{Case 21)}
    \begin{equation*}
        \begin{split}
            &(ceg)^{i_1}cbg(ceg)^{i_2}f(egc)^{i_3}h(gce)^{i_4}d(ceg)^{m-2-i_1-i_2-i_3-i_4}\\
            =&q^{-2i+2j+2k-2l}*cbgfhd(ceg)^{m-2}\\
            =&q^{-2i+2j+2k-2l}*[bfgcdh(ceg)^{m-2}-(q-q^{-1})*bfg(ceg)^{m-1}]
        \end{split}
    \end{equation*}
    \textbf{Case 22)}
    \begin{equation*}
        \begin{split}
            &(ceg)^{i_1}cbg(ceg)^{i_2}chg(ceg)^{i_3}fe(gce)^{i_4}d(ceg)^{m-3-i_1-i_2-i_3-i_4}\\
            =&q^{-2i+2j+2k-2l}*cbgchgfed(ceg)^{m-3}\\
            =&q^{-2i+2j+2k-2l}*[q^{-1}*bfgcdh(ceg)^{m-2}-(1-q^{-2})*bfg(ceg)^{m-1}]
        \end{split}
    \end{equation*}
    \textbf{Case 23)}
    \begin{equation*}
        \begin{split}
            &(ceg)^{i_1}ced(ceg)^{i_2}f(egc)^{i_3}hg(ceg)^{i_4}cbg(ceg)^{m-3-i_1-i_2-i_3-i_4}\\
            =&q^{-2i+2j+2k-2l}*cedfhgcbg(ceg)^{m-3}\\
            =&q^{-2i+2j+2k-2l}*[q^{-1}*bfgcdh(ceg)^{m-2}-(1-q^{-2})cdh(ceg)^{m-1}]
        \end{split}
    \end{equation*}
    \textbf{Case 24)}
    \begin{equation*}
        \begin{split}
            &(ceg)^{i_1}ced(ceg)^{i_2}chg(ceg)^{i_3}f(egc)^{i_4}bg(ceg)^{m-3-i_1-i_2-i_3-i_4}\\
            =&q^{-2i+2j+2k-2l}*cedchgfbg(ceg)^{m-3}\\
            =&q^{-2i+2j+2k-2l}*[bfgcdh(ceg)^{m-2}-(q-q^{-1})cdh(ceg)^{m-1}]
        \end{split}
    \end{equation*}

\subsubsection{Contribution to the linear relation corresponding to different comparing basis}
First, we introduce the following notation:
\begin{equation*}
    \begin{split}
        f_1(q,m)=&\sum_{i=0}^{m-2}\sum_{j=i}^{m-2}\sum_{k=j}^{m-2}\sum_{l=k}^{m-2} q^{2i_1-2i_2+2i_3-2i_4}\\
        =&\frac{(m-1)q^{-2m-4}-(m+2)q^{-2m-2}}{(1-q^{-2})^4}\\
    &+\frac{\frac{(m+1)(m+2)}{2}q^{-4}-(m+2)(m-1)q^{-2}+\frac{m(m-1)}{2}}{(1-q^{-2})^4}
    \end{split}
\end{equation*}
\begin{equation*}
    \begin{split}
        f_2(q,m)=&\sum_{i=0}^{m-2}\sum_{j=i}^{m-2}\sum_{k=j}^{m-2}\sum_{l=k}^{m-2} q^{2i_1+2i_2-2i_3-2i_4}\\
        =&\frac{m-1}{(1-q^{-2})^3(1+q^{-2})}+\frac{q^{-4m-4}-q^{-8}}{(1-q^{-2})^4(1+q^{-2})^2}\\
        &+\frac{(m+1)q^{-2m}-mq^{-2m-2}-2q^{-2}+q^{-4}}{(1-q^{-2})^4}\\
    \end{split}
\end{equation*}
\begin{equation*}
    \begin{split}
        f_3(q,m)=&\sum_{i=0}^{m-2}\sum_{j=i}^{m-2}\sum_{k=j}^{m-2}\sum_{l=k}^{m-2} q^{2i_1-2i_2-2i_3+2i_4}\\
         =&\frac{q^{2m-4}+q^{-2m-2}}{(1-q^{-2})^4(1+q^{-2})}-\frac{q^{-2m-2}-q^{-4}}{(1-q^{-2})^3}\\
         &-\frac{(m-1)(m+2)q^{-2}}{2(1-q^{-2})^2}-\frac{q^{-2}}{(1-q^{-2})^4}\\
    \end{split}
\end{equation*}
\paragraph{Comparing basis $(aek)^{m-2}afhbdk$}\label{4.3.1}
Using the results from subsection \ref{4.1} and \ref{4.2}, \textbf{the coefficient of} \\$\boldsymbol{bfgcdh(ceg)^{m-2}}$ is:
\begin{equation*}
    \begin{split}
        &(1+q^{-2})\cdot f_1(q,m)+2q^{-2}\cdot f_1(q,m-1)+3q^2\cdot f_1(q^{-1},m-1)\\
        &+q^4\cdot f_1(q^{-1},m-2)+\\
        &(q^{-4}+2q^{-2})\cdot f_2(q,m)+q^{-4}\cdot f_2(q,m-1)+q^2\cdot f_2(q^{-1},m)\\
        &+2q^4\cdot f_2(q^{-1},m-1)+q^6\cdot f_2(q^{-1},m-2)+\\
        &f_3(q,m)+(2+q^2)\cdot f_3(q,m-1)+f_3(q^{-1},m)+(2+q^2)\cdot f_3(q^{-1},m-1)\\
        =&\frac{(q^{2m-2}-1)(q^{2m}-1)^3}{q^{4m-4}(q^2-1)^4}
    \end{split}
\end{equation*}
The coefficient of $bfg(ceg)^{m-1}$ consist of two parts: contribution from comparing basis $(aek)^{m-1}bdk$ and from comparing basis $(aek)^{m-2}afhbdk$. The contribution from $(aek)^{m-1}bdk$ has been computed in \ref{3.3.2}. Here we compute the contribution from comparing basis $(aek)^{m-2}afhbdk$:
\begin{equation*}
    \begin{split}
        &(-q+q^{-3})f_1(q,n)+\frac{1-q^2}{q^3}f_1(q,n-1)+(-q^3+q)f_1(q^{-1},n-1)\\
        &+(q^{-2}+2)\frac{1-q^2}{q^3}f_2(q,n)+\frac{1-q^2}{q^5}f_2(q,n-1)\\
        &+(q^{-1}-q^3)f_3(q,n-1)+(-q+1/q)f_3(q^{-1},n)\\
        &+(-q+q^{-1})f_3(q^{-1},n-1)\\
        =&\frac{(q^2-q^{2m})(q^{2m}-1)(1+mq^{2m+2}-(m+1)q^{2m})}{q^{4m-1}(q^2-1)^3}
    \end{split}
\end{equation*}
Together, \textbf{the coefficient of} $\boldsymbol{bfg(ceg)^{m-1}}$ is:
\begin{equation*}
    \begin{split}
        &\frac{(q^2-q^{2m})(q^{2m}-1)(1+mq^{2m+2}-(m+1)q^{2m})}{q^{4m-1}(q^2-1)^3}\\
        &+\frac{(m-2)q^3-mq}{(1-q^{2})^2}+\frac{q^{-2m+3}+mq^{2m+1}-(m-1)q^{2m+3}}{(1-q^{2})^2}\\
        =&\frac{(q^{2m}-1)^2}{q^{4m-3}(q^2-1)}\left(q^{2m-2}-\frac{1+mq^{2m+2}-(m+1)q^{2m})}{(q^2-1)^2}\right)
    \end{split}
\end{equation*}
The coefficient of $cdh(ceg)^{m-1}$ consist of two parts: contribution from comparing basis $(aek)^{m-1}afh$ and from comparing basis $(aek)^{m-2}afhbdk$. The contribution from $(aek)^{m-1}afh$ has been computed in \ref{2.3.2}. Here we compute the contribution from comparing basis $(aek)^{m-2}afhbdk$:
\begin{equation*}
    \begin{split}
        &(q^{-3}-q)\cdot f_1(q,m)+\frac{1-q^2}{q^3}\cdot f_1(q,m-1)+(-q^3+q)\cdot f_1(q^{-1},m-1)+\\
        &(\frac{1-q^2}{q^5}+2\frac{1-q^2}{q^3})\cdot f_2(q,m)+\frac{1-q^2}{q^5}\cdot f_2(q,m-1)+\\
        &(-q+1/q)\cdot f_3(q,m)+(-q+q^{-1})\cdot f_3(q,m-1)\\
        &+(q^{-1}-q^3)\cdot f_3(q^{-1},m-1)\\
        &=\frac{-q^{-4m-3}-mq^{2m-3}+(m+1)q^{2m-5}-mq^{-2m-1}}{(1-q^{-2})^3}\\
        &+\frac{(m+2)q^{-2m-3}+q^{-2m-5}+mq^{-1}-q^{-3}-(m+2)q^{-5}}{(1-q^{-2})^3}\\
    \end{split}
\end{equation*}
Together, \textbf{the coefficient of} $\boldsymbol{cdh(ceg)^{m-1}}$ is:
\begin{equation*}
    \begin{split}
        &\frac{-q^{-4m-3}-mq^{2m-3}+(m+1)q^{2m-5}-mq^{-2m-1}}{(1-q^{-2})^3}\\
        &+\frac{(m+2)q^{-2m-3}+q^{-2m-5}+mq^{-1}-q^{-3}-(m+2)q^{-5}}{(1-q^{-2})^3}\\
        &+\frac{(1-q^{2m})(mq^2-q^{2m}-m+1)}{q^{2m-1}(1-q^2)^2}\\
        =&\frac{(1-mq^{2m-2}+(m-1)q^{2m})(q^{2m}-1)^2}{q^{4m-3}(1-q^2)^3}
    \end{split}
\end{equation*}
The coefficient of $(ceg)^{m}$ consist of four parts: contribution from comparing basis $(aek)^{m-1}afh$, $(aek)^{m-1}bdk$, $(aek)^{m-2}afhbdk$, and contribution from the quantum determinant. The contribution from $(aek)^{m-1}afh$ and $(aek)^{m-1}bdk$ has been computed in \ref{2.3.2} and \ref{3.3.2}, respectively. The contribution from comparing basis $(aek)^{m-2}afhbdk$:
\begin{equation*}
    \begin{split}
        &\frac{(q^2-1)^2(1+q^{-2})}{q^2}f_1(q,n)\\
        &+\frac{(1+2q^2)(q^2-1)^2}{q^6}f_2(q,n)+\frac{(q^2-1)^2}{q^6}f_2(q,n-1)\\
        =&\frac{q^{-4n-2}-q^{-2n-4}-(2n+1)q^{-2n-2}+2nq^{-2n}}{(1-q^{-2})^2}\\
        &+\frac{(n^2-n)q^2-(n^2-n)-(n^2+3n)q^{-2}+(n^2+3n+2)q^{-4}}{2(1-q^{-2})^2}
    \end{split}
\end{equation*}
To compute the contribution from the quantum determinant, we consider terms in the form of $(aek)^lafh(aek)^{m-1-l}$, $(aek)^lbdk(aek)^{m-1-l}$, \\$(aek)^lafh(aek)^kbdk(aek)^{m-2-l-k}$, and $(aek)^lbdk(aek)^kafh(aek)^{m-2-l-k}$ in the expansion of $D_q^m$.\\
\\
The decomposition of $(aek)^lafh(aek)^{m-1-l}$ and $(aek)^lbdk(aek)^{m-1-l}$ are computed in subsection \ref{2.1.1} and \ref{3.1.1}, respectively. Notice that the contribution of $(aek)^lafh(aek)^{m-1-l}$ cancels with that of $(aek)^lbdk(aek)^{m-1-l}$.\\
\\
There are $n(n-1)/2$ terms of form $(aek)^{l}afh(aek)^{k}bdk(aek)^{m-2-l-k}$ and $n(n-1)/2$ terms of form 
 $(aek)^{l}bdk(aek)^{k}afh(aek)^{m-2-l-k}$. Notice that 
\begin{equation*}
    \begin{split}
        &(aek)^{l}bdk(aek)^{k}afh(aek)^{m-2-l-k}\\
        =&(aek)^{m-2}bdkafh+\cdots\\
        =&q^{-2}*(aek)^{m-2}afhbdk+(1-q^{-2})*(aek)^{m-1}bfg\\
        &+(1-q^{-2})*(aek)^{m-1}cdh-\frac{(1-q^2)^2}{q^3}*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
Therefore, the coefficient of $(aek)^{m-2}afhbdk$ in $D_q^m$ is $\frac{n(n-1)}{2}(1+q^{-2})q^2$ and the contribution from the quantum determinant is $-\frac{n(n-1)}{2}(1+q^{2})$.\\
\\
Together, \textbf{the coefficient of} $\boldsymbol{(ceg)^{m}}$ is:
\begin{equation*}
    \begin{split}
        &-\frac{n(n-1)}{2}(1+q^{2})-(q^2-1)\frac{m(m-1)}{2}+\frac{q^{-2}-mq^{-2m}+(m-1)q^{-2m-2}}{1-q^{-2}}\\
        &+\frac{-2q^{-2m+2}+(m^2-m)q^4+(2-2m^2)q^2+m^2+m}{2(q^2-1)}\\
        &+\frac{q^{-4n-2}-q^{-2n-4}-(2n+1)q^{-2n-2}+2nq^{-2n}}{(1-q^{-2})^2}\\
        &+\frac{(n^2-n)q^2-(n^2-n)-(n^2+3n)q^{-2}+(n^2+3n+2)q^{-4}}{2(1-q^{-2})^2}\\
        &=-(nq^{2n-2}+nq^{2n}-\frac{(q^{2n+2}-1)}{q^{2}-1})\cdot\frac{(q^{2n}-1)}{q^{4n-2}(q^{2}-1)}\\
    \end{split}
\end{equation*}
\paragraph{Comparing basis $(aek)^{m-1}bfg$}\label{4.3.2}
$(aek)^{m-1}bfg$ appears in the decomposition of case 1), 4), 5), 6), 9), 11), 13), 14), 17), 19), 21), and 22).\\
\\
The contribution to the coefficient of $bfgcdh(ceg)^{m-2}$ in the linear relation corresponding to comparing basis $(aek)^{m-1}bfg$ is:
\begin{equation*}
    \begin{split}
        &(1-q^{-2})f_1(q,m)+(1-q^{-2})f_1(q,m-1)+2(q^4-q^2)f_1(q^{-1},m-1)\\
        &+(1-q^{-4})f_2(q,m)+(q^4-q^2)f_2(q^{-1},m)+(q^6-q^4)f_2(q^{-1},m-1)\\
        &+(q^2-1)f_3(q,m)+(q^2-1)f_3(q,m-1)+(q^2-1)f_3(q^{-1},m)\\
        &+(q^2-1)f_3(q^{-1},m-1)\\
        &=\frac{q^{-4n-4}+q^{4n-4}+2(q^{-2}+q^{-4}+q^{-6})}{(1-q^{-2})^3(1+q^{-2})}-\frac{q^{-2n-4}+q^{-2n-2}+q^{2n-2}+q^{2n-4}}{(1-q^{-2})^3}
    \end{split}
\end{equation*}
The contribution to the coefficient of $bfg(ceg)^{m-1}$ in the linear relation corresponding to comparing basis $(aek)^{m-1}bfg$ is:
\begin{equation*}
    \begin{split}
        &(1-q^{-2})(-q+1/q)f_1(q,m)+\frac{1-q^2}{q^5}(q^4-q^2)f_1(q,m-1)\\
        &+(-q^3+q)(q^2-1)f_1(q^{-1},m-1)\\
        &+(\frac{1-q^2}{q^4}(q-1/q)+\frac{1-q^2}{q^3}(q^2-1))f_2(q,m)\\
        &+(-1+q^{-2})(q^3-q)f_3(q,m-1)+(-q+1/q)(q^2-1)f_3(q^{-1},m)\\
        &+(-1+q^{-2})(q^3-q)f_3(q^{-1},m-1)\\
        =&\frac{-q^{-4m-3}-q^{-2m-1}+q^{2m-5}}{(1-q^{-2})^2(1+q^{-2})}+\frac{(m-2)q^{-1}-3q^{-3}-(m+2)q^{-5}}{(1-q^{-2})^2(1+q^{-2})}\\
        &+\frac{q^{-2m-3}+2q^{-2m-1}+mq^{2m-3}-(m-1)q^{2m-1}}{(1-q^{-2})^2}\\
    \end{split}
\end{equation*}
The contribution to the coefficient of $cdh(ceg)^{m-1}$ in the linear relation corresponding to comparing basis $(aek)^{m-1}bfg$ is:
\begin{equation*}
    \begin{split}
        &-q(1-q^{-2})^2f_1(q,m)-\frac{(q^2-1)^2(1+q^2)}{q^5}f_2(q,m)-q^3(1-q^{-2})^2f_3(q,m)\\
        &=\frac{-q^{-4m-3}-q^{2m-1}-q^{-2m+1}}{(1-q^{-2})^2(1+q^{-2})}-\frac{mq^{-2m+1}}{1-q^{-2}}+\frac{q^{-2m-3}}{(1-q^{-2})^2}\\
        &+\frac{q+(m+1)q^{-1}-(m+1)q^{-5}}{(1-q^{-2})^2(1+q^{-2})}
    \end{split}
\end{equation*}
The contribution to the coefficient of $(ceg)^{m}$ in the linear relation corresponding to comparing basis $(aek)^{m-1}bfg$ is:
\begin{equation*}
    \begin{split}
        &\frac{(q^2-1)^2}{q^2}(1-q^{-2})f_1(q,m)+\left(\frac{(q^2-1)^2}{q^5}(q-q^{-1})+\frac{(q^2-1)^2}{q^4}(q^2-1)\right)f_2(q,m)\\
        &=\frac{q^{-4m-2}}{(1-q^{-2})(1+q^{-2})}+\frac{(m+1)q^{-2m+2}-(m+1)q^{-2m}-q^{-2m-2}}{(1-q^{-2})}\\
        &+\frac{(m^2+m-2)q^2-(m^2-3m)-(m^2+m-2)q^{-2}+(m^2+3m+2)q^{-4}}{2(1-q^{-2})(1+q^{-2})}
    \end{split}
\end{equation*}
\paragraph{Comparing basis $(aek)^{m-1}cdh$}\label{4.3.3}
$(aek)^{m-1}cdh$ appears in the decomposition of case 1), 3), 5), 7), 9), 10), 13), 15), 17), 18), 21), and 23).\\
\\
The contribution to the coefficient of $bfgcdh(ceg)^{m-2}$ in the linear relation corresponding to comparing basis $(aek)^{m-1}cdh$ is:
\begin{equation*}
    \begin{split}
        &(1-q^{-2})f_1(q,m)+(1-q^{-2})f_1(q,m-1)+2(q^4-q^2)f_1(q^{-1},m-1)\\
        &+(1-q^{-4})f_2(q,m)+(q^4-q^2)f_2(q^{-1},m)+(q^6-q^4)f_2(q^{-1},m-1)\\
        &+(q^2-1)f_3(q,m)+(q^2-1)f_3(q,m-1)+(q^2-1)f_3(q^{-1},m)\\
        &+(q^2-1)f_3(q^{-1},m-1)\\
        &=\frac{q^{-4m-4}+q^{4m-4}+2(q^{-2}+q^{-4}+q^{-6})}{(1-q^{-2})^3(1+q^{-2})}-\frac{q^{-2m-4}+q^{-2m-2}+q^{2m-2}+q^{2m-4}}{(1-q^{-2})^3}
    \end{split}
\end{equation*}
The contribution to the coefficient of $bfg(ceg)^{m-1}$ in the linear relation corresponding to comparing basis $(aek)^{m-1}cdh$ is:
\begin{equation*}
    \begin{split}
        &(-q+1/q)(1-q^{-2})\cdot f_1(q,m)+(\frac{1-q^2}{q^4}(q-1/q)+\frac{1-q^2}{q^3}(q^2-1))\cdot f_2(q,m)\\
        &+(-q+1/q)(q^2-1)\cdot f_3(q^{-1},m)\\
        &=\frac{-q^{-4m-3}-q^{-2m-3}-q^{2m-5}}{(1-q^{-2})^2(1+q^{-2})}+\frac{q+(m+1)q^{-1}-(m+1)q^{-5}}{(1-q^{-2})^2(1+q^{-2})}\\
        &+\frac{q^{-2m-3}+(m+1)q^{-2m-1}-(m+1)q^{-2m+1}-q^{2m-1}+q^{2m-3}}{(1-q^{-2})^2}
    \end{split}
\end{equation*}
The contribution to the coefficient of $cdh(ceg)^{m-1}$ in the linear relation corresponding to comparing basis $(aek)^{m-1}cdh$ is:
\begin{equation*}
    \begin{split}
        &-(q-q^{-1})(1-q^{-2})f_1(q,m)+\frac{1-q^2}{q^5}(q^4-q^2)f_1(q,m-1)\\
        &+(-q^3+q)(q^2-1)f_1(q^{-1},m-1)+(\frac{1-q^2}{q^4}(q-q^{-1})-\frac{(q^2-1)^2}{q^3})f_2(q,m)\\
        &-(q-q^{-1})(q^2-1)f_3(q,m)-(1-q^{-2})(q^3-q)f_3(q,m-1)\\
        &-(1-q^{-2})(q^3-q)f_3(q^{-1},m-1)\\
        =&\frac{-q^{-4m-3}-q^{-2m-1}+q^{2m-5}}{(1-q^{-2})^2(1+q^{-2})}+\frac{(m-2)q^{-1}-3q^{-3}-(m+2)q^{-5}}{(1-q^{-2})^2(1+q^{-2})}\\
        &+\frac{q^{-2m-3}+2q^{-2m-1}+mq^{2m-3}-(m-1)q^{2m-1}}{(1-q^{-2})^2}
    \end{split}
\end{equation*}
The contribution to the coefficient of $(ceg)^{m}$ in the linear relation corresponding to comparing basis $(aek)^{m-1}cdh$ is:
\begin{equation*}
    \begin{split}
        &\frac{(q^2-1)^2}{q^2}(1-q^{-2})f_1(q,m)+(\frac{(q^2-1)^2}{q^5}(q-1/q)+\frac{(q^2-1)^2}{q^4}(q^2-1))f_2(q,m)\\
        &=\frac{q^{-4m-2}}{(1-q^{-2})(1+q^{-2})}+\frac{-q^{-2m-2}-(m+1)q^{-2m}+(m+1)q^{-2m+2}}{(1-q^{-2})}\\
        &+\frac{(m^2+m-2)q^2-(m^2+3m)-(m^2+m-2)q^{-2}+(m^2+3m+2)q^{-4}}{2(1-q^{-2})(1+q^{-2})}
    \end{split}
\end{equation*}
\paragraph{Comparing basis $(aek)^{m-1}ceg$}\label{4.3.4}
$(aek)^{m-1}ceg$ appears in the decomposition of case 1), 3), 4), 5), 6), 7), 9), 10), 11), 13), 14), 15), 17), 18), 19), 21), 22), and 23).\\
\\
The contribution to the coefficient of $bfgcdh(ceg)^{m-2}$ in the linear relation corresponding to comparing basis $(aek)^{m-1}ceg$ is:
\begin{equation*}
    \begin{split}
        &-\frac{(q^2-1)^2}{q^3}f_1(q,m)-2\frac{(q^2-1)^2}{q^3}f_1(q,m-1)-3q(q^2-1)^2f_1(q^{-1},m-1)\\
        &-\left(\frac{(q^2-1)^2}{q^5}+2\frac{(q^2-1)^2}{q^3}\right)f_2(q,m)-q(q^2-1)^2f_2(q^{-1},m)\\
        &-2q^3(q^2-1)^2f_2(q^{-1},m-1)-\frac{(q^2-1)^2}{q}f_3(q,m)-2\frac{(q^2-1)^2}{q}f_3(q,m-1)\\
        &-\frac{(q^2-1)^2}{q}f_3(q^{-1},m)-2\frac{(q^2-1)^2}{q}f_3(q^{-1},m-1)\\
        =&\frac{-mq^9+(m-3)q^7+(m-6)q^5-(m+6)q^3-3q}{(q^4-1)^2}\\
        &+\frac{2q^{2m+7}+4q^{2m+5}+4q^{2m+3}+2q^{2m+1}}{(q^4-1)^2}\\
        &+\frac{q^{-2m+7}+5q^{-2m+5}+5q^{-2m+3}+q^{-2m+1}}{(q^4-1)^2}\\
        &+\frac{-q^{4m+5}-2q^{-4m+5}-2q^{4m+3}-q^{-4m+3}}{(q^4-1)^2}
    \end{split}
\end{equation*}
The contribution to the coefficient of $bfg(ceg)^{m-1}$ in the linear relation corresponding to comparing basis $(aek)^{m-1}ceg$ is:
\begin{equation*}
    \begin{split}
        &(q-1/q)\frac{(q^2-1)^2}{q^3}f_1(q,m)+\frac{(q^2-1)^3}{q^4}f_1(q,m-1)+(q^2-1)^3f_1(q^{-1},m-1)\\
        &+\left(\frac{(q^2-1)^3}{q^6}+2\frac{(q^2-1)^3}{q^4}\right)f_2(q,m)\\
        &+(q^2-1)^2(1-q^{-2})f_3(q,m-1)+(q^2-1)^2(1-q^{-2})f_3(q^{-1},m)\\
        &+(q^2-1)^2(1-q^{-2})f_3(q^{-1},m-1)\\
        &=\frac{q^{-4m-4}+2q^{-4m-2}}{(1-q^{-2})(1+q^{-2})^2}+\frac{2q^{2m-2}+q^{2m}+q^{-2m-2}+2q^{-2m}}{(1-q^{-2})(1+q^{-2})}\\
        &+\frac{-3q^{2m-2}-3q^{-2m-2}}{1-q^{-2}}+(m-2)q^{2m}-2q^{-2m}+(m+1)q^{-2m+2}\\
        &+\frac{(m-1)q^2-m-(2m-3)q^{-2}+(m+5)q^{-4}+(m+2)q^{-6}}{(1-q^{-2})(1+q^{-2})^2}\\
    \end{split}
\end{equation*}
The contribution to the coefficient of $cdh(ceg)^{m-1}$ in the linear relation corresponding to comparing basis $(aek)^{m-1}ceg$ is:
\begin{equation*}
    \begin{split}
        &\frac{(q^2-1)^3}{q^4}f_1(q,m)+\frac{(q^2-1)^3}{q^4}f_1(q,m-1)+(q^2-1)^3f_1(q^{-1},m-1)\\
        &+\left(\frac{(q^2-1)^3}{q^6}+2\frac{(q^2-1)^3}{q^4}\right)f_2(q,m)\\
        &+(q^2-1)^2(1-q^{-2})f_3(q,m)+(q^2-1)^2(1-q^{-2})f_3(q,m-1)\\
        &+(q^2-1)^2(1-q^{-2})f_3(q^{-1},m-1)\\
        =&\frac{q^{-4m-4}+2q^{-4m-2}}{(1-q^{-2})(1+q^{-2})^2}+\frac{2q^{2m-2}+q^{2m}+q^{-2m-2}+2q^{-2m}}{(1-q^{-2})(1+q^{-2})}\\
        &-\frac{3q^{2m-2}+3q^{-2m-2}}{1-q^{-2}}+(m-2)q^{2m}-2q^{-2m}+(m+1)q^{-2m+2}\\
        &+\frac{(m-1)q^2-m-(2m-3)q^{-2}+(m+5)q^{-4}+(m+2)q^{-6}}{(1-q^{-2})(1+q^{-2})^2}\\
    \end{split}
\end{equation*}
The contribution to the coefficient of $(ceg)^{m}$ in the linear relation corresponding to comparing basis $(aek)^{m-1}ceg$ is:
\begin{equation*}
    \begin{split}
        &-\frac{(q^2-1)^4}{q^5}f_1(q,m)-\left(\frac{(q^2-1)^4}{q^7}+2\frac{(q^2-1)^4}{q^5}\right)f_2(q,m)\\
        &=-\frac{q^{-4m-3}+2q^{-4m-1}}{(1+q^{-2})^2}+(2m+1)q^{-2m+1}+q^{-2m-1}-2(m+1)q^{-2m+3}\\
        &-\frac{(m^2+3m-4)q^3-(2m+6)q-(2m^2+6m+2)q^{-1}+(2m+4)q^{-3}}{2(1+q^{-2})^2}\\
        &-\frac{(m^2+3m+2)q^{-5}}{2(1+q^{-2})^2}
    \end{split}
\end{equation*}

==> Chapters/Source_Matrix/bdk.tex <==
\subsection{Linear relation derived from comparing basis $(aek)^{m-1}bdk$}
\subsubsection{Left components}
Based on the order restriction, there are 3 possible forms of left component whose decomposition contains $(aek)^{m-1}bdk$:
\begin{enumerate}
    \item[1)] $(aek)^lbdk(aek)^{m-1-l}$
    \item[2)] $(aek)^lbek(aek)^kadk(aek)^{m-2-l-k}$
    \item[3)] $(aek)^ladk(aek)^kbek(aek)^{m-2-l-k}$ 
\end{enumerate}
\paragraph{Left components in the form of $(aek)^lbdk(aek)^{m-1-l}$}\label{3.1.1}
Since there is only $m-1$ generator $a$'s in these left components, we may ignore the new monomials generated by switching $a$ with other generators.
\begin{equation*}
    \begin{split}
        &(aek)^lbdk(aek)^{m-1-l}\\
        =&(aek)^{m-1}bdk+(q-q^{-1})*\sum_{i=1}^{m-1-l}(aek)^{l+i-1}aech(aek)^{m-1-l-i}dk\\
        &+(q-q^{-1})*\sum_{i=1}^{m-1-l}(aek)^lb(aek)^{i-1}aefg(aek)^{m-1-l-i}k\\
        &-(q-q^{-1})*\sum_{i=1}^{m-1-l}(aek)^lbd(aek)^{i-1}afhk(aek)^{m-1-l-i}+\cdots\\
    \end{split}
\end{equation*}
Notice that every term appearing in the decomposition contains exactly $m-1$ generator $a$ and $m-1$ generator $k$ besides $(aek)^{m-1}bdk$. Thus, we have:
\begin{equation*}
    \begin{split}
        &(aek)^{l+i-1}aech(aek)^{m-1-l-i}dk\\
        =&q^2*(aek)^{m-1}cdh-q^2(q-q^{-1})*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
and
\begin{equation*}
    \begin{split}
        &(aek)^lb(aek)^{i-1}aefg(aek)^{m-1-l-i}k\\
        =&q^2*(aek)^{m-1}bfg+\cdots\\
    \end{split}
\end{equation*}
and
\begin{equation*}
    \begin{split}
        &(aek)^lbd(aek)^{i-1}afhk(aek)^{m-1-l-i}\\
        =&(aek)^{m-2}afhbdk+(q^2-1)*(aek)^{m-1}bfg+(q^2-1)*(aek)^{m-1}cdh\\
        &-(q^2 - 1)^2/q*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
Together, we have:
\begin{equation*}
    \begin{split}
        &(aek)^lbdk(aek)^{m-1-l}\\
        =&(aek)^{m-1}bdk-(q-q^{-1})(m-1-l)*(aek)^{m-2}afhbdk\\
        &+(q-q^{-1})(m-1-l)*(aek)^{m-1}bfg+(q-q^{-1})(m-1-l)*(aek)^{m-1}cdh\\
        &-(q-q^{-1})^2(m-1-l)*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\paragraph{Left components in the form of $(aek)^lbek(aek)^kadk(aek)^{m-2-l-k}$}\label{3.1.2}
Again, we may ignore the new monomials generated from switching generator $a$ with other generators. Thus, we get:
\begin{equation*}
    \begin{split}
        &(aek)^lbek(aek)^kadk(aek)^{m-2-l-k}\\
        =&(aek)^{l+k+1}bdk(aek)^{m-2-l-k}\\
        &+(q-q^{-1})q^2(k+1)*(aek)^{m-1}cdh\\
        &-(q-q^{-1})^2q^2(k+1)*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
Then, using the result of subsection \ref{3.1.1}, we get:
\begin{equation*}
    \begin{split}
        &(aek)^lbek(aek)^kadk(aek)^{m-2-l-k}\\
        =&(aek)^{m-1}bdk-(q-q^{-1})(m-2-l-k)*(aek)^{m-2}afhbdk\\
        &+(q-q^{-1})(m-2-l-k)*(aek)^{m-1}bfg\\
        &+(q-q^{-1})(q^2(k+1)+m-2-l-k)*(aek)^{m-1}cdh\\
        &-(q-q^{-1})^2(q^2(k+1)+m-2-l-k)*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\paragraph{Left components in the form of $(aek)^ladk(aek)^kbek(aek)^{m-2-l-k}$}\label{3.1.3}
Again, we may ignore the new monomials generated from switching generator $a$ with other generators. Thus, we get:
\begin{equation*}
    \begin{split}
        &(aek)^ladk(aek)^kbek(aek)^{m-2-l-k}\\
         =&q^2*(aek)^lbdk(aek)^{m-1-l}-q^2(q-q^{-1})(k+1)*(aek)^{m-1}cdh+\cdots\\
    \end{split}
\end{equation*}
Then, using the result of subsection \ref{3.1.1}, we get:
\begin{equation*}
    \begin{split}
        &(aek)^ladk(aek)^kbek(aek)^{m-2-l-k}\\
        =&q^2*(aek)^{m-1}bdk-(q-q^{-1})q^2(m-1-l)*(aek)^{m-2}afhbdk\\
        &+(q-q^{-1})q^2(m-1-l)*(aek)^{m-1}bfg\\
        &+(q-q^{-1})q^2(m-2-l-k)*(aek)^{m-1}cdh\\
        &-(q-q^{-1})^2q^2(m-1-l)*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\subsubsection{Right components}
\paragraph{Right component corresponding to $(aek)^lbdk(aek)^{m-1-l}$}
When the left component is $(aek)^lbdk(aek)^{m-1-l}$, the corresponding right component is $(ceg)^lfbg(ceg)^{m-1-l}$. We have:
\begin{equation*}
    (ceg)^lfbg(ceg)^{m-1-l}=bfg(ceg)^{m-1}-(q-q^{-1})*(ceg)^m
\end{equation*}
Recall the decomposition of $(aek)^lbdk(aek)^{m-1-l}$ in subsection \ref{3.1.1}. By summing over index $l$, the contribution of $(ceg)^lfbg(ceg)^{m-1-l}$ to the linear relation corresponding to comparing basis $\boldsymbol{(aek)^{m-1}bdk}$ is:
$$m*bfg(ceg)^{m-1}-m(q-q^{-1})*(ceg)^m.$$
The contribution to the linear relation corresponding to comparing basis \\ $\boldsymbol{(aek)^{m-2}afhbdk}$ is:
\begin{equation*}
    \begin{split}
        &-(q-q^{-1})\sum_{l=0}^{m-1}(m-1-l)*\left[bfg(ceg)^{m-1}-(q-q^{-1})*(ceg)^m\right]\\
        =&-(q-q^{-1})\frac{m(m-1)}{2}*bfg(ceg)^{m-1}+(q-q^{-1})^2\frac{m(m-1)}{2}*(ceg)^{m}
    \end{split}
\end{equation*}
The contribution to the linear relation corresponding to comparing basis \\ $\boldsymbol{(aek)^{m-1}bfg}$ and $\boldsymbol{(aek)^{m-1}cdh}$ is:
\begin{equation*}
    \begin{split}
        &(q-q^{-1})\sum_{l=0}^{m-1}(m-1-l)*\left[bfg(ceg)^{m-1}-(q-q^{-1})*(ceg)^m\right]\\
        =&(q-q^{-1})\frac{m(m-1)}{2}*bfg(ceg)^{m-1}-(q-q^{-1})^2\frac{m(m-1)}{2}*(ceg)^{m}
    \end{split}
\end{equation*}
The contribution to the linear relation corresponding to comparing basis \\ $\boldsymbol{(aek)^{m-1}ceg}$ is:
\begin{equation*}
    \begin{split}
        &-(q-q^{-1})^2\sum_{l=0}^{m-1}(m-1-l)*\left[bfg(ceg)^{m-1}-(q-q^{-1})*(ceg)^m\right]\\
        =&-(q-q^{-1})^2\frac{m(m-1)}{2}*bfg(ceg)^{m-1}+(q-q^{-1})^3\frac{m(m-1)}{2}*(ceg)^{m}
    \end{split}
\end{equation*}
\paragraph{Right component corresponding to $(aek)^lbek(aek)^kadk(aek)^{m-2-l-k}$}
When the left component is $(aek)^lbek(aek)^kadk(aek)^{m-2-l-k}$, the corresponding right component is $(ceg)^lfeg(ceg)^kcbg(ceg)^{m-2-l-k}$. We have:
\begin{equation*}
    \begin{split}
        &(ceg)^lfeg(ceg)^kcbg(ceg)^{m-2-l-k}\\
        =&q^{-2k-2}*\left[bfg(ceg)^{m-1}-(q-q^{-1})*(ceg)^m\right]
    \end{split}
\end{equation*}
Recall the decomposition of $(aek)^lbek(aek)^kadk(aek)^{m-2-l-k}$ in subsection \ref{3.1.2}. We write $\mathcal{G}=bfg(ceg)^{m-1}-(q-q^{-1})*(ceg)^m$. By summing over index $l$ and $k$, the contribution of $(ceg)^lfeg(ceg)^kcbg(ceg)^{m-2-l-k}$ to the linear relation corresponding to comparing basis $\boldsymbol{(aek)^{m-1}bdk}$ is:
\begin{equation*}
    \begin{split}
        &\sum_{l=0}^{m-2}\sum_{k=0}^{m-2-l}q^{-2k-2}*\mathcal{G}\\
        =&\left[\frac{m-1}{q^2-1}+\frac{q^{-2m+2}-1}{(1-q^2)^2}\right]*\mathcal{G}
    \end{split}
\end{equation*}
the contribution to the linear relation corresponding to comparing basis\\ $\boldsymbol{(aek)^{m-2}afhbdk}$ is:
\begin{equation*}
    \begin{split}
        &-(q-q^{-1})\sum_{l=0}^{m-2}\sum_{k=0}^{m-2-l}(m-2-l-k)q^{-2k-2}*\mathcal{G}\\
        =&\left[\frac{q^{-2m+3}-(m-1)q^{-1}+(m-2)q}{(1-q^{2})^2}-\frac{(m-2)(m-1)q^{-1}}{2}\right]*\mathcal{G}
    \end{split}
\end{equation*}
the contribution to the linear relation corresponding to comparing basis\\ $\boldsymbol{(aek)^{m-1}bfg}$ is:
\begin{equation*}
    \begin{split}
        &(q-q^{-1})\sum_{l=0}^{m-2}\sum_{k=0}^{m-2-l}(m-2-l-k)q^{-2k-2}*\mathcal{G}\\
        =&\left[\frac{(m-2)(m-1)q^{-1}}{2}-\frac{q^{-2m+3}-(m-1)q^{-1}+(m-2)q}{(1-q^{2})^2}\right]*\mathcal{G}
    \end{split}
\end{equation*}
the contribution to the linear relation corresponding to comparing basis\\ $\boldsymbol{(aek)^{m-1}cdh}$ is:
\begin{equation*}
    \begin{split}
        &(q-q^{-1})\sum_{l=0}^{m-2}\sum_{k=0}^{m-2-l}((k+1)q^2+m-2-l-k)q^{-2k-2}*\mathcal{G}\\
        =&\frac{(q^{-2m}-1)(2q^6-2mq^4+2mq^6)}{2q(1-q^2)^2}*\mathcal{G}\\
        &+\frac{4mq^6+(m^2-7m)q^4-(2m^2-4m)q^2+m^2-m}{2q(1-q^2)^2}*\mathcal{G}
    \end{split}
\end{equation*}
the contribution to the linear relation corresponding to comparing basis\\ $\boldsymbol{(aek)^{m-1}ceg}$ is:
\begin{equation*}
    \begin{split}
        &-(q-q^{-1})^2\sum_{l=0}^{m-2}\sum_{k=0}^{m-2-l}((k+1)q^2+m-2-l-k)q^{-2k-2}*\mathcal{G}\\
        =&\frac{(q^{-2m}-1)(2q^6-2mq^4+2mq^6)}{2q^2(1-q^2)}*\mathcal{G}\\
        &+\frac{4mq^6+(m^2-7m)q^4-(2m^2-4m)q^2+m^2-m}{2q^2(1-q^2)}*\mathcal{G}
    \end{split}
\end{equation*}
\paragraph{Right component corresponding to $(aek)^ladk(aek)^kbek(aek)^{m-2-l-k}$}
When the left component is $(aek)^ladk(aek)^kbek(aek)^{m-2-l-k}$, the corresponding right component is $(ceg)^lcbg(ceg)^kfeg(ceg)^{m-2-l-k}$. We have:
\begin{equation*}
    (ceg)^lcbg(ceg)^kfeg(ceg)^{m-2-l-k}
    =q^{2k}*bfg(ceg)^{m-1}
\end{equation*}
Recall the decomposition of $(aek)^ladk(aek)^kbek(aek)^{m-2-l-k}$ in subsection \ref{3.1.3}. By summing over the index $l$ and $k$, the contribution of $(ceg)^lcbg(ceg)^kfeg(ceg)^{m-2-l-k}$ to the linear relation corresponding to comparing basis $\boldsymbol{(aek)^{m-1}bdk}$ is:
\begin{equation*}
    \begin{split}
        &\sum_{l=0}^{m-2}\sum_{k=0}^{m-2-l}q^{2k+2}*bfg(ceg)^{m-1}\\
        =&\left[(m-1)\frac{1}{q^{-2}-1}+\frac{q^{2m-2}-1}{(1-q^{-2})^2}\right]*bfg(ceg)^{m-1}
    \end{split}
\end{equation*}
the contribution to the linear relation corresponding to comparing basis $\boldsymbol{(aek)^{m-2}afhbdk}$ is:
\begin{equation*}
    \begin{split}
        &-(q-q^{-1})\sum_{l=0}^{m-2}\sum_{k=0}^{m-2-l}(m-1-l)q^{2k+2}*bfg(ceg)^{m-1}\\
        =&\left[\frac{m(m-1)q}{2}-\frac{q^{3}-mq^{2m+1}+(m-1)q^{2m+3}}{(1-q^{2})^2}\right]*bfg(ceg)^{m-1}
    \end{split}
\end{equation*}
the contribution to the linear relation corresponding to comparing basis $\boldsymbol{(aek)^{m-1}bfg}$ is:
\begin{equation*}
    \begin{split}
        &(q-q^{-1})\sum_{l=0}^{m-2}\sum_{k=0}^{m-2-l}(m-1-l)q^{2k+2}*bfg(ceg)^{m-1}\\
        =&\left[\frac{q^{3}-mq^{2m+1}+(m-1)q^{2m+3}}{(1-q^{2})^2}-\frac{m(m-1)q}{2}\right]*bfg(ceg)^{m-1}
    \end{split}
\end{equation*}
the contribution to the linear relation corresponding to comparing basis $\boldsymbol{(aek)^{m-1}cdh}$ is:
\begin{equation*}
    \begin{split}
        &(q-q^{-1})\sum_{l=0}^{m-2}\sum_{k=0}^{m-2-l}(m-2-l-k)q^{2k+2}*bfg(ceg)^{m-1}\\
        =&\left[\frac{q^{2m-3}-(m-1)q+(m-2)q^{-1}}{(1-q^{-2})^2}-\frac{(m-2)(m-1)q}{2}\right]*bfg(ceg)^{m-1}
    \end{split}
\end{equation*}
the contribution to the linear relation corresponding to comparing basis $\boldsymbol{(aek)^{m-1}ceg}$ is:
\begin{equation*}
    \begin{split}
        &-(q-q^{-1})^2\sum_{l=0}^{m-2}\sum_{k=0}^{m-2-l}(m-1-l)q^{2k+2}*bfg(ceg)^{m-1}\\
        =&\left[\frac{m(m-1)(q^2-1)}{2}-\frac{q^{2}-mq^{2m}+(m-1)q^{2m+2}}{(q^{2}-1)}\right]*bfg(ceg)^{m-1}
    \end{split}
\end{equation*}
\subsubsection{Contribution to the linear relation corresponding to different comparing basis}
\paragraph{Comparing basis $(aek)^{m-1}bdk$}\label{3.3.1}
The linear relation corresponding to $(aek)^{m-1}bdk$ contains standard monomial $bfg(ceg)^{m-1}$ and $(ceg)^m$. The coefficient of $bfg(ceg)^{m-1}$ is:
\begin{equation*}
    \begin{split}
        &m+\frac{m-1}{q^2-1}+\frac{q^{-2m+2}-1}{(1-q^2)^2}+\frac{m-1}{q^{-2}-1}+\frac{q^{2m-2}-1}{(1-q^{-2})^2}\\
        =&\frac{q^2(q^m-q^{-m})^2}{(1-q^{2})^2}
    \end{split}
\end{equation*}
When computing the coefficient of $(ceg)^m$, we have to consider the coefficient of $(aek)^{m-1}bdk$ in $D_q^m$. Using an argument similar to the case of $(aek)^{m-1}afh$, we find that the coefficient is $-mq$. Then, the coefficient of $(ceg)^{m}$ is:
\begin{equation*}
    \begin{split}
        &-m(q-q^{-1})+mq-(q-q^{-1})\left[\frac{m-1}{q^2-1}+\frac{q^{-2m+2}-1}{(1-q^2)^2}\right]\\
        =&\frac{q(q^{-2m}-1)}{1-q^2}
    \end{split}
\end{equation*}
\paragraph{Comparing basis $(aek)^{m-2}afhbdk$}\label{3.3.2}
The contribution to the coefficient of $bfg(ceg)^{m-1}$ in the linear relation corresponding to comparing basis $(aek)^{m-2}afhbdk$ is:
\begin{equation*}
    \begin{split}
        &-(q-q^{-1})\frac{m(m-1)}{2}+\frac{q^{-2m+3}-(m-1)q^{-1}+(m-2)q}{(1-q^{2})^2}\\
        &-\frac{(m-2)(m-1)q^{-1}}{2}+\frac{m(m-1)q}{2}-\frac{q^{3}-mq^{2m+1}+(m-1)q^{2m+3}}{(1-q^{2})^2}\\
        =&\frac{(m-2)q^3-mq}{(1-q^{2})^2}+\frac{q^{-2m+3}+mq^{2m+1}-(m-1)q^{2m+3}}{(1-q^{2})^2}
    \end{split}
\end{equation*}
The contribution to the coefficient of $(ceg)^{m}$ in the linear relation corresponding to comparing basis $(aek)^{m-2}afhbdk$ is:
\begin{equation*}
    \begin{split}
        &(q-q^{-1})^2\frac{m(m-1)}{2}+(q-q^{-1})\frac{(m-2)(m-1)q^{-1}}{2}\\
        &-(q-q^{-1})\frac{q^{-2m+3}-(m-1)q^{-1}+(m-2)q}{(1-q^{2})^2}\\
        =&\frac{-2q^{-2m+2}+(m^2-m)q^4+(2-2m^2)q^2+m^2+m}{2(q^2-1)}
    \end{split}
\end{equation*}
\paragraph{Comparing basis $(aek)^{m-1}bfg$}\label{3.3.3}
Notice that the sign of the coefficient of $(aek)^{m-1}bfg$ is always the opposite as that of $(aek)^{m-2}afhbdk$ in the decomposition of all 3 possible forms of right components. The contribution to the coefficient of $bfg(ceg)^{m-1}$ in the linear relation corresponding to comparing basis $(aek)^{m-1}bfg$ is:
\begin{equation*}
    \begin{split}
        &(q-q^{-1})\frac{m(m-1)}{2}+\frac{(m-2)(m-1)q^{-1}}{2}\\
        &-\frac{q^{-2m+3}-(m-1)q^{-1}+(m-2)q}{(1-q^{2})^2}-\frac{m(m-1)q}{2}\\
        &+\frac{q^{3}-mq^{2m+1}+(m-1)q^{2m+3}}{(1-q^{2})^2}\\
         =&-\frac{(m-2)q^3-mq}{(1-q^{2})^2}-\frac{q^{-2m+3}+mq^{2m+1}-(m-1)q^{2m+3}}{(1-q^{2})^2}
    \end{split}
\end{equation*}
The contribution to the coefficient of $(ceg)^{m}$ in the linear relation corresponding to comparing basis $(aek)^{m-1}bfg$ is:
\begin{equation*}
    \begin{split}
        &-(q-q^{-1})^2\frac{m(m-1)}{2}-(q-q^{-1})\frac{(m-2)(m-1)q^{-1}}{2}\\
        &+(q-q^{-1})\frac{q^{-2m+3}-(m-1)q^{-1}+(m-2)q}{(1-q^{2})^2}\\
        =&\frac{2q^{-2m+2}-(m^2-m)q^4-(2-2m^2)q^2-m^2-m}{2(q^2-1)}
    \end{split}
\end{equation*}
\paragraph{Comparing basis $(aek)^{m-1}cdh$}\label{3.3.4}
The contribution to the coefficient of $bfg(ceg)^{m-1}$ in the linear relation corresponding to comparing basis $(aek)^{m-1}cdh$ is:
\begin{equation*}
    \begin{split}
        &(q-q^{-1})\frac{m(m-1)}{2}+\frac{(q^{-2m}-1)(2q^6-2mq^4+2mq^6)}{2q(1-q^2)^2}\\
        &+\frac{4mq^6+(m^2-7m)q^4-(2m^2-4m)q^2+m^2-m}{2q(1-q^2)^2}-\frac{(m-2)(m-1)q}{2}\\
        &+\frac{q^{2m-3}-(m-1)q+(m-2)q^{-1}}{(1-q^{-2})^2}\\
        =&\frac{q^{-2m}(q^5-mq^3+mq^5)+q^{2m+1}}{(1-q^2)^2}+\frac{(m-1)q^5-3mq^3+(2m-1)q}{(1-q^2)^2}
    \end{split}
\end{equation*}
The contribution to the coefficient of $(ceg)^{m}$ in the linear relation corresponding to comparing basis $(aek)^{m-1}cdh$ is:
\begin{equation*}
    \begin{split}
        &-(q-q^{-1})^2\frac{m(m-1)}{2}-(q-q^{-1})\frac{(q^{-2m}-1)(2q^6-2mq^4+2mq^6)}{2q(1-q^2)^2}\\
        &-(q-q^{-1})\frac{4mq^6+(m^2-7m)q^4-(2m^2-4m)q^2+m^2-m}{2q(1-q^2)^2}\\
        =&\frac{q^{-2m}(q^4-mq^2+mq^4)}{(1-q^2)}+\frac{(m^2+m-2)q^4-(2m^2+2m)q^2+m^2+m}{2(1-q^2)}
    \end{split}
\end{equation*}
\paragraph{Comparing basis $(aek)^{m-1}ceg$}\label{3.3.5}
The contribution to the coefficient of $bfg(ceg)^{m-1}$ in the linear relation corresponding to comparing basis $(aek)^{m-1}ceg$ is:
\begin{equation*}
    \begin{split}
        &-(q-q^{-1})^2\frac{m(m-1)}{2}+\frac{(q^{-2m}-1)(2q^6-2mq^4+2mq^6)}{2q^2(1-q^2)}\\
        &+\frac{4mq^6+(m^2-7m)q^4-(2m^2-4m)q^2+m^2-m}{2q^2(1-q^2)}+\frac{m(m-1)(q^2-1)}{2}\\
        &-\frac{q^{2}-mq^{2m}+(m-1)q^{2m+2}}{(q^{2}-1)}\\
        =&\frac{q^{-2m}(q^4-mq^2+mq^4)-mq^{2m}+(m-1)q^{2m+2}}{(1-q^2)}-(m-1)q^2+m
    \end{split}
\end{equation*}
The contribution to the coefficient of $(ceg)^{m}$ in the linear relation corresponding to comparing basis $(aek)^{m-1}ceg$ is:
\begin{equation*}
    \begin{split}
        &(q-q^{-1})^3\frac{m(m-1)}{2}-(q-q^{-1})\frac{(q^{-2m}-1)(2q^6-2mq^4+2mq^6)}{2q^2(1-q^2)}\\
        &-(q-q^{-1})\frac{4mq^6+(m^2-7m)q^4-(2m^2-4m)q^2+m^2-m}{2q^2(1-q^2)}\\
        =&q^{-2m}(q^3-mq+mq^3)+\frac{(m^2+m-2)q^3}{2}+(\frac{1}{2q}-q)(m^2+m)
    \end{split}
\end{equation*}

==> Chapters/Source_Matrix/bfg.tex <==
\subsection{Linear relation derived from comparing basis $(aek)^{m-1}bfg$}
\subsubsection{Left components}\label{5.1}
Beside the variants of comparing basis $(aek)^{m-1}afh$, $(aek)^{m-1}bdk$, and\\ $(aek)^{m-2}afhbdk$, there are 6 possible forms of left components whose decomposition contains $(aek)^{m-1}bfg$. These 6 possible forms corresponds to the permutation of generator $b$, $f$, and $g$:
\begin{enumerate}
    \item[1)] $(aek)^{i_1}b(eka)^{i_2}f(kae)^{i_3}g(aek)^{m-1-i_1-i_2-i_3}$ 
    \item[2)] $(aek)^{i_1}afk(aek)^{i_2}be(kae)^{i_3}g(aek)^{m-2-i_1-i_2-i_3}$ 
    \item[3)] $(aek)^{i_1}be(kae)^{i_2}g(aek)^{i_3}afk(aek)^{m-2-i_1-i_2-i_3}$ 
    \item[4)] $(aek)^{i_1}af(kae)^{i_2}g(aek)^{i_3}bek(aek)^{m-2-i_1-i_2-i_3}$ 
    \item[5)] $(aek)^{i_1}aeg(aek)^{i_2}b(eka)^{i_3}fk(aek)^{m-2-i_1-i_2-i_3}$ 
    \item[6)] $(aek)^{i_1}aeg(aek)^{i_2}afk(aek)^{i_3}bek(aek)^{m-3-i_1-i_2-i_3}$ 
\end{enumerate}
Each of the 6 cases contains only $m-1$ generator $a$ and $m-1$ generator $k$. Thus, when considering the decomposition of these monomials, we may ignore the new monomials generated by switching generator $a$ and $k$ with other generators.\\
\textbf{Case 1):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}b(eka)^{i_2}f(kae)^{i_3}g(aek)^{m-1-i_1-i_2-i_3}\\
        =&(aek)^{m-1}bfg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 2):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}afk(aek)^{i_2}be(kae)^{i_3}g(aek)^{m-2-i_1-i_2-i_3}\\
        =&(aek)^{m-2}afkbeg+\cdots\\
        =&q*(aek)^{m-1}bfg+(1-q^2)*(aek)^{m-1}ceg\cdots
    \end{split}
\end{equation*}
\textbf{Case 3):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}be(kae)^{i_2}g(aek)^{i_3}afk(aek)^{m-2-i_1-i_2-i_3}\\
        =&(aek)^{m-2}begafk+\cdots\\
        =&q*(aek)^{m-1}bfg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 4):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}af(kae)^{i_2}g(aek)^{i_3}bek(aek)^{m-2-i_1-i_2-i_3}\\
        =&(aek)^{m-2}afgbek+\cdots\\
        =&q^2*(aek)^{m-1}bfg-(q^3-q)*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 5):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}aeg(aek)^{i_2}b(eka)^{i_3}fk(aek)^{m-2-i_1-i_2-i_3}\\
         =&(aek)^{m-2}aegbfk+\cdots\\
         =&q^2*(aek)^{m-1}bfg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 6):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}aeg(aek)^{i_2}afk(aek)^{i_3}bek(aek)^{m-3-i_1-i_2-i_3}\\
        =&(aek)^{m-3}aegafkbek+\cdots\\
        =&q^3*(aek)^{m-1}bfg-(q^4-q^2)*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\subsubsection{Right components}\label{5.2}
The right components corresponding to the 6 types of left components are:
\begin{enumerate}
    \item[1)] $(ceg)^{i_1}f(egc)^{i_2}h(gce)^{i_3}a(ceg)^{m-1-i_1-i_2-i_3}$
    \item[2)] $(ceg)^{i_1}chg(ceg)^{i_2}fe(gce)^{i_3}a(ceg)^{m-2-i_1-i_2-i_3}$
    \item[3)] $(ceg)^{i_1}fe(gce)^{i_2}a(ceg)^{i_3}chg(ceg)^{m-2-i_1-i_2-i_3}$ 
    \item[4)] $(ceg)^{i_1}ch(gce)^{i_2}a(ceg)^{i_3}feg(ceg)^{m-2-i_1-i_2-i_3}$ 
    \item[5)] $(ceg)^{i_1}cea(ceg)^{i_2}f(egc)^{i_3}hg(ceg)^{m-2-i_1-i_2-i_3}$ 
    \item[6)] $(ceg)^{i_1}cea(ceg)^{i_2}chg(ceg)^{i_3}feg(ceg)^{m-3-i_1-i_2-i_3}$ 
\end{enumerate}
\textbf{Case 1):}
\begin{equation*}
    \begin{split}
        &(ceg)^{i_1}f(egc)^{i_2}h(gce)^{i_3}a(ceg)^{m-1-i_1-i_2-i_3}\\
        =&q^{2i_1-2i_3}*afh(ceg)^{m-1}+(q^{-2(i_2+2i_3)}-q^{2i_1-2i_3})*bfgcdh(ceg)^{m-2}\\
        &-(q-q^{-1})q^{-2(i_2+2i_3)}*bfg(ceg)^{m-1}-(q-q^{-1})q^{-2(i_2+2i_3)}*cdh(ceg)^{m-1}\\
        &+(q-q^{-1})^2q^{-2(i_2+2i_3)}*(ceg)^{m}\\
    \end{split}
\end{equation*}
\textbf{Case 2):}
\begin{equation*}
    \begin{split}
        &(ceg)^{i_1}chg(ceg)^{i_2}fe(gce)^{i_3}a(ceg)^{m-2-i_1-i_2-i_3}\\
        =&q^{2i_1-2i_3-1}*afh(ceg)^{m-1}\\
        &+(q^{-2(i_2+2i_3)-3}-q^{2i_1-2i_3-1})*bfgcdh(ceg)^{m-2}\\
        &-(q-q^{-1})q^{-2(i_2+2i_3)-3}*bfg(ceg)^{m-1}\\
        &-(q-q^{-1})q^{-2(i_2+2i_3)-3}*cdh(ceg)^{m-1}\\
        &+(q-q^{-1})^2q^{-2(i_2+2i_3)-3}*(ceg)^{m}\\
    \end{split}
\end{equation*}
\textbf{Case 3):}
\begin{equation*}
    \begin{split}
        &(ceg)^{i_1}fe(gce)^{i_2}a(ceg)^{i_3}chg(ceg)^{m-2-i_1-i_2-i_3}\\
        =&q^{2i_1+2i_3+1}*afh(ceg)^{m-1}\\
        &+(q^{2i_3-2i_2-1}-q^{2i_1+2i_3+1})*bfgcdh(ceg)^{m-2}\\
        &-(q-q^{-1})q^{2i_3-2i_2-1}*cdh(ceg)^{m-1}\\
    \end{split}
\end{equation*}
\textbf{Case 4):}
\begin{equation*}
    \begin{split}
        &(ceg)^{i_1}ch(gce)^{i_2}a(ceg)^{i_3}feg(ceg)^{m-2-i_1-i_2-i_3}\\
        =&q^{2i_1+2i_3}*afh(ceg)^{m-1}\\
        &+(q^{2i_3-2i_2}-q^{2i_1+2i_3})*bfgcdh(ceg)^{m-2}\\
        &-(q-q^{-1})q^{2i_3-2i_2}*bfg(ceg)^{m-1}\\
    \end{split}
\end{equation*}
\textbf{Case 5):}
\begin{equation*}
    \begin{split}
        &(ceg)^{i_1}cea(ceg)^{i_2}f(egc)^{i_3}hg(ceg)^{m-2-i_1-i_2-i_3}\\
        =&q^{2i_1+4i_2+2i_3+2}*afh(ceg)^{m-1}\\
        &+(q^{4i_2+2i_3}-q^{2i_1+4i_2+2i_3+2})*bfgcdh(ceg)^{m-2}
    \end{split}
\end{equation*}
\textbf{Case 6):}
\begin{equation*}
    \begin{split}
        &(ceg)^{i_1}cea(ceg)^{i_2}chg(ceg)^{i_3}feg(ceg)^{m-3-i_1-i_2-i_3}\\
        =&q^{2i_1+4i_2+2i_3+3}*afh(ceg)^{m-1}\\
        &+(q^{4i_2+2i_3+1}-q^{2i_1+4i_2+2i_3+3})*bfgcdh(ceg)^{m-2}
    \end{split}
\end{equation*}
\subsubsection{Contribution to the linear relation corresponding to different comparing basis}\label{5.3}
Before we compute the contribution, we introduce the following notation:
\begin{equation*}
    \begin{split}
        g_1(q,m)=&\sum_{i_1=0}^{m-1}\sum_{i_2=0}^{m-1-i_1}\sum_{i_3=0}^{m-1-i_1-i_2}q^{2i_1-2i_3}\\
        =&-\frac{(m+1)q^{-2}}{(1-q^{-2})^2}+\frac{q^{2m-2}-q^{-2m-6}}{(1+q^{-2})(1-q^{-2})^3}\\ 
        g_2(q,m)=&\sum_{i_1=0}^{m-1}\sum_{i_2=0}^{m-1-i_1}\sum_{i_3=0}^{m-1-i_1-i_2}q^{2i_1+2i_3}\\
        =&\frac{mq^{-4}}{(1-q^{-2})^2}+2\frac{q^{-4}-q^{2m-4}}{(1-q^{-2})^3}+\frac{mq^{2m-2}}{(1-q^{-2})^2}\\
        g_3(q,m)=&\sum_{i_1=0}^{m-1}\sum_{i_2=0}^{m-1-i_1}\sum_{i_3=0}^{m-1-i_1-i_2}q^{2i_1+4i_2+2i_3}\\
        =&-\frac{q^{-8}-(m+1)q^{2m-8}+(m+1)q^{2m-4}-q^{4m-4}}{(1-q^{-2})^3(1+q^{-2})}\\
        h_1(q,m)=&\sum_{i_1=0}^{m-1}\sum_{i_2=0}^{m-1-i_1}\sum_{i_3=0}^{m-1-i_1-i_2}q^{-2(i_2+2i_3)}\\
        =&\frac{m}{(1-q^{-4})(1-q^{-2})}-\frac{q^4(q^{-2m}-1)}{(1-q^2)^3}+\frac{q^{-4m+4}-q^4}{(1-q^{2})(1-q^4)^2}\\
        h_2(q,m)=&\sum_{i_1=0}^{m-1}\sum_{i_2=0}^{m-1-i_1}\sum_{i_3=0}^{m-1-i_1-i_2}q^{2i_3-2i_2}\\
        =&\frac{m}{(1-q^2)(1-q^{-2})}+\frac{q^{2m+2}-q^2-q^{-2m-2}+q^{-2}}{(1-q^2)^2(1-q^{-4})}\\
        h_3(q,m)=&\sum_{i_1=0}^{m-1}\sum_{i_2=0}^{m-1-i_1}\sum_{i_3=0}^{m-1-i_1-i_2}q^{4i_2+2i_3}\\
        =&\frac{m}{(1-q^2)(1-q^4)}-\frac{q^6(q^{4m}-1)}{(1-q^2)(1-q^4)^2}+\frac{q^{2m+2}-q^2}{(1-q^2)^3}
    \end{split}
\end{equation*}
\paragraph{Comparing basis $(aek)^{m-1}bfg$}\label{5.3.1}
First we compute the coefficient of $afh(ceg)^{m-1}$. By the results of subsection \ref{5.1} and \ref{5.2}, \textbf{the coefficient of} $\boldsymbol{afh(ceg)^{m-1}}$ is:
\begin{equation*}
    \begin{split}
        &g_1(q,m)+g_1(q,m-1)+2q^2\cdot g_2(q,m-1)+q^4\cdot g_3(q,m-1)\\
        &+q^6\cdot g_3(q,m-2)\\
        =&\frac{(q^{2m}-1)^3}{q^{2m-2}(q^2-1)^3}
    \end{split}
\end{equation*}
The coefficient of $bfgcdh(ceg)^{m-2}$ comes from two parts: contribution from comparing basis $(aek)^{m-1}bfg$ and $(aek)^{m-2}afhbdk$. The contribution from comparing basis $(aek)^{m-2}afhbdk$ is computed in subsection \ref{4.3.2}. Here, we compute the contribution from comparing basis $(aek)^{m-1}bfg$:
\begin{equation*}
    \begin{split}
        &(h_1(q,m)-g_1(q,m))+(q^{-2}\cdot h_1(q,m-1)-g_1(q,m-1))\\
        &+((1+q^2)\cdot h_2(q,m-1)-2q^2\cdot g_2(q,m-1))\\
        &+(q^2\cdot h_3(q,m-1)-q^4\cdot g_3(q,m-1))+(q^4\cdot h_3(q,m-2)-q^6\cdot g_3(q,m-2))
    \end{split}
\end{equation*}
We have already known the summation of the $g_n(m)$ functions part. It suffices to compute:
\begin{equation*}
    \begin{split}
        &h_1(q,m)+q^{-2}\cdot h_1(q,m-1)+(1+q^2)\cdot h_2(q,m-1)+q^2\cdot h_3(q,m-1)\\
        &+q^4\cdot h_3(q,m-2)\\
        =&\frac{q^{4m+2}+q^{2m}(q^6-q^4-2q^2)-2q^6+q^4+q^2+q^{-2m}(q^6+q^4)-q^{-4m+4}}{(q^2+1)(q^2-1)^3}
    \end{split}
\end{equation*}
Together with the contribution from comparing basis  $(aek)^{m-2}afhbdk$, \textbf{the coefficient of } $\boldsymbol{bfgcdh(ceg)^{m-2}}$ is:
\begin{equation*}
    \begin{split}
        &\frac{q^{-4n-4}+q^{4n-4}+2(q^{-2}+q^{-4}+q^{-6})}{(1-q^{-2})^3(1+q^{-2})}-\frac{q^{-2n-4}+q^{-2n-2}+q^{2n-2}+q^{2n-4}}{(1-q^{-2})^3}\\
        &+\frac{q^{4m+2}+q^{2m}(q^6-q^4-2q^2)-2q^6+q^4+q^2+q^{-2m}(q^6+q^4)-q^{-4m+4}}{(q^2+1)(q^2-1)^3}\\
        &-\frac{(q^{2m}-1)^3}{q^{2m-2}(q^2-1)^3}\\
        =&\frac{q^{6m}-3q^{4m}+3q^{2m}-1}{q^{2m-2}(q^2-1)^3}-\frac{(q^{2m}-1)^3}{q^{2m-2}(q^2-1)^3}\\
        =&0
    \end{split}
\end{equation*}
The coefficient of $bfg(ceg)^{m-1}$ comes from 3 parts: the contribution from comparing basis $(aek)^{m-1}bdk$, $(aek)^{m-2}afhbdk$, and $(aek)^{m-1}bfg$. The contribution from $(aek)^{m-1}bdk$ and $(aek)^{m-2}afhbdk$ has been computed in subsection \ref{3.3.3} and \ref{4.3.2}. Here, we compute the contribution from comparing basis $(aek)^{m-1}bfg$:
\begin{equation*}
    \begin{split}
        &-(q-q^{-1})(h_1(q,m)+q^{-2}\cdot h_1(q,m-1)+q^2\cdot h_2(q,m-1))\\
        =&\frac{q^3-2q^{-2m+3}-q^{-2m+5}+2q^5-q^{2m+5}+q^{-4m+3}}{(1+q^2)(1-q^2)^2}
    \end{split}
\end{equation*}
Together, \textbf{the coefficient of} $\boldsymbol{bfg(ceg)^{m-1}}$ is:
\begin{equation*}
    \begin{split}
        &-\frac{(m-2)q^3-mq}{(1-q^{2})^2}-\frac{q^{-2m+3}+mq^{2m+1}-(m-1)q^{2m+3}}{(1-q^{2})^2}\\
        &+\frac{-q^{-4m-3}-q^{-2m-1}+q^{2m-5}}{(1-q^{-2})^2(1+q^{-2})}+\frac{(m-2)q^{-1}-3q^{-3}-(m+2)q^{-5}}{(1-q^{-2})^2(1+q^{-2})}\\
        &+\frac{q^{-2m-3}+2q^{-2m-1}+mq^{2m-3}-(m-1)q^{2m-1}}{(1-q^{-2})^2}\\
        &+\frac{q^3-2q^{-2m+3}-q^{-2m+5}+2q^5-q^{2m+5}+q^{-4m+3}}{(1+q^2)(1-q^2)^2}\\
        =&-\frac{(q^{2m}-1)^2}{q^{2m-1}(q^2-1)}
    \end{split}
\end{equation*}
The coefficient of $cdh(ceg)^{m-1}$ comes from 3 parts: the contribution from comparing basis $(aek)^{m-1}afh$, $(aek)^{m-2}afhbdk$, and $(aek)^{m-1}bfg$. The contribution from $(aek)^{m-1}afh$ and $(aek)^{m-2}afhbdk$ has been computed in subsection \ref{2.3.3} and \ref{4.3.2}, respectively. Here, we compute the contribution from comparing basis $(aek)^{m-1}bfg$:
\begin{equation*}
    \begin{split}
        &-(q-q^{-1})(h_1(q,m)+q^{-2}\cdot h_1(q,m-1)+h_2(q,m-1))\\
        =&\frac{q^{-4m+3}+q^{-2m+3}-2q^{-2m+5}-q^{2m+3}-mq+(m+1)q^3+(m+2)q^5-mq^7}{(1-q^2)^2(1+q^2)}
    \end{split}
\end{equation*}
Together, \textbf{the coefficient of} $\boldsymbol{cdh(ceg)^{m-1}}$ is:
\begin{equation*}
    \begin{split}
        &\frac{q^{-4m+3}+q^{-2m+3}-2q^{-2m+5}-q^{2m+3}-mq+(m+1)q^3+(m+2)q^5-mq^7}{(1-q^2)^2(1+q^2)}\\
        &+\frac{-q^{-4m-3}-q^{2m-1}-q^{-2m+1}}{(1-q^{-2})^2(1+q^{-2})}-\frac{mq^{-2m+1}}{1-q^{-2}}+\frac{q^{-2m-3}}{(1-q^{-2})^2}\\
        &+\frac{q+(m+1)q^{-1}-(m+1)q^{-5}}{(1-q^{-2})^2(1+q^{-2})}\\
        &+\frac{2mq^5-(3m+1)q^3+mq}{(1-q^2)^2}+\frac{mq^{2m+1}-(m-1)q^{2m+3}}{(1-q^2)^2}\\
        &+\frac{(mq^5-2mq^3+mq+q^5+q^3-q)(q^{-2m}-1)}{(1-q^2)^2}\\
        =&-\frac{m(q^{2m}-1)^2}{q^{2m-1}(q^2-1)}
    \end{split}
\end{equation*}
The coefficient of $(ceg)^{m}$ comes from 5 parts: the contribution from comparing basis $(aek)^{m-1}afh$, $(aek)^{m-1}bdk$, $(aek)^{m-2}afhbdk$, $(aek)^{m-1}bfg$, and the coefficient of $(aek)^{m-1}bfg$ in the decomposition of $D_q^m$. The contribution from $(aek)^{m-1}afh$, $(aek)^{m-1}bdk$, and $(aek)^{m-2}afhbdk$ has been computed in subsection \ref{2.3.3}, \ref{3.3.3} and \ref{4.3.2}, respectively.\\
\\
In the expansion of $D_q^m$, the possible terms that may contribute to the coefficient of $(aek)^{m-1}bfg$ are $(aek)^lafh(aek)^{m-2-l}$, $(aek)^lbdk(aek)^{m-2-l}$, \\$(aek)^lbdk(aek)^{k}afh(aek)^{m-3-l-k}$, and $(aek)^lbfg(aek)^{m-2-l}$. As shown in \ref{2.1.1} and \ref{3.1.1}, the contribution of $(aek)^lafh(aek)^{m-2-l}$ and $(aek)^lbdk(aek)^{m-2-l}$ cancels each other. Comparing with subsection \ref{4.1} case 1), the contribution of one $(aek)^lbdk(aek)^{k}afh(aek)^{m-3-l-k}$ term is $(1-q^{-2})$. Since there are $\frac{m(m-1)}{2}$ many $(aek)^lbdk(aek)^{k}afh(aek)^{m-3-l-k}$ terms and the coefficient is $q^2$, the total contribution coming from terms in the form of $(aek)^lbdk(aek)^{k}afh(aek)^{m-3-l-k}$ to the coefficient of $(aek)^{m-1}bfg$ is $\frac{m(m-1)}{2}(q^2-1)$. The contribution from $(aek)^lbfg(aek)^{m-2-l}$ is $mq^2$. Hence, the coefficient of $(aek)^{m-1}bfg$ in $D_q^m$ is:
\begin{equation*}
    \frac{m(m+1)}{2}q^2-\frac{m(m-1)}{2}
\end{equation*}
Then, we compute the contribution from comparing basis $(aek)^{m-1}bfg$:
\begin{equation*}
    \begin{split}
        &(q-q^{-1})^2(h_1(q,m)+q^{-2}\cdot h_2(q,m-1))\\
        =&\frac{mq^6-mq^2-2q^4-q^2+2q^{-2m+4}+2q^{-2m+2}-q^{-4m+2}}{(q^2-1)(q^2+1)}
    \end{split}
\end{equation*}
Together, \textbf{the coefficient of} $\boldsymbol{(ceg)^m}$ is:
\begin{equation*}
    \begin{split}
        &\frac{(m^2+m-2)q^2-(m^2-3m)-(m^2+m-2)q^{-2}+(m^2+3m+2)q^{-4}}{2(1-q^{-2})(1+q^{-2})}\\
        &+\frac{q^{-4m-2}}{(1-q^{-2})(1+q^{-2})}+\frac{(m+1)q^{-2m+2}-(m+1)q^{-2m}-q^{-2m-2}}{(1-q^{-2})}\\
        &+\frac{(5m-m^2)q^4+(2m^2-8m)q^2+(3m-m^2)}{2(1-q^2)}\\
        &+\frac{(mq^4-2mq^2+m+q^4+q^2-1)(q^{-2m}-1)}{1-q^2}\\
        &+\frac{2q^{-2m+2}-(m^2-m)q^4-(2-2m^2)q^2-m^2-m}{2(q^2-1)}\\
        &+\frac{mq^6-mq^2-2q^4-q^2+2q^{-2m+4}+2q^{-2m+2}-q^{-4m+2}}{(q^2-1)(q^2+1)}\\
        &-\left[ \frac{m(m+1)}{2}q^2-\frac{m(m-1)}{2}\right]\\
        =&-\frac{((m+1)q^2-m)(q^{2m}-1)}{q^{2m}(q^2-1)}
    \end{split}
\end{equation*}
\paragraph{Comparing basis $(aek)^{m-1}ceg$}\label{5.3.2}
Comparing with the results in \ref{5.1}, the comparing basis $(aek)^{m-1}ceg$ appears in case 2), 4), and 6).\\
The contribution to the coefficient of $afh(ceg)^{m-1}$ in the linear relation corresponding to $(aek)^{m-1}ceg$ is:
\begin{equation*}
    \begin{split}
        &\frac{1-q^2}{q}\cdot g_1(q,m-1)-(q^3-q)\cdot g_2(q,m-1)-(q^4-q^2)q^3\cdot g_3(q,m-2)\\
        =&\frac{-q^{4m-5}+q^{-2m-3}+q^{2m-3}+2q^{2m-5}}{(1-q^{-2})^2(1+q^{-2})}-\frac{2q^{-3}+q^{-5}}{(1-q^{-2})^2(1+q^{-2})}
    \end{split}
\end{equation*}
The contribution to the coefficient of $bfgcdh(ceg)^{m-2}$ in the linear relation corresponding to $(aek)^{m-1}ceg$ is:
\begin{equation*}
    \begin{split}
        &(1-q^2)\left(\frac{h_1(q,m-1)}{q^3}-\frac{g_1(q,m-1)}{q}\right)\\
        &-(q^3-q)(h_2(q,m-1)-g_2(q,m-1))\\
        &-(q^4-q^2)(q\cdot h_3(q,m-2)-q^3\cdot g_3(q,m-2))\\
        =&\frac{q^{4m+3}+q^{-4m+5}+mq^9+(1-m)q^7+(2-m)q^5+(m+2)q^3+q}{(1-q^4)^2}
        \\&-\frac{q^{2m+3}+2q^{-2m+3}+q^{2m+1}+2q^{-2m+5}+q^{2m+5}+q^{2m+7}}{(1-q^4)^2}
    \end{split}
\end{equation*}
The contribution to the coefficient of $bfg(ceg)^{m-1}$ in the linear relation corresponding to $(aek)^{m-1}ceg$ is:
\begin{equation*}
    \begin{split}
        &-(1-q^2)(q-q^{-1})/q^3\cdot h_1(q,m-1)+(q^3-q)(q-q^{-1})\cdot h_2(q,m-1)\\
        =&\frac{-q^{-4m+4}+q^{2m+6}+q^{2m+4}+q^{-2m+4}+q^{-2m+2}}{(q^2-1)(q^2+1)^2}\\
        &+\frac{-mq^8-q^6+(m-1)q^4-q^2}{(q^2-1)(q^2+1)^2}
    \end{split}
\end{equation*}
The contribution to the coefficient of $cdh(ceg)^{m-1}$ and $(ceg)^{m}$ in the linear relation corresponding to $(aek)^{m-1}ceg$ is $(1-q^2)^2/q^4\cdot h_1(q,m-1)$ and $(1-q^2)^3/q^5\cdot h_1(q,m-1)$, respectively.

==> Chapters/Source_Matrix/cdh.tex <==
\subsection{Linear relation derived from comparing basis $(aek)^{m-1}cdh$}
\subsubsection{Left components}\label{6.1}
Beside the variants of comparing basis $(aek)^{m-1}afh$, $(aek)^{m-1}bdk$, and\\ $(aek)^{m-2}afhbdk$, there are 6 possible forms of left components whose decomposition contains $(aek)^{m-1}cdh$. These 6 possible forms corresponds to the permutation of generator $c$, $d$, and $h$:
\begin{enumerate}
    \item[1)] $(aek)^{i_1}c(eka)^{i_2}d(kae)^{i_3}h(aek)^{m-1-i_1-i_2-i_3}$ 
    \item[2)] $(aek)^{i_1}ce(kae)^{i_2}h(aek)^{i_3}adk(aek)^{m-2-i_1-i_2-i_3}$ 
    \item[3)] $(aek)^{i_1}aeh(aek)^{i_2}c(eka)^{i_3}dk(aek)^{m-2-i_1-i_2-i_3}$ 
    \item[4)] $(aek)^{i_1}adk(aek)^{i_2}ce(kae)^{i_3}h(aek)^{m-2-i_1-i_2-i_3}$ 
    \item[5)] $(aek)^{i_1}ad(kae)^{i_2}h(aek)^{i_3}cek(aek)^{m-2-i_1-i_2-i_3}$ 
    \item[6)] $(aek)^{i_1}aeh(aek)^{i_2}adk(aek)^{i_3}cek(aek)^{m-3-i_1-i_2-i_3}$ 
\end{enumerate}
Each of the 6 cases contains only $m-1$ generator $a$ and $m-1$ generator $k$. Thus, when considering the decomposition of these monomials, we may ignore the new monomials generated by switching generator $a$ and $k$ with other generators.\\
\textbf{Case 1):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}c(eka)^{i_2}d(kae)^{i_3}h(aek)^{m-1-i_1-i_2-i_3}\\
        =&(aek)^{m-1}cdh+\cdots
    \end{split}
\end{equation*}
\textbf{Case 2):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}ce(kae)^{i_2}h(aek)^{i_3}adk(aek)^{m-2-i_1-i_2-i_3}\\
        =&q*(aek)^{m-1}cdh+(1-q^2)*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 3):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}aeh(aek)^{i_2}c(eka)^{i_3}dk(aek)^{m-2-i_1-i_2-i_3}\\
         =&q^2*(aek)^{m-1}cdh-(q^3-q)*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 4):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}adk(aek)^{i_2}ce(kae)^{i_3}h(aek)^{m-2-i_1-i_2-i_3}\\
        =&q*(aek)^{m-1}cdh+\cdots
    \end{split}
\end{equation*}
\textbf{Case 5):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}ad(kae)^{i_2}h(aek)^{i_3}cek(aek)^{m-2-i_1-i_2-i_3}\\
        =&q^2*(aek)^{m-1}cdh+\cdots
    \end{split}
\end{equation*}
\textbf{Case 6):}
\begin{equation*}
    \begin{split}
        &(aek)^{i_1}aeh(aek)^{i_2}adk(aek)^{i_3}cek(aek)^{m-3-i_1-i_2-i_3}\\
        =&q^3*(aek)^{m-1}cdh-(q^4-q^2)*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}

\subsubsection{Right components}\label{6.2}
The right components corresponding to the 6 types of left components are:
\begin{enumerate}
    \item[1)] $(ceg)^{i_1}k(egc)^{i_2}b(gce)^{i_3}d(ceg)^{m-1-i_1-i_2-i_3}$
    \item[2)]  $(ceg)^{i_1}k(egc)^{i_2}ed(ceg)^{i_3}cbg(ceg)^{m-2-i_1-i_2-i_3}$
    \item[3)] $(ceg)^{i_1}ced(ceg)^{i_2}k(egc)^{i_3}bg(ceg)^{m-2-i_1-i_2-i_3}$
    \item[4)] $(ceg)^{i_1}cbg(ceg)^{i_2}k(egc)^{i_3}ed(ceg)^{m-2-i_1-i_2-i_3}$
    \item[5)] $(ceg)^{i_1}cb(gce)^{i_2}d(ceg)^{i_3}keg(ceg)^{m-2-i_1-i_2-i_3}$ 
    \item[6)] $(ceg)^{i_1}ced(ceg)^{i_2}cbg(ceg)^{i_3}keg(ceg)^{m-3-i_1-i_2-i_3}$ 
\end{enumerate}
\textbf{Case 1):}
\begin{equation*}
    \begin{split}
        &(ceg)^{i_1}k(egc)^{i_2}b(gce)^{i_3}d(ceg)^{m-1-i_1-i_2-i_3}\\
        =&q^{-2i_1-4i_2-2i_3}*bdk(ceg)^{m-1}\\
        &+(q^{-4i_2-2i_3}-q^{-2i_1-4i_2-2i_3})*bfgcdh(ceg)^{m-2}\\
        &-(q-q^{-1})q^{-4i_2-2i_3}*bfg(ceg)^{m-1}\\
        &-(q-q^{-1})q^{-4i_2-2i_3}*cdh(ceg)^{m-1}\\
        &+(q-q^{-1})^2q^{-4i_2-2i_3}*(ceg)^{m}\\
    \end{split}
\end{equation*}
\textbf{Case 2):}
\begin{equation*}
    \begin{split}
        &(ceg)^{i_1}k(egc)^{i_2}ed(ceg)^{i_3}cbg(ceg)^{m-2-i_1-i_2-i_3}\\
        =&q^{-2i_1-4i_2-2i_3-3}*bdk(ceg)^{m-1}\\
        &+(q^{-4i_2-2i_3-3}-q^{-2i_1-4i_2-2i_3-3})*bfgcdh(ceg)^{m-2}\\
        &-(q-q^{-1})q^{-4i_2-2i_3-3}*bfg(ceg)^{m-1}\\
        &-(q-q^{-1})q^{-4i_2-2i_3-3}*cdh(ceg)^{m-1}\\
        &+(q-q^{-1})^2q^{-4i_2-2i_3-3}*(ceg)^{m}\\
    \end{split}
\end{equation*}
\textbf{Case 3):}
\begin{equation*}
    \begin{split}
        &(ceg)^{i_1}ced(ceg)^{i_2}k(egc)^{i_3}bg(ceg)^{m-2-i_1-i_2-i_3}\\
        =&q^{-2i_1-2i_3-2}*bdk(ceg)^{m-1}\\
        &+(q^{2i_2-2i_3}-q^{-2i_1-2i_3-2})*bfgcdh(ceg)^{m-2}\\
        &-(q-q^{-1})*q^{2i_2-2i_3}*cdh(ceg)^{m-1}\\
    \end{split}
\end{equation*}
\textbf{Case 4):}
\begin{equation*}
    \begin{split}
        &(ceg)^{i_1}cbg(ceg)^{i_2}k(egc)^{i_3}ed(ceg)^{m-2-i_1-i_2-i_3}\\
        =&q^{-2i_1-2i_3-1}*bdk(ceg)^{m-1}\\
        &+(q^{2i_2-2i_3-1}-q^{-2i_1-2i_3-1})*bfgcdh(ceg)^{m-2}\\
        &-q^{2i_2-2i_3-1}(q-q^{-1})*bfg(ceg)^{m-1}\\
    \end{split}
\end{equation*}
\textbf{Case 5):}
\begin{equation*}
    \begin{split}
        &(ceg)^{i_1}cb(gce)^{i_2}d(ceg)^{i_3}keg(ceg)^{m-2-i_1-i_2-i_3}\\
        =&q^{-2i_1+2i_3}*bdk(ceg)^{m-1}\\
        &+(q^{2i_2+4i_3}-q^{-2i_1+2i_3})*bfgcdh(ceg)^{m-2}
    \end{split}
\end{equation*}
\textbf{Case 6):}
\begin{equation*}
    \begin{split}
        &(ceg)^{i_1}ced(ceg)^{i_2}cbg(ceg)^{i_3}keg(ceg)^{m-3-i_1-i_2-i_3}\\
        =&q^{-2i_1+2i_3-1}*bdk(ceg)^{m-1}\\
        &+(q^{2i_2+4i_3+1}-q^{-2i_1+2i_3-1})*bfgcdh(ceg)^{m-2}
    \end{split}
\end{equation*}
\subsubsection{Contribution to the linear relation corresponding to different comparing basis}
We will use function $g_i$ and $h_i$ ($1\le i\le 3$) from subsection \ref{5.3}.
\paragraph{Comparing basis $(aek)^{m-1}cdh$}\label{6.3.1}
First we compute the coefficient of $bdk(ceg)^{m-1}$. By the results of subsection \ref{6.1} and \ref{6.2}, \textbf{the coefficient of} $\boldsymbol{bdk(ceg)^{m-1}}$ is:
\begin{equation*}
    \begin{split}
        &g_3(q^{-1},m)+q^{-2}\cdot g_3(q^{-1},m-1)+2\cdot g_2(q^{-1},m-1)\\
        &+q^2\cdot g_1(q^{-1},m-1)+q^2\cdot g_1(q^{-1},m-2)\\
        =&\frac{q^4(q^{2m}-1)^3}{q^{4m}(q^2-1)^3}
    \end{split}
\end{equation*}
The coefficient of $bfgcdh(ceg)^{m-2}$ comes from two parts: contribution from comparing basis $(aek)^{m-1}cdh$ and $(aek)^{m-2}afhbdk$. The contribution from comparing basis $(aek)^{m-2}afhbdk$ is computed in subsection \ref{4.3.3}. Here, we compute the contribution from comparing basis $(aek)^{m-1}cdh$:
\begin{equation*}
    \begin{split}
        &h_3(q^{-1},m)-g_3(q^{-1},m)+q^{-2}\cdot (h_3(q^{-1},m-1)-g_3(q^{-1},m-1))\\
        &+(1+q^2)\cdot h_2(q^{-1},m-1)-2\cdot g_2(q^{-1},m-1)+\\
        &+q^2\cdot h_1(q^{-1},m-1)-q^2\cdot g_1(q^{-1},m-1)\\
        &+q^4\cdot h_1(q^{-1},m-2)-q^2\cdot g_1(q^{-1},m-2)
    \end{split}
\end{equation*}
The $g_i$ part has been computed above. Here, we consider the $h_i$ part:
\begin{equation*}
    \begin{split}
        &h_3(q^{-1},m)+q^{-2}\cdot h_3(q^{-1},m-1)+(1+q^2)\cdot h_2(q^{-1},m-1)+\\
        &+q^2\cdot h_1(q^{-1},m-1)+q^4\cdot h_1(q^{-1},m-2)\\
        =&\frac{-q^{4-4m}+q^{4m+2}-2q^{2m+2}-q^{2m+4}+q^{2m+6}+q^{-2m+4}+q^{-2m+6}}{(q^2-1)^3(q^2+1)}\\
        &+\frac{q^2+q^{4}-2q^{6}}{(q^2-1)^3(q^2+1)}
    \end{split}
\end{equation*}
Together, \textbf{the coefficient of} $\boldsymbol{bfgcdh(ceg)^{m-2}}$ is:
\begin{equation*}
    \begin{split}
        &\frac{q^{-4m-4}+q^{4m-4}+2(q^{-2}+q^{-4}+q^{-6})}{(1-q^{-2})^3(1+q^{-2})}-\frac{q^{-2m-4}+q^{-2m-2}+q^{2m-2}+q^{2m-4}}{(1-q^{-2})^3}\\
        &+\frac{-q^{4-4m}+q^{4m+2}-2q^{2m+2}-q^{2m+4}+q^{2m+6}+q^{-2m+4}+q^{-2m+6}}{(q^2-1)^3(q^2+1)}\\
        &+\frac{q^2+q^{4}-2q^{6}}{(q^2-1)^3(q^2+1)}-\frac{q^4(q^{2m}-1)^3}{q^{4m}(q^2-1)^3}\\
        =&\frac{q^2(q^{2m}-1)^3}{q^{2m}(q^2-1)^3}-\frac{q^4(q^{2m}-1)^3}{q^{4m}(q^2-1)^3}\\
        =&\frac{(q^{2m+2}-q^4)(q^{2m}-1)^3}{q^{4m}(q^2-1)^3}
    \end{split}
\end{equation*}
The coefficient of $bfg(ceg)^{m-1}$ comes from 3 parts: the contribution from comparing basis $(aek)^{m-1}bdk$, $(aek)^{m-2}afhbdk$, and $(aek)^{m-1}cdh$. The contribution from $(aek)^{m-1}bdk$ and $(aek)^{m-2}afhbdk$ has been computed in subsection \ref{3.3.4} and \ref{4.3.3}. Here, we compute the contribution from comparing basis $(aek)^{m-1}cdh$:
\begin{equation*}
    \begin{split}
        &-(q-q^{-1})\left(h_3(q^{-1},m)+q^{-2}\cdot h_3(q^{-1},m-1)+h_2(q^{-1},m-1)\right)\\
        =&\frac{q^{-4m+3}-2q^{-2m+5}-q^{2m+3}-q^{-2m+3}-mq^7+(m+2)q^5+(m+1)q^3-mq}{(q^2-1)^2(q^2+1)}
    \end{split}
\end{equation*}
Together, \textbf{the coefficient of} $\boldsymbol{bfg(ceg)^{m-1}}$ is:
\begin{equation*}
    \begin{split}
        &\frac{q^{-4m+3}-2q^{-2m+5}-q^{2m+3}-q^{-2m+3}-mq^7+(m+2)q^5+(m+1)q^3-mq}{(q^2-1)^2(q^2+1)}\\
        &+\frac{q^{-2m}(q^5-mq^3+mq^5)+q^{2m+1}}{(1-q^2)^2}+\frac{(m-1)q^5-3mq^3+(2m-1)q}{(1-q^2)^2}\\
        &+\frac{-q^{-4m-3}-q^{-2m-3}-q^{2m-5}}{(1-q^{-2})^2(1+q^{-2})}+\frac{q+(m+1)q^{-1}-(m+1)q^{-5}}{(1-q^{-2})^2(1+q^{-2})}\\
        &+\frac{q^{-2m-3}+(m+1)q^{-2m-1}-(m+1)q^{-2m+1}-q^{2m-1}+q^{2m-3}}{(1-q^{-2})^2}\\
        =&\frac{q(q^{2m}-1)^2}{q^{2m}(1-q^2)}
    \end{split}
\end{equation*}
The coefficient of $cdh(ceg)^{m-1}$ comes from 3 parts: the contribution from comparing basis $(aek)^{m-1}afh$, $(aek)^{m-2}afhbdk$, and $(aek)^{m-1}cdh$. The contribution from $(aek)^{m-1}afh$ and $(aek)^{m-2}afhbdk$ has been computed in subsection \ref{2.3.4} and \ref{4.3.3}, respectively. Here, we compute the contribution from comparing basis $(aek)^{m-1}cdh$:
\begin{equation*}
    \begin{split}
        &-(q-q^{-1})\left(h_3(q^{-1},m)+q^{-2}\cdot h_3(q^{-1},m-1)+q^2\cdot h_2(q^{-1},m-1)\right)\\
        =&\frac{q^3-2q^{-2m+3}-q^{-2m+5}+2q^{5}-q^{2m+5}+q^{-4m+3}}{(q^2-1)^2(q^2+1)}
    \end{split}
\end{equation*}
Together, \textbf{the coefficient of} $\boldsymbol{cdh(ceg)^{m-1}}$ is:
\begin{equation*}
    \begin{split}
        &\frac{q^3-2q^{-2m+3}-q^{-2m+5}+2q^{5}-q^{2m+5}+q^{-4m+3}}{(q^2-1)^2(q^2+1)}\\
        &+\frac{-q^{-4m-3}-q^{-2m-1}+q^{2m-5}}{(1-q^{-2})^2(1+q^{-2})}+\frac{(m-2)q^{-1}-3q^{-3}-(m+2)q^{-5}}{(1-q^{-2})^2(1+q^{-2})}\\
        &+\frac{q^{-2m-3}+2q^{-2m-1}+mq^{2m-3}-(m-1)q^{2m-1}}{(1-q^{-2})^2}\\
        &-\frac{q^{2m-3}-mq^{-1}+(m-2)q^{-3}+mq^{-2m-1}-(m-1)q^{-2m-3}}{(1-q^{-2})^2}\\
        =&\frac{mq(q^{2m}-1)^2}{q^{2m}(1-q^2)}
    \end{split}
\end{equation*}
The coefficient of $(ceg)^{m}$ comes from 5 parts: the contribution from comparing basis $(aek)^{m-1}afh$, $(aek)^{m-1}bdk$, $(aek)^{m-2}afhbdk$, $(aek)^{m-1}cdh$, and the coefficient of $(aek)^{m-1}cdh$ in the decomposition of $D_q^m$. The contribution from $(aek)^{m-1}afh$, $(aek)^{m-1}bdk$, and $(aek)^{m-2}afhbdk$ has been computed in subsection \ref{2.3.4}, \ref{3.3.4} and \ref{4.3.3}, respectively. Using an argument similar to that of $(aek)^{m-1}bfg$ in subsection \ref{5.3.1}, the coefficient of $(aek)^{m-1}cdh$ in the decomposition of $D_q^m$ is:
\begin{equation*}
    \frac{m(m+1)}{2}q^2-\frac{m(m-1)}{2}.
\end{equation*}
Then, we compute the contribution from comparing basis $(aek)^{m-1}cdh$:
\begin{equation*}
    \begin{split}
        &(q-q^{-1})^2\left(h_3(q^{-1},m)+q^{-2}\cdot h_3(q^{-1},m-1)\right)\\
        =&\frac{mq^6-(m+1)q^2-2q^4+2q^{4-2m}+2q^{2-2m}-q^{2-4m}}{q^4-1}
    \end{split}
\end{equation*}
Together, \textbf{the coefficient of} $\boldsymbol{(ceg)^m}$ is:
\begin{equation*}
    \begin{split}
        &(q^2-1)\frac{m(m-1)}{2}-\frac{q^{-2}-mq^{-2m}+(m-1)q^{-2m-2}}{1-q^{-2}}\\
        &+\frac{q^{-2m}(q^4-mq^2+mq^4)}{(1-q^2)}+\frac{(m^2+m-2)q^4-(2m^2+2m)q^2+m^2+m}{2(1-q^2)}\\
        &+\frac{q^{-4m-2}}{(1-q^{-2})(1+q^{-2})}+\frac{-q^{-2m-2}-(m+1)q^{-2m}+(m+1)q^{-2m+2}}{(1-q^{-2})}\\
        &+\frac{(m^2+m-2)q^2-(m^2+3m)-(m^2+m-2)q^{-2}+(m^2+3m+2)q^{-4}}{2(1-q^{-2})(1+q^{-2})}\\
        &-\left[\frac{m(m+1)}{2}q^2-\frac{m(m-1)}{2}\right]\\
        =&\frac{(q^{2m}-1)((m+1)q^2-m)}{q^{2m}(1-q^2)}
    \end{split}
\end{equation*}
\paragraph{Comparing basis $(aek)^{m-1}ceg$}\label{6.3.2}
Comparing with the results in \ref{6.1}, the comparing basis $(aek)^{m-1}ceg$ appears in case 2), 3), and 6).\\
The contribution to the coefficient of $bdk(ceg)^{m-1}$ in the linear relation corresponding to $(aek)^{m-1}ceg$ is:
\begin{equation*}
    \begin{split}
        &(1-q^2)/q^3\cdot g_3(q^{-1},m-1)-(q^3-q)/q^2\cdot g_2(q^{-1},m-1)\\
        &-(q^4-q^2)/q\cdot g_1(q^{-1},m-2)\\
        =&\frac{q^5-q^{2m+3}+q^{-4m+5}-2q^{-2m+5}+2q^3-q^{-2m+3}}{(q^2-1)^2(q^2+1)}
    \end{split}
\end{equation*}
The contribution to the coefficient of $bfgcdh(ceg)^{m-2}$ in the linear relation corresponding to $(aek)^{m-1}ceg$ is:
\begin{equation*}
    \begin{split}
        &(1-q^2)/q^3\cdot (h_3(q^{-1},m-1)-g_3(q^{-1},m-1))\\
        &-(q^3-q)(h_2(q^{-1},m-1)-q^{-2}\cdot g_2(q^{-1},m-1))\\
        &-(q^4-q^2)(q\cdot h_1(q^{-1},m-2)-q^{-1}\cdot g_1(q^{-1},m-2))\\
        =&\frac{q^{-4m+5}-q^{4m+3}+mq^9-(m-1)q^7-(m+2)q^{5}+(m+2)q^3+q}{(q^4-1)^2}\\
        &+\frac{-q^{2m+7}-q^{2m+5}-q^{2m+3}-q^{2m+1}-2q^{-2m+5}-2q^{-2m+3}}{(q^4-1)^2}
    \end{split}
\end{equation*}
The contribution to the coefficient of $bfg(ceg)^{m-1}$ and $(ceg)^m$ in the linear relation corresponding to $(aek)^{m-1}ceg$ is $-(1-q^2)(q-q^{-1})/q^3\cdot h_3(q^{-1},m-1)$ and $(1-q^2)(q-q^{-1})^2/q^3\cdot h_3(q^{-1},m-1)$, respectively.\\
\\
The contribution to the coefficient of $cdh(ceg)^{m-1}$ in the linear relation corresponding to $(aek)^{m-1}ceg$ is
\begin{equation*}
    \begin{split}
        &-(q-q^{-1})((1-q^2)/q^{3}\cdot h_3(q^{-1},m-1)-(q^3-q)\cdot h_2(q^{-1},m-1))\\
        =&\frac{-q^{-4m+4}+q^{2m+6}+q^{2m+4}+q^{-2m+4}+q^{-2m+2}-mq^8-q^6+(m-1)q^4-q^2}{(q^2-1)(q^2+1)^2}
    \end{split}
\end{equation*}

==> Chapters/Source_Matrix/ceg.tex <==
\subsection{Linear relation derived from comparing basis $(aek)^{m-1}ceg$}
\subsubsection{Left components}
Besides the variant of comparing basis $(aek)^{m-1}afh$, $(aek)^{m-1}bdk$, \\ $(aek)^{m-2}afhbdk$, $(aek)^{m-1}bfg$, and $(aek)^{m-1}cdh$, there are 2 possible forms of left components whose decomposition contains $(aek)^{m-1}ceg$:
\begin{enumerate}
    \item[1)] $(aek)^laeg(aek)^kcek(aek)^{m-2-l-k}$ 
    \item[2)] $(aek)^lce(kae)^kg(aek)^{m-2-l-k}$ 
\end{enumerate}
The 2 cases contain only $m-1$ generator $a$ and $m-1$ generator $k$. Thus, when considering the decomposition of these monomials, we may ignore the new monomials generated by switching generator $a$ and $k$ with other generators.\\
\\
\textbf{Case 1):}
\begin{equation*}
    \begin{split}
        &(aek)^laeg(aek)^kcek(aek)^{m-2-l-k}\\
        =&q^2*(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\textbf{Case 2):}
\begin{equation*}
    \begin{split}
        &(aek)^lce(kae)^kg(aek)^{m-1-l-k}\\
        =&(aek)^{m-1}ceg+\cdots
    \end{split}
\end{equation*}
\subsubsection{Right components}
The right components corresponding to the 2 types of left components are:
\begin{enumerate}
    \item[1)] $(ceg)^lcea(ceg)^kkeg(ceg)^{m-2-l-k}$ 
    \item[2)] $(ceg)^lke(gce)^ka(ceg)^{m-1-l-k}$ 
\end{enumerate}
\textbf{Case 1):}
\begin{equation*}
    \begin{split}
        &(ceg)^lcea(ceg)^kkeg(ceg)^{m-2-l-k}\\
        =&(ceg)^lae(ceg)^kk(ceg)^{m-1-l-k}-(q-q^{-1})q^{4k}*(ceg)^{l+k}bdk(ceg)^{m-1-l-k}\\
        =&q^{2k}*(ceg)^laek(ceg)^{m-1-l}+(q-q^{-1})*\sum_{i=1}^kq^{4k-2i+2}*(ceg)^lafh(ceg)^{m-1-l}\\
        &-(q-q^{-1})q^{2k-2l}*bdk(ceg)^{m-1}-(q-q^{-1})(q^{4k}-q^{2k-2l})*bfgcdh(ceg)^{m-2}\\
        =&q^{2k}*(ceg)^laek(ceg)^{m-1-l}+(q^{4k+1}-q^{2k+1})*(ceg)^lafh(ceg)^{m-1-l}\\
        &-(q-q^{-1})q^{2k-2l}*bdk(ceg)^{m-1}-(q-q^{-1})(q^{4k}-q^{2k-2l})*bfgcdh(ceg)^{m-2}\\
        =&q^{2k}*(ceg)^laek(ceg)^{m-1-l}\\
        &+(q^{4k+1}-q^{2k+1})q^{2l}*afh(ceg)^{m-1}+(q^{4k+1}-q^{2k+1})(1-q^{2l})*bfgcdh(ceg)^{m-2}\\
        &-(q-q^{-1})q^{2k-2l}*bdk(ceg)^{m-1}-(q-q^{-1})(q^{4k}-q^{2k-2l})*bfgcdh(ceg)^{m-2}\\
    \end{split}
\end{equation*}
Notice that:
\begin{equation*}
    cegaek=aekceg+(q^3-q)*afhceg-(q-q^{-1})*bdkceg-\frac{(q^2-1)^2}{q}*bfgcdh
\end{equation*}
By applying the equation multiple times, we find that:
\begin{equation*}
    \begin{split}
        &(ceg)^laek\\
        =&aek(ceg)^l+(q^3-q)*\sum_{j=1}^l(ceg)^{l-j}afh(ceg)^{j}\\
        &-(q-q^{-1})*\sum_{j=1}^l(ceg)^{l-j}bdk(ceg)^{j}-l\frac{(q^2-1)^2}{q}*bfgcdh(ceg)^{l-1}\\
        =&aek(ceg)^l\\
        &+(q^3-q)\sum_{j=1}^lq^{2l-2j}*afh(ceg)^{l}+(q^3-q)\sum_{j=1}^l(1-q^{2l-2j})*bfgcdh(ceg)^{l-1}\\
        &-(q-q^{-1})\sum_{j=1}^lq^{2j-2l}*bdk(ceg)^{l}-(q-q^{-1})\sum_{j=1}^l(1-q^{-2l+2j})*bfgcdh(ceg)^{l-1}\\
        &-l\frac{(q^2-1)^2}{q}*bfgcdh(ceg)^{l-1}\\
        =&aek(ceg)^l+(q^{2l+1}-q)*afh(ceg)^{l}+((q^3-q)l-(q^{2l+1}-q))*bfgcdh(ceg)^{l-1}\\
        &+(q^{1-2l}-q)*bdk(ceg)^{l}-((q-q^{-1})l+(q^{1-2l}-q))*bfgcdh(ceg)^{l-1}\\
        &-l\frac{(q^2-1)^2}{q}*bfgcdh(ceg)^{l-1}\\
        =&aek(ceg)^l+(q^{2l+1}-q)*afh(ceg)^{l}+(q^{1-2l}-q)*bdk(ceg)^{l}\\
        &-q(q^l-q^{-l})^2*bfgcdh(ceg)^{l-1}\\
    \end{split}
\end{equation*}
Thus, case 1) becomes:
\begin{equation*}
    \begin{split}
        &(ceg)^lcea(ceg)^kkeg(ceg)^{m-2-l-k}\\
        =&q^{2k}*aek(ceg)^{m-1}+q^{2k}(q^{2l+1}-q)*afh(ceg)^{m-1}+q^{2k}(q^{1-2l}-q)*bdk(ceg)^{m-1}\\
        &-q^{2k+1}(q^l-q^{-l})^2*bfgcdh(ceg)^{m-2}\\
        &+(q^{4k+1}-q^{2k+1})q^{2l}*afh(ceg)^{m-1}+(q^{4k+1}-q^{2k+1})(1-q^{2l})*bfgcdh(ceg)^{m-2}\\
        &-(q-q^{-1})q^{2k-2l}*bdk(ceg)^{m-1}-(q-q^{-1})(q^{4k}-q^{2k-2l})*bfgcdh(ceg)^{m-2}\\
        =&q^{2k}*aek(ceg)^{m-1}\\
        &+q^{2k+1}(q^{2k+2l}-1)*afh(ceg)^{m-1}
        \\
        &+q^{2k-1}(q^{-2l}-q^2)*bdk(ceg)^{m-1}\\
        &+q^{2k}(q+q^{2k-1}-q^{-2l-1}-q^{2k+2l+1})*bfgcdh(ceg)^{m-2}\\
    \end{split}
\end{equation*}
\textbf{Case 2):}
\begin{equation*}
    \begin{split}
        &(ceg)^lke(gce)^ka(ceg)^{m-1-l-k}\\
        =&q^{-2k}*(ceg)^lkea(ceg)^{m-1-l}\\
        &-(q-q^{-1})\sum_{i=1}^{k}q^{-2(i-1)}*(ceg)^lke(ceg)^{k-i}cgbd(ceg)^{i-1+m-1-l-k}\\
        =&q^{-2k}*(ceg)^lkea(ceg)^{m-1-l}\\
        &-(q-q^{-1})q^{-4k-2}\sum_{i=1}^{k}q^{2i}*(ceg)^lkbd(ceg)^{m-1-l}\\
        =&q^{-2k}*(ceg)^lkea(ceg)^{m-1-l}\\
        &+(q^{-4k-1}-q^{-2k-1})*(ceg)^lkbd(ceg)^{m-1-l}\\
        =&q^{-2k}*(ceg)^laek(ceg)^{m-1-l}-(q-q^{-1})q^{2l-2k}*afh(ceg)^{m-1}\\
        &+(q^{-4k-1}-q^{-2k+1})q^{-2l}*bdk(ceg)^{m-1}\\
        &+\left((q^{-4k-1}-q^{-2k+1})(1-q^{-2l})-(q-q^{-1})q^{-2k}(1-q^{2l})\right)*bfgcdh(ceg)^{m-2}\\
        &-(q-q^{-1})(q^{-4k-1}-q^{-2k+1})*\left(bfg(ceg)^{m-1}+cdh(ceg)^{m-1}\right)\\
        &+\left((q-q^{-1})^2q^{-4k-1}-(q^3-q)q^{-2k}\right)*(ceg)^{m}\\
        =&q^{-2k}*aek(ceg)^l\\
        &+q^{-2k-1}(q^{2l}-q^2)*afh(ceg)^{l}\\
        &+q^{-2k+1}(q^{-2k-2l-2}-1)*bdk(ceg)^{l}\\
        &+q^{-2k-2l-1}(q^{2l}-1)(q^{-2k}-q^{2l})*bfgcdh(ceg)^{l-1}\\
        &-(q-q^{-1})(q^{-4k-1}-q^{-2k+1})*\left(bfg(ceg)^{m-1}+cdh(ceg)^{m-1}\right)\\
        &+\left((q-q^{-1})^2q^{-4k-1}-(q^3-q)q^{-2k}\right)*(ceg)^{m}
    \end{split}
\end{equation*}
\subsubsection{Linear relation corresponding to comparing basis $(aek)^{m-1}ceg$}\label{7.3}
\textbf{The coefficient of} $\boldsymbol{aek(ceg)^{m-1}}$ is:
\begin{equation*}
    \begin{split}
        &q^2\sum_{l=0}^{m-2}\sum_{k=0}^{m-2-l}q^{2k}+\sum_{l=0}^{m-1}\sum_{k=0}^{m-1-l}q^{-2k}\\
        =&\frac{q^2(q^{2m}-1)^2}{q^{2m}(q^2-1)^2}
    \end{split}
\end{equation*}
The coefficient of $afh(ceg)^{m-1}$ comes from 2 parts: the contribution from comparing basis $(aek)^{m-1}bfg$ and $(aek)^{m-1}ceg$. The contribution from $(aek)^{m-1}bfg$ has been computed in subsection \ref{5.3.2}. Here, we compute the contribution from $(aek)^{m-1}ceg$:
\begin{equation*}
    \begin{split}
        &q^2\sum_{l=0}^{m-2}\sum_{k=0}^{m-2-l}(q^{4k+2l+1}-q^{2k+1})+\sum_{l=0}^{m-1}\sum_{k=0}^{m-1-l}q^{-2k-1}(q^{2l}-q^2)\\
        =&\frac{q^{4m+1}-q^{2m+1}-q^{-2m+3}-q^{-2m+5}-q^{2m+3}-q^{2m+5}+q^{-2m+1}}{(q^2-1)^2(1+q^2)}\\
        &+\frac{2q^5+2q^3-q}{(q^2-1)^2(1+q^2)}
    \end{split}
\end{equation*}
Together, \textbf{the coefficient of} $\boldsymbol{afh(ceg)^{m-1}}$ is:
\begin{equation*}
    \begin{split}
        &\frac{q^{4m+1}-q^{2m+1}-q^{-2m+3}-q^{-2m+5}-q^{2m+3}-q^{2m+5}+q^{-2m+1}}{(q^2-1)^2(1+q^2)}\\
        &+\frac{2q^5+2q^3-q}{(q^2-1)^2(1+q^2)}\\
        &+\frac{-q^{4m-5}+q^{-2m-3}+q^{2m-3}+2q^{2m-5}}{(1-q^{-2})^2(1+q^{-2})}-\frac{2q^{-3}+q^{-5}}{(1-q^{-2})^2(1+q^{-2})}\\
        =&\frac{q(q^m-q^{-m})^2}{1-q^2}
    \end{split}
\end{equation*}
The coefficient of $bdk(ceg)^{m-1}$ comes from 2 parts: the contribution from comparing basis $(aek)^{m-1}cdh$ and $(aek)^{m-1}ceg$. The contribution from $(aek)^{m-1}bfg$ has been computed in subsection \ref{6.3.2}. Here, we compute the contribution from $(aek)^{m-1}ceg$:
\begin{equation*}
    \begin{split}
        &q^2\sum_{l=0}^{m-2}\sum_{k=0}^{m-2-l}q^{2k-1}(q^{-2l}-q^2)+\sum_{l=0}^{m-1}\sum_{k=0}^{m-1-l}q^{-2k+1}(q^{-2k-2l-2}-1)\\
        =&\frac{q^3-2q^{-2m+3}-q^{-2m+5}+2q^{5}-q^{2m+5}+q^{-4m+3}}{(q^2-1)^2(q^2+1)}
    \end{split}
\end{equation*}
Together, \textbf{the coefficient of} $\boldsymbol{bdk(ceg)^{m-1}}$ is:
\begin{equation*}
    \begin{split}
        &\frac{q^5-q^{2m+3}+q^{-4m+5}-2q^{-2m+5}+2q^3-q^{-2m+3}}{(q^2-1)^2(q^2+1)}\\
        &+\frac{q^3-2q^{-2m+3}-q^{-2m+5}+2q^{5}-q^{2m+5}+q^{-4m+3}}{(q^2-1)^2(q^2+1)}\\
        =&\frac{q^3(1-q^{2m})^3}{q^{4m}(q^2-1)^2}
    \end{split}
\end{equation*}
The coefficient of $bfgcdh(ceg)^{m-2}$ comes from 4 parts: the contribution from comparing basis $(aek)^{m-2}afhbdk$, $(aek)^{m-1}bfg$, $(aek)^{m-1}cdh$, and $(aek)^{m-1}ceg$. The contribution of $(aek)^{m-2}afhbdk$, $(aek)^{m-1}bfg$, and $(aek)^{m-1}cdh$ has been computed in subsection \ref{4.3.4}, \ref{5.3.2}, and \ref{6.3.2}, respectively. Here, we compute the contribution from $(aek)^{m-1}ceg$:
\begin{equation*}
    \begin{split}
        &q^2\sum_{l=0}^{m-2}\sum_{k=0}^{m-2-l}q^{2k}(q+q^{2k-1}-q^{-2l-1}-q^{2k+2l+1})\\
        &+\sum_{l=0}^{m-1}\sum_{k=0}^{m-1-l}q^{-2k-2l-1}(q^{2l}-1)(q^{-2k}-q^{2l})\\
        =&\frac{q^{2m+7}+q^{2m+5}+2q^{-2m+5}-q^{-4m+5}-q^{4m+3}+q^{2m+3}+2q^{-2m+3}+q^{2m+1}}{(q^4-1)^2}\\
        &+\frac{-mq^9+(m-1)q^7+(m-2)q^5-(m+2)q^3-q}{(q^4-1)^2}
    \end{split}
\end{equation*}
Together, \textbf{the coefficient of} $\boldsymbol{bfgcdh(ceg)^{m-2}}$ is:
\begin{equation*}
    \begin{split}
        &\frac{q^{2m+7}+q^{2m+5}+2q^{-2m+5}-q^{-4m+5}-q^{4m+3}+q^{2m+3}+2q^{-2m+3}+q^{2m+1}}{(q^4-1)^2}\\
        &+\frac{-mq^9+(m-1)q^7+(m-2)q^5-(m+2)q^3-q}{(q^4-1)^2}\\
        &+\frac{-mq^9+(m-3)q^7+(m-6)q^5-(m+6)q^3-3q}{(q^4-1)^2}\\
        &+\frac{2q^{2m+7}+4q^{2m+5}+4q^{2m+3}+2q^{2m+1}}{(q^4-1)^2}\\
        &+\frac{q^{-2m+7}+5q^{-2m+5}+5q^{-2m+3}+q^{-2m+1}}{(q^4-1)^2}\\
        &+\frac{-q^{4m+5}-2q^{-4m+5}-2q^{4m+3}-q^{-4m+3}}{(q^4-1)^2}\\
        &+\frac{q^{-4m+5}-q^{4m+3}+mq^9-(m-1)q^7-(m+2)q^{5}+(m+2)q^3+q}{(q^4-1)^2}\\
        &+\frac{-q^{2m+7}-q^{2m+5}-q^{2m+3}-q^{2m+1}-2q^{-2m+5}-2q^{-2m+3}}{(q^4-1)^2}\\
        &+\frac{-q^{-4m+7}-q^{4m+1}+mq^9-mq^7-(m+3)q^{5}+(m-3)q^3}{(q^4-1)^2}\\
        &+\frac{-q^{2m+7}+q^{2m+5}+3q^{2m+3}+q^{2m+1}+2q^{-2m+7}+2q^{-2m+5}}{(q^4-1)^2}\\
        =&\frac{-(q^{2m-2}-1)(q^{2m}-1)^3}{q^{4m-3}(q^2-1)^2}
    \end{split}
\end{equation*}
The coefficient of $bfg(ceg)^{m-1}$ comes from 5 parts: the contribution from comparing basis $(aek)^{m-1}bdk$, $(aek)^{m-2}afhbdk$, $(aek)^{m-1}bfg$, $(aek)^{m-1}cdh$, and $(aek)^{m-1}ceg$. The contribution of $(aek)^{m-1}bdk$, $(aek)^{m-2}afhbdk$, $(aek)^{m-1}bfg$, and $(aek)^{m-1}cdh$ has been computed in subsection \ref{3.3.5}, \ref{4.3.4}, \ref{5.3.2}, and \ref{6.3.2}, respectively. Here, we compute the contribution from $(aek)^{m-1}ceg$:
\begin{equation*}
    \begin{split}
        &-(q-q^{-1})\sum_{l=0}^{m-1}\sum_{k=0}^{m-1-l}(q^{-4k-1}-q^{-2k+1})\\
        =&\frac{mq^8-(m+2)q^4-q^6+q^{-2m+6}+2q^{-2m+4}+q^{-2m+2}-q^{-4m+2}}{(q^2-1)(q^2+1)^2}
    \end{split}
\end{equation*}
Together, \textbf{the coefficient of} $\boldsymbol{bfg(ceg)^{m-1}}$ is:
\begin{equation*}
    \begin{split}
        &\frac{q^{-2m}(q^4-mq^2+mq^4)-mq^{2m}+(m-1)q^{2m+2}}{(1-q^2)}-(m-1)q^2+m\\
        &+\frac{q^{-4n-4}+2q^{-4n-2}}{(1-q^{-2})(1+q^{-2})^2}+\frac{2q^{2n-2}+q^{2n}+q^{-2n-2}+2q^{-2n}}{(1-q^{-2})(1+q^{-2})}\\
        &+\frac{-3q^{2n-2}-3q^{-2n-2}}{1-q^{-2}}+(n-2)q^{2n}-2q^{-2n}+(n+1)q^{-2n+2}\\
        &+\frac{(n-1)q^2-n-(2n-3)q^{-2}+(n+5)q^{-4}+(n+2)q^{-6}}{(1-q^{-2})(1+q^{-2})^2}\\
        &+\frac{-q^{-4m+4}+q^{2m+6}+q^{2m+4}+q^{-2m+4}+q^{-2m+2}}{(q^2-1)(q^2+1)^2}\\
        &+\frac{-mq^8-q^6+(m-1)q^4-q^2}{(q^2-1)(q^2+1)^2}\\
        &+\frac{(m-1)q^{6}-q^4-(m+1)q^2+q^{-2m+6}+2q^{-2m+4}-q^{-4m+4}+q^{-2m+2}}{(q^2-1)(q^2+1)^2}\\
        &+\frac{mq^8-(m+2)q^4-q^6+q^{-2m+6}+2q^{-2m+4}+q^{-2m+2}-q^{-4m+2}}{(q^2-1)(q^2+1)^2}\\
        =&q^{2m}-2+q^{-2m}\\
        =&\frac{(q^{2m}-1)^2}{q^{2m}}
    \end{split}
\end{equation*}
The coefficient of $cdh(ceg)^{m-1}$ comes from 5 parts: the contribution from comparing basis $(aek)^{m-1}afh$, $(aek)^{m-2}afhbdk$, $(aek)^{m-1}bfg$, $(aek)^{m-1}cdh$, and $(aek)^{m-1}ceg$. The contribution of $(aek)^{m-1}afh$, $(aek)^{m-2}afhbdk$, $(aek)^{m-1}bfg$, and $(aek)^{m-1}cdh$ has been computed in subsection \ref{2.3.5}, \ref{4.3.4}, \ref{5.3.2}, and \ref{6.3.2}, respectively. Here, we compute the contribution from $(aek)^{m-1}ceg$:
\begin{equation*}
    \begin{split}
        &-(q-q^{-1})\sum_{l=0}^{m-1}\sum_{k=0}^{m-1-l}(q^{-4k-1}-q^{-2k+1})\\
        =&\frac{mq^8-(m+2)q^4-q^6+q^{-2m+6}+2q^{-2m+4}+q^{-2m+2}-q^{-4m+2}}{(q^2-1)(q^2+1)^2}
    \end{split}
\end{equation*}
Together, \textbf{the coefficient of} $\boldsymbol{cdh(ceg)^{m-1}}$ is:
\begin{equation*}
    \begin{split}
        &\frac{(mq^4-2mq^2+m+q^4+q^2-1)(q^{-2m}-1)}{(1-q^2)}+\frac{-2mq^4+2mq^2+q^{2m}-1}{q^2-1}\\
        &+\frac{q^{-4m-4}+2q^{-4m-2}}{(1-q^{-2})(1+q^{-2})^2}+\frac{2q^{2m-2}+q^{2m}+q^{-2m-2}+2q^{-2m}}{(1-q^{-2})(1+q^{-2})}\\
        &-\frac{3q^{2m-2}+3q^{-2m-2}}{1-q^{-2}}+(m-2)q^{2m}-2q^{-2m}+(m+1)q^{-2m+2}\\
        &+\frac{(m-1)q^2-m-(2m-3)q^{-2}+(m+5)q^{-4}+(m+2)q^{-6}}{(1-q^{-2})(1+q^{-2})^2}\\
        &+\frac{(m-1)q^6-q^4-(m+1)q^2+q^{-2m+6}+2q^{-2m+4}-q^{-4m+4}+q^{-2m+2}}{(q^2-1)(q^2+1)^2}\\
        &+\frac{-q^{-4m+4}+q^{2m+6}+q^{2m+4}+q^{-2m+4}+q^{-2m+2}}{(q^2-1)(q^2+1)^2}\\
        &+\frac{-mq^8-q^6+(m-1)q^4-q^2}{(q^2-1)(q^2+1)^2}\\
        =&mq^{2m}-2m+mq^{-2m}\\
        =&\frac{m(q^{2m}-1)^2}{q^{2m}}
    \end{split}
\end{equation*}
The coefficient of $(ceg)^{m}$ comes from 7 parts: the contribution from comparing basis $(aek)^{m-1}afh$, $(aek)^{m-1}bdk$, $(aek)^{m-2}afhbdk$, $(aek)^{m-1}bfg$, $(aek)^{m-1}cdh$, $(aek)^{m-1}ceg$, and the coefficient of $(aek)^{m-1}ceg$ in the decomposition of $D_q^m$. The contribution of $(aek)^{m-1}afh$, $(aek)^{m-1}bdk$, $(aek)^{m-2}afhbdk$, $(aek)^{m-1}bfg$, and $(aek)^{m-1}cdh$ has been computed in subsection \ref{2.3.5}, \ref{3.3.5}, \ref{4.3.4}, \ref{5.3.2}, and \ref{6.3.2}, respectively. \\
\\
Similar to the case of $(aek)^{m-1}bfg$ and $(aek)^{m-1}cdh$, the possible terms that may contribute to the coefficient of $(aek)^{m-1}ceg$ in the decomposition of $D_q^m$ are terms in form $(aek)^lbdk(aek)^kafh(aek)^{m-2-l-k}$ and $(aek)^lceg(aek)^{m-1-l}$. There are $\frac{n(n-1)}{2}$ many $(aek)^lbdk(aek)^kafh(aek)^{m-2-l-k}$ terms with coefficient $q^2$ in the expansion of $D_q^m$ and the coefficient of $(aek)^{m-1}ceg$ in the decomposition of these terms is $\frac{-(q^2-1)^2}{q^3}$. There are $n$ many $(aek)^lceg(aek)^{m-1-l}$ terms with coefficient $-q^3$ in the expansion of $D_q^m$ and the coefficient of $(aek)^{m-1}ceg$ in the decomposition of these terms is $1$. Together, the coefficient of $(aek)^{m-1}ceg$ in the decomposition of $D_q^m$ is:
\begin{equation*}
    \begin{split}
        &-mq^3-\frac{m(m-1)}{2}q^2\frac{(q^2-1)^2}{q^3}\\
        =&-\frac{m(m+1)}{2}q^3+m(m-1)q-\frac{m(m-1)}{2}q^{-1}
    \end{split}
\end{equation*}
The contribution from comparing basis $(aek)^{m-1}ceg$ is:
\begin{equation*}
    \begin{split}
        &\sum_{l=0}^{m-1}\sum_{k=0}^{m-1-l}(q-q^{-1})^2q^{-4k-1}-(q^3-q)q^{-2k}\\
        =&\frac{q^{-4m+3}-q^{-4m+1}-q^{-2m+7}-2q^{-2m+5}-q^{-2m+3}}{(q^2-1)(q^2+1)^2}\\
        &+\frac{-mq^9+q^7+2q^5+(m+1)q}{(q^2-1)(q^2+1)^2}
    \end{split}
\end{equation*}
Together, \textbf{the coefficient of} $(ceg)^m$ is:
\begin{equation*}
    \begin{split}
        &\frac{(3m-m^2-2)q^3}{2}+(m^2-2m-1)q+\frac{m+2-m^2}{2q}+(m+1)q^{-2m+3}\\
        &+(1-2m)q^{-2m+1}+(m-1)q^{-2m-1}\\
        &+q^{-2m}(q^3-mq+mq^3)+\frac{(m^2+m-2)q^3}{2}+(\frac{1}{2q}-q)(m^2+m)\\
        &-\frac{q^{-4m-3}+2q^{-4m-1}}{(1+q^{-2})^2}+(2m+1)q^{-2m+1}+q^{-2m-1}-2(m+1)q^{-2m+3}\\
        &-\frac{(m^2+3m-4)q^3-(2m+6)q-(2m^2+6m+2)q^{-1}+(2m+4)q^{-3}}{2(1+q^{-2})^2}\\
        &-\frac{(m^2+3m+2)q^{-5}}{2(1+q^{-2})^2}\\
        &+\frac{(1-m)q^5+q^3+(m+1)q-q^{-2m+5}-2q^{-2m+3}-q^{-2m+1}+q^{-4m+3}}{(q^2+1)^2}\\
        &-\frac{(m-1)q^5-q^3-(m+1)q+q^{-2m+5}+2q^{-2m+3}-q^{-4m+3}+q^{-2m+1}}{(q^2+1)^2}\\
        &+\frac{q^{-4m+3}-q^{-4m+1}-q^{-2m+7}-2q^{-2m+5}-q^{-2m+3}}{(q^2-1)(q^2+1)^2}\\
        &+\frac{-mq^9+q^7+2q^5+(m+1)q}{(q^2-1)(q^2+1)^2}\\
        &-\left[-\frac{m(m+1)}{2}q^3+m(m-1)q-\frac{m(m-1)}{2}q^{-1}\right]\\
        =&\frac{(q^{2m}-1)(mq^4-2mq^2+m+q^4)}{q^{2m+1}(q^2-1)}
    \end{split}
\end{equation*}

==> Chapters/basis_of_3.tex <==
\section{A monomial basis consisting of standard monomials}\label{basis_of_3}
In this section, we will provide a criterion to pick a monomial basis from the set of all standard monomials and define a monomials basis based on the criterion.
\begin{proposition}\label{prop 6}
    Let $M=(m_{ij})_{i,j=1}^3$ be a $3\times 3$ $k$-doubly stochastic matrix. If there exist $1\le i',j'\le 3$ such that $m_{i',j'}=0$, then $M$ is uniquely decomposed into a linear combination of matrices in $A_3(1)$.
\end{proposition}
\begin{proof}
    Index the 6 matrices in $A_3(1)$ as:
    \begin{multicols}{3}
        \begin{enumerate}
            \item[] \begin{equation*}
                S_1=\begin{bmatrix}
            1&0&0\\
            0&1&0\\
            0&0&1
        \end{bmatrix}
            \end{equation*}
        \item[] \begin{equation*}
            S_2=\begin{bmatrix}
            1&0&0\\
            0&0&1\\
            0&1&0
        \end{bmatrix}
        \end{equation*}
        \item[] \begin{equation*}
            S_3=\begin{bmatrix}
            0&0&1\\
            0&1&0\\
            1&0&0
        \end{bmatrix}
        \end{equation*}
        \item[] \begin{equation*}
        S_4=\begin{bmatrix}
            0&1&0\\
            1&0&0\\
            0&0&1
        \end{bmatrix}
    \end{equation*}
    \item[] \begin{equation*}
        S_5=\begin{bmatrix}
            0&1&0\\
            0&0&1\\
            1&0&0
        \end{bmatrix}
    \end{equation*}
    \item[] \begin{equation*}
        S_6=\begin{bmatrix}
            0&0&1\\
            1&0&0\\
            0&1&0
        \end{bmatrix}
    \end{equation*}
    \end{enumerate}
    \end{multicols}
    \noindent Without loss of generality, assume that $m_{11}=0$. Then, matrix $S_1$ and $S_2$ cannot appear in the decomposition of $M$. The only matrix in $A_3(1)$ whose $(2,2)$-entry is not zero is $S_3$. Hence, the coefficient of $S_3$ in the decomposition of $M$ is $m_{22}$. Similarly, the only matrix in $A_3(1)$ whose $(3,3)$-entry is not zero is $S_4$, so the coefficient of $S_4$ in the decomposition of $M$ is $m_{33}$; the only matrix in $A_3(1)$ whose $(2,3)$-entry is not zero is $S_5$, so the coefficient of $S_5$ in the decomposition of $M$ is $m_{23}$; the only matrix in $A_3(1)$ whose $(3,2)$-entry is not zero is $S_6$, so the coefficient of $S_6$ in the decomposition of $M$ is $m_{32}$. Hence, $M$ is decomposed into:
    $$M=m_{22}\cdot S_3+m_{33}\cdot S_4+m_{23}\cdot S_5+m_{32}\cdot S_6.$$
    The arguments for other cases are identical to $m_{11}=0$
\end{proof}
\noindent Denote 
\begin{equation*}
    F=\begin{bmatrix}
        1&1&1\\
        1&1&1\\
        1&1&1
    \end{bmatrix}
\end{equation*}
Then, every $3\times 3$ $k$-doubly stochastic matrix $M$ can be written as:
$$M=a\cdot F+N$$
where $a=\text{min}\{m_{i,j},1\le i,j\le 3\}$ and $N$ is a $(k-3a)$-doubly stochastic matrix with at least one entry equals to $0$. By Proposition \ref{prop 6}, the decomposition of $N$ is unique. To define a monomial basis consisting of standard monomials, we need to specify the decomposition of matrix $F$. In this paper, we choose the standard monomial corresponding to matrix $F$ as:
$$aekbfgcdh.$$
Thus, if the unique standard monomial corresponding to $N$ is:
$$(aek)^{n_1}(afh)^{n_2}(bdk)^{n_3}(bfg)^{n_4}(cdh)^{n_5}(ceg)^{n_6},$$
the standard monomial corresponding to $M$ is:
$$(aek)^{n_1+a}(afh)^{n_2}(bdk)^{n_3}(bfg)^{n_4+a}(cdh)^{n_5+a}(ceg)^{n_6}.$$
Notice that in the monomial corresponding to $N$, at least one of $n_1$, $n_4$, and $n_5$ has to be zero since $N$ has a zero entry. For the same reason, at least one of $n_2$, $n_3$, and $n_6$ has to be zero. This implies that for every $k$-doubly stochastic matrix $M$, the corresponding standard monomial contains at most two of the three segments $afh$, $bdk$, $ceg$. Hence, we define the \textbf{monomial basis consisting of standard monomials} as:
$$\{(aek)^{m_1}(afh)^{m_2}(bdk)^{m_3}(bfg)^{m_4}(cdh)^{m_5}(ceg)^{m_6}, m_i\in\mathbf{N}_0 \text{ and } m_2\cdot m_3\cdot m_6=0\}.$$

==> Chapters/chdceg_recursive.tex <==
\section{The recursive relation for the Haar state of standard monomials in the form of $(cdh)^i(ceg)^{m-i}$ and $(bfg)^i(ceg)^{m-i}$}
Recall the double flip anti-homomorphism $\omega$ which preserves the Haar state value. Applying $\omega$ to $(cdh)^i(ceg)^{m-i}$ and using the fact that low-complexity segments commute with each other, we get:
$$\omega\left((cdh)^i(ceg)^{m-i}\right)=(ceg)^{m-i}(bfg)^i=(bfg)^i(ceg)^{m-i}.$$
Thus, $h\left((cdh)^i(ceg)^{m-i}\right)=h\left((bfg)^i(ceg)^{m-i}\right)$. In the following, we will derive the recursive relation of $h\left((cdh)^i(ceg)^{m-i}\right)$ and the relation is true for $h\left((bfg)^i(ceg)^{m-i}\right)$ as well.\\
\\
The case $i=1$ is solved in the Source Matrix. We will start with the general case $3\le i\le m-1$ and the case $i=2, m$ are special cases of the general case.  

\subsection{Recursive relation of $3\le i\le m-1$}
We use the linear relation derived from $(cdh)^{i-1}(ceg)^{m-i+1}$ and equation basis $(aek)^{m-1}afh$ to derive the recursive relation of the Haar state of $(cdh)^{i}(ceg)^{m-i}$. As discussed before, the left components containing $(aek)^{m-1}afh$ are
\begin{enumerate}
    \item[1)] $(aek)^lafh(aek)^{m-1-l}$
    \item[2)] $(aek)^lafk(aek)^kaeh(aek)^{m-2-l-k}$
    \item[3)] $(aek)^laeh(aek)^kafk(aek)^{m-2-l-k}$ 
\end{enumerate}
\noindent When the left component is in the form $(aek)^lafh(aek)^{m-1-l}$, the coefficient of $(aek)^{m-1}afh$ in the decomposition of $(aek)^lafh(aek)^{m-1-l}$ is $1$ and the corresponding relation components are:
\begin{itemize}
    \item[1)] $(cdh)^lcge(cdh)^{i-2-l}(ceg)^{m-i+1}$ 
    \item[2)] $(cdh)^{i-1}(ceg)^lchd(ceg)^{m-i-l}$
\end{itemize}
When the left component is in the form $(aek)^lafk(aek)^kaeh(aek)^{m-2-l-k}$, the coefficient of $(aek)^{m-1}afh$ in the decomposition of $(aek)^lafk(aek)^kaeh(aek)^{m-2-l-k}$ is $1$ and the corresponding relation components are:
\begin{itemize}
    \item[3)] $(cdh)^lcgh(cdh)^kcde(cdh)^{i-3-l-k}(ceg)^{m-i+1}$
    \item[4)] $(cdh)^lcgh(cdh)^{i-2-l}(ceg)^kced(ceg)^{m-i-k}$
    \item[5)] $(cdh)^{i-1}(ceg)^lchg(ceg)^kced(ceg)^{m-i-1-l-k}$
\end{itemize}
When the left component is in the form $(aek)^laeh(aek)^kafk(aek)^{m-2-l-k}$, the coefficient of $(aek)^{m-1}afh$ in the decomposition of $(aek)^laeh(aek)^kafk(aek)^{m-2-l-k}$ is $q^2$ and the corresponding relation components are:
\begin{itemize}
    \item[6)] $(cdh)^lcde(cdh)^kcgh(cdh)^{i-3-l-k}(ceg)^{m-i+1}$
    \item[7)] $(cdh)^lcde(cdh)^{i-2-l}(ceg)^kchg(ceg)^{m-i-k}$
    \item[8)] $(cdh)^{i-1}(ceg)^lced(ceg)^kchg(ceg)^{m-i-1-l-k}$
\end{itemize}
For case 1), we have:
\begin{equation*}
    (cdh)^lcge(cdh)^{i-2-l}(ceg)^{m-i+1}=(cdh)^{i-2}(ceg)^{m-i+2}
\end{equation*}
The contribution of case 1) to the linear relation is:
\begin{equation*}
    (i-1)(cdh)^{i-2}(ceg)^{m-i+2}
\end{equation*}
For case 2), we have:
\begin{equation*}
    (cdh)^{i-1}(ceg)^lchd(ceg)^{m-i-l}=(cdh)^{i}(ceg)^{m-i}-(q-1/q)*(cdh)^{i-1}(ceg)^{m-i+1}
\end{equation*}
The contribution of case 2) to the linear relation is:
\begin{equation*}
    (m-i+1)*(cdh)^{i}(ceg)^{m-i}-(m-i+1)(q-1/q)*(cdh)^{i-1}(ceg)^{m-i+1}
\end{equation*}
For case 3), we have:
\begin{equation*}
    \begin{split}
        &(cdh)^lcgh(cdh)^kcde(cdh)^{i-3-l-k}(ceg)^{m-i+1}\\
        &=(cdh)^l(chd)^{k+1}(cdh)^{i-3-l-k}(ceg)^{m-i+2}\\
        &=(cdh)^l(cdh-(q-1/q)ceg)^{k+1}(cdh)^{i-3-l-k}(ceg)^{m-i+2}\\
        &=\sum_{j=0}^{k+1}(-(q-1/q))^j{k+1\choose j}(cdh)^{i-2-j}(ceg)^{m-i+2+j}
    \end{split}
\end{equation*}
The contribution of case 3) to the linear relation is:
\begin{equation*}
\begin{split}
    &\sum_{l=0}^{i-3}\sum_{k=0}^{i-3-l}\sum_{j=0}^{k+1}(-(q-1/q))^j{k+1\choose j}(cdh)^{i-2-j}(ceg)^{m-i+2+j}\\
    &+\sum_{l=0}^{i-3}\sum_{j=1}^{i-2-l}(-(q-1/q))^j{i-1-l\choose j+1}(cdh)^{i-2-j}(ceg)^{m-i+2+j}\\
    =&\frac{(i-1)(i-2)}{2}*(cdh)^{i-2}(ceg)^{m-i+2}\\
    &+\sum_{k=3}^{i}(-(q-1/q))^{k-2}{i\choose k}(cdh)^{i-k}(ceg)^{m-i+k}\\
\end{split}
\end{equation*}
For case 4), we have:
\begin{equation*}
    \begin{split}
        &(cdh)^lcgh(cdh)^{i-2-l}(ceg)^kced(ceg)^{m-i-k}\\
        &=q^{-2k-1}*(cdh)^l(chd)^{i-1-l}(ceg)^{m-i+1}\\
        &=q^{-2k-1}\sum_{j=0}^{i-1-l}(-(q-1/q))^j{i-1-l\choose j}*(cdh)^{i-1-j}(ceg)^{m-i+1+j}\\
    \end{split}
\end{equation*}
The contribution of case 4) to the linear relation is:
\begin{equation*}
\begin{split}
    &\sum_{k=0}^{m-i}q^{-2k-1}\sum_{l=0}^{i-2}\sum_{j=0}^{i-1-l}(-(q-1/q))^j{i-1-l\choose j}*(cdh)^{i-1-j}(ceg)^{m-i+1+j}\\
    &\sum_{k=0}^{m-i}q^{-2k-1}\sum_{l=1}^{i-1}\sum_{j=0}^{l}(-(q-1/q))^j{l\choose j}*(cdh)^{i-1-j}(ceg)^{m-i+1+j}\\
    =&q^{-1}\frac{1-q^{-2(m-i+1)}}{1-q^{-2}}((i-1)(cdh)^{i-1}(ceg)^{m-i+1}\\
    &+\sum_{k=2}^{i}(-(q-1/q))^{k-1}{i \choose k}*(cdh)^{i-k}(ceg)^{m-i+k})
\end{split}
\end{equation*}
For case 5), we have:
\begin{equation*}
    \begin{split}
        &(cdh)^{i-1}(ceg)^lchg(ceg)^kced(ceg)^{m-i-1-l-k}\\
        =&(cdh)^{i-1}(ceg)^lch(ceg)^{k+1}d(ceg)^{m-i-1-l-k}\\
        =&q^{-2k-2}*(cdh)^{i-1}chd(ceg)^{m-i}\\
        =&q^{-2k-2}*((cdh)^{i}(ceg)^{m-i}-(q-1/q)*(cdh)^{i-1}(ceg)^{m-i+1})
    \end{split}
\end{equation*}
The contribution of case 5) to the linear relation is:
\begin{equation*}
\begin{split}
    &\sum_{l=0}^{m-i-1}\sum_{k=0}^{m-i-1-l}q^{-2k-2}*((cdh)^{i}(ceg)^{m-i}-(q-1/q)*(cdh)^{i-1}(ceg)^{m-i+1})\\
    =&(\frac{m-i}{q^2-1}+\frac{q^{-2(m-i)}-1}{(1-q^2)^2})*((cdh)^{i}(ceg)^{m-i}-(q-1/q)*(cdh)^{i-1}(ceg)^{m-i+1})
\end{split}
\end{equation*}
For case 6), we have:
\begin{equation*}
    \begin{split}
        &(cdh)^lcde(cdh)^kcgh(cdh)^{i-3-l-k}(ceg)^{m-i+1}\\
        =&q^2*(cdh)^lcd(cdh)^kh(cdh)^{i-3-l-k}(ceg)^{m-i+2}\\
        =&q^2*(cdh)^lcd(hcd+(q+1/q)*ceg)^kh(cdh)^{i-3-l-k}(ceg)^{m-i+2}\\
        =&q^2\sum_{j=0}^k(q-1/q)^j{k \choose j}*(cdh)^{l+k-j}cd(ceg)^jh(cdh)^{i-3-l-k}(ceg)^{m-i+2}\\
        =&q^2\sum_{j=0}^k(q-1/q)^jq^{2j}{k \choose j}*(cdh)^{i-2-j}(ceg)^{m-i+2+j}\\
    \end{split}
\end{equation*}
The contribution of case 6) to the linear relation is:
\begin{equation*}
\begin{split}
    &q^4\sum_{l=0}^{i-3}\sum_{k=0}^{i-3-l}\sum_{j=0}^k(q-1/q)^jq^{2j}{k \choose j}*(cdh)^{i-2-j}(ceg)^{m-i+2+j}\\
    &=\sum_{k=2}^{i-1}(q-1/q)^{k-2}q^{2k}{i-1\choose k}*(cdh)^{i-k}(ceg)^{m-i+k}
\end{split}
\end{equation*}
For case 7), we have:
\begin{equation*}
    \begin{split}
        &(cdh)^lcde(cdh)^{i-2-l}(ceg)^kchg(ceg)^{m-i-k}\\
        =&q^{2k+1}\sum_{j=0}^{i-2-l}(q-1/q)^jq^{2j}{i-2-l\choose j}*(cdh)^{i-1-j}(ceg)^{m-i+1+j}\\
    \end{split}
\end{equation*}
The contribution of case 7) to the linear relation is:
\begin{equation*}
\begin{split}
    &q^2\sum_{k=0}^{m-i}q^{2k+1}\sum_{l=0}^{i-2}\sum_{j=0}^{i-2-l}(q-1/q)^jq^{2j}{i-2-l\choose j}*(cdh)^{i-1-j}(ceg)^{m-i+1+j}\\
     =&q\frac{1-q^{2(m-i+1)}}{1-q^2}\sum_{k=1}^{i-1}(q-1/q)^{k-1}q^{2k}{i-1\choose k}*(cdh)^{i-k}(ceg)^{m-i+k}
\end{split}
\end{equation*}
For case 8), we have:
\begin{equation*}
    \begin{split}
        &(cdh)^{i-1}(ceg)^lced(ceg)^kchg(ceg)^{m-i-1-l-k}\\
        =&q^{2k}*(cdh)^{i}(ceg)^{m-i}
    \end{split}
\end{equation*}
The contribution of case 8) to the linear relation is:
\begin{equation*}
\begin{split}
    &q^2\sum_{l=0}^{m-i-1}\sum_{k=0}^{m-i-1-l}q^{2k}*(cdh)^{i}(ceg)^{m-i}\\
    =&\left(\frac{(m-i)q^2}{1-q^2}+\frac{q^4(q^{2(m-i)}-1)}{(1-q^{2})^2}\right)*(cdh)^{i}(ceg)^{m-i}
\end{split}
\end{equation*}
The term $(cdh)^{i}(ceg)^{m-i}$ appears in case 2), 5), and 8). Summing the contributions from these cases, the coefficient of $(cdh)^{i}(ceg)^{m-i}$ is:
\begin{equation*}
    \begin{split}
        &\frac{q^2(q^{m-i+1}-q^{-(m-i+1)})^2}{(1-q^2)^2}
    \end{split}
\end{equation*}
The term $(cdh)^{i-1}(ceg)^{m-i+1}$ appears in case 2), 4), 5), 7), and the right-hand side of Equation (\ref{eq:3}). Summing the contributions from these cases, the coefficient of $(cdh)^{i-1}(ceg)^{m-i+1}$ is:
\begin{equation*}
    \begin{split}
        &\frac{-(i-1)q^{2(m-i)+5}+iq^{-2(m-i)-1}-q}{(1-q^2)}
    \end{split}
\end{equation*}
The term $(cdh)^{i-2}(ceg)^{m-i+2}$ appears in case 1), 3), 4), 6), and 7). Notice that if we combine the contribution of case 1) and case 3), we get:
\begin{equation*}
    (i-1)+\frac{(i-1)(i-2)}{2}=\frac{i(i-1)}{2}={i\choose 2}
\end{equation*}
which corresponds to $k=2$ in the summation of case 3). Thus, we can treat $(cdh)^{i-2}(ceg)^{m-i+2}$ in the same way as the general case $(cdh)^{i-k}(ceg)^{m-i+k}$, $3\le k\le i-1$ which appears in case 3), 4), 6), and 7). Summing the contributions from these cases, the coefficient of $(cdh)^{i-k}(ceg)^{m-i+k}$ for $2\le k\le i-1$ is:
\begin{equation*}
    \begin{split}
        &(q^{-1}-q)^{k-2}{i\choose k}q^{-2(m-i+1)}+(q-q^{-1})^{k-2}q^{2k}{i-1\choose k}q^{2(m-i+1)}
    \end{split}
\end{equation*}
Notice that if we put $k=1$ in the above coefficient, we get:
\begin{equation*}
    \begin{split}
        &(q^{-1}-q)^{-1}iq^{-2(m-i+1)}+(q-q^{-1})^{-1}q^2(i-1)q^{2(m-i+1)}\\
        =&\frac{iq^{-2m+2i-1}-(i-1)q^{2m-2i+5}}{1-q^2}
    \end{split}
\end{equation*}
The term $(ceg)^m$ appears in case 3) and 4). Summing the contributions from these cases, the coefficient of $(ceg)^{m}$ is:
\begin{equation*}
\begin{split}
    &(q^{-1}-q)^{i-2}q^{-2(m-i+1)}
\end{split}
\end{equation*}
The expressions of the coefficients of $(cdh)^{i-2}(ceg)^{m-i+2}$ and $(cdh)^{i-k}(ceg)^{m-i+k}$ for $3\le k\le i-1$ are consistent. Thus, the expression of $(cdh)^{i}(ceg)^{m-i}$ is:
\begin{equation}
    \begin{split}
         &\frac{q^2(q^{m-i+1}-q^{-(m-i+1)})^2}{(1-q^2)^2}*h((cdh)^i(ceg)^{m-i})\\
         =&-\frac{q}{q^2-1}*h((cdh)^{i-1}(ceg)^{m-i+1})\\     
         &-\sum_{k=1}^{i-1}c_k*h((cdh)^{i-k}(ceg)^{m-i+k})-(q^{-1}-q)^{i-2}q^{-2(m-i+1)}h((ceg)^{m})\\
    \end{split}\label{recursive:1}
\end{equation}
where
\begin{equation*}
\begin{split}
    c_k=(q^{-1}-q)^{k-2}{i\choose k}q^{-2(m-i+1)}+(q-1/q)^{k-2}q^{2k}{i-1\choose k}q^{2(m-i+1)}.
\end{split}
\end{equation*}
\subsection{$i=2$}
We use the linear relation derived from $cdh(ceg)^{m-1}$ and equation basis $(aek)^{m-1}afh$. The situation in this subsection is similar to the previous subsection but we do not have case 3) and 6) anymore. The linear relation in this case only involves $(cdh)^2(ceg)^{m-2}$, $cdh(ceg)^{m-1}$, and $(ceg)^m$. Here, $(ceg)^m$ is the same as $(cdh)^{i-2}(ceg)^{m-i+2}$ in the previous subsection. If we substitute $i=2$ into the contribution of case 3) and 6), we find that the contributions corresponding the two cases are automatically zero. Thus, recursive relation Equation (\ref{recursive:1}) is consistent with the case in subsection 10.2.


\subsection{$i=m$}
We use the linear relation derived from $(cdh)^{m-1}ceg$ and equation basis $(aek)^{m-1}afh$. The situation in this subsection is similar to the previous subsection but we do not have case 5) and 8) anymore. Thus, the coefficient of $(cdh)^m$ is $1$ and the coefficient of $(cdh)^{m-1}ceg$ is:
\begin{equation*}
    \begin{split}
        &-(q-1/q)+q^{-1}(m-1)+q^3(m-1)+mq\\
        &=mq^{-1}+(m-1)q+(m-1)q^3
    \end{split}
\end{equation*}
On the other hand, if we substitute $i=m$ in to the coefficient of $(cdh)^{i}(ceg)^{m-i}=(cdh)^{m}$, we get $1$ and coefficient of $(cdh)^{i-1}(ceg)^{m-i+1}=(cdh)^{m-1}ceg$, we get:
\begin{equation*}
    \begin{split}
        &\frac{mq^{-1}-(m-1)q^{5}-q}{1-q^2}\\
        &=(m-1)q^3+(m-1)q+mq^{-1}
    \end{split}
\end{equation*}
Thus, recursive relation Equation (\ref{recursive:1}) is consistent with the case in subsection 10.3.

==> ack.tex <==
\section*{Acknowledgement}

\noindent
This author is advised by Professor Jeffrey Kuan from Texas A\&M University and Professor Micheal Brannan from University of Waterloo.
This work is partially funded by National Science Foundation (NSF grant DMS-2000331).
